Maximizing Welfare in Social Networks under a Utility Driven Influence Diffusion Model

Motivated by applications such as viral marketing, the problem of influence maximization (IM) has been extensively studied in the literature. The goal is to select a small number of users to adopt an item such that it results in a large cascade of adoptions by others. Existing works have three key limitations. (1) They do not account for economic considerations of a user in buying/adopting items. (2) Most studies on multiple items focus on competition, with complementary items receiving limited attention. (3) For the network owner, maximizing social welfare is important to ensure customer loyalty, which is not addressed in prior work in the IM literature. In this paper, we address all three limitations and propose a novel model called UIC that combines utility-driven item adoption with influence propagation over networks. Focusing on the mutually complementary setting, we formulate the problem of social welfare maximization in this novel setting. We show that while the objective function is neither submodular nor supermodular, surprisingly a simple greedy allocation algorithm achieves a factor of $(1-1/e-\epsilon)$ of the optimum expected social welfare. We develop \textsf{bundleGRD}, a scalable version of this approximation algorithm, and demonstrate, with comprehensive experiments on real and synthetic datasets, that it significantly outperforms all baselines.

==> sec-algos.tex <==
\note[Laks]{suggested org of this section. \\ 
- main result \\ 
  + greedy algorithm \\ 
  + main theorem \\ 
- social welfare accounting technique \\ 
  + technique \\ 
  + proof \\
- preserving prefix property \\ 
  + primm algorithm 
  + proof of correctness and running time complexity. \\ 
- putting it all together 
  + summary of how pieces fit together} 

\subsection{Overview}\label{sec:overview} 

Given that the welfare function is neither submodular nor supermodular, designing an efficient approximation algorithm for WelMax is challenging. Nevertheless, in this section we show that for given $\epsilon$ and $\ell$, a $(1-\frac{1}{e} - \epsilon)$-approximation to the optimal welfare can be achieved with probability at least $1 - \frac{1}{|V|^{\ell}}$, using a simple greedy algorithm. To the best of our knowledge, this is the first instance in the context of viral marketing, where we are able to guarantee an {\sl efficient approximation for a non-submodular objective at the same level as has been done in the literature for submodular objectives}. We first present our algorithm and then proceed to analyzing its correctness and efficiency.

Our algorithm, called $\algo$ (for Greedy Welfare Maximization) and shown Algorithm \ref{alg:greedy_allocation}, is based on greedy allocation of seed nodes to items. Given a graph $G$, the universe of items $\allitems$, item  budget vector $\bvec$, $\epsilon$, and $\ell$, $\algo$ first selects the top-$\bmax$ seed nodes $\greedSeeds$ for the IC model (disregarding item utilities), where $\bmax = max\{b_i \mid b_i\in \bvec \}$. We will show that it achieves a $(1-\frac{1}{e} - \epsilon)$-approximation to the optimal expected social welfare. For this to work, the algorithm must ensure that the $\bmax$ seeds $S_{\bmax}$ selected satisfy a \emph{prefix preserving} property. It intuitively says that for every budget $b_i \in \bvec$, the top-$b_i$ seeds among $\greedSeeds$ provide a $(1-\frac{1}{e} - \epsilon)$-approximation to the optimal expected spread under budget $b_i$. This property is ensured by invoking the $\PRIMM$ algorithm (Algorithm~\ref{alg:IMM_adopted}) in line~\ref{alg:PRIMM} of Algorithm~\ref{alg:greedy_allocation}. Algorithm~\ref{alg:IMM_adopted} is described and its correctness and running time complexity are establihsed in Section~\ref{sec:PRIMM}.  
\eat{
Note that we need to user a prefix-preserving influence maximization for this purpose to find
	an ordered seed set $\greedSeeds$ (details to be explained shortly). 
} 
Then $\algo$ allocates the top-$b_i$ nodes in $\greedSeeds$ as seeds for each item $i \in \allitems$. Here is a preview of the main result of this section. 


%\weic{I think it is important to provide the theorem summarizing the result here, rather than give at the end of the analysis.}

\begin{theorem-non}\label{thm:main}
	Let $\greedAlloc$ be the greedy allocation  generated by $\algo$, 
	and $\optAlloc$	be the optimal allocation. 
	Given $\epsilon>0$ and $\ell>0$, with probability at least $1 - \frac{1}{|V|^{\ell}}$, 
	we have 
	\begin{equation} \label{eq:approxsw}
	\sw(\greedAlloc) \geq (1 - \frac{1}{e} - \epsilon ) \cdot \sw(\optAlloc).
	\end{equation}
The running time of $\algo$ is $O((\bmax+\ell)(m+n)\log n / \epsilon^2)$.
\end{theorem-non}

The proof of this result is highly non-trivial. In the next section, we develop a novel accounting technique for calculating the expected social welfare of a given allocation and leverage it to prove the above theorem. 

\eat{ 
\weic{
I am not sure about the running time result, since Prithu has not finished the analysis of the {\PRIMM} algorithm.
In particular, I am not sure if we would add factor $|\allitems|$ into the running time.
}
} 

Our algorithm $\algo$ has the remarkable property that it actually does not need access to the valuation functions,
prices, and the distribution of noises as input, and thus the algorithm works for all possible utility settings. 
This means that the algorithm does not rely on potentially complicated and hard-to-get product utility information.
It precisely reflects the power of bundling in the mutually complementary setting --- as long as we know that
	all items are mutually complementary, then bundling them together as much as possible would always provide
	a good solution in terms of social welfare, no matter what the actual utilities. This is significant since most of the known algorithms for social welfare maximization in the auction literature typically assume a value oracle, which given a query as an itemset, returns the utility of the itemset. Realizing such an oracle can be quite expensive in practice for non-additive utility functions, since there are exponentially many itemsets. 

\eat{ 
\weic{I think is important to give the high level idea of the analysis of the block method here before
	delving into the technical details. Also, this part of the analysis is more important than the
	prefix-preserving algorithm, so should be explained first. The following is my addition of such an explanation.}
} 

%We now proceed to analyze the approximation guarantee that $\algo$ provides.
The analysis of the algorithm is highly non-trivial, because it needs to consider all possible seed allocations, propagation scenarios, even when budgets are not uniform among items.
Our main idea is a ``block'' based accounting method: we break the items into ``atomic'' blocks, in the sense that
	each block has non-negative marginal utility given previous blocks, so that it can propagate as an atomic
	unit in the diffusion process.
Then we account for each block's contribution to the social welfare during a  propagation, and argue that for
	every block, the contribution of the block achieved by the greedy allocation is always at least 
	$(1-1/e - \epsilon)$ times the contribution under any allocation.
The technical subtlety of the analysis includes properly defining the blocks, showing why each blocks can be
	accounted for separately, dealing with partial item propagation within blocks, etc.

\eat{ 
For ease of understanding, we first present the analysis for the uniform budget case in 
	Section~\ref{sec:same_budget}, which contains the basic ideas in the block-based accounting analysis.
We then present the additional analysis needed for the nonuniform budget case in Section~\ref{sec:nonuniformBudget}.
} 

\eat{
Our algorithm also needs an extension to the existing influence maximization algorithm to make it
	prefix-preserving, as we now explain. 
} 
We now formalize the prefix preserving property mentioned above. Recall that this property requires that every prefix of size $b_i$ of $\greedSeeds$ should be an approximately optimal solution to influence maximization under budget $b_i$, where $b_i \in \bvec$. One way of trivially satisfying this property is to find the {\sl exact} greedy solution.  However, exact computation of expected spread (and hence marginal gain) is intractable \cite{}. Known scalable approximation algorithms for IM such as TIM \cite{}, IMM \cite{}, SSA \cite{} only provide an approximately optimal solution with a certain (high) probability. If such an algorithm is used to find $S_{\bmax} = \greedSeeds$, there is no guarantee that the top-$b_i$ seeds in $\greedSeeds$ will be approximately optimal for IM under budget $b_i$. We formalize the prefix preserving property next. 
\eat{ 
E.g.,  given $\epsilon$ and $\ell$, state-of-the-art influence maximization algorithms like IMM \cite{tang15} find a seed set $\greedSeeds$ such that $\sigma(\greedSeeds) \geq (1-\frac{1}{e} - \epsilon)\sigma(\optSeeds)$ with probability at least $1 - \frac{1}{|V|^{\ell}}$,  where $\greedSeeds$ and $\optSeeds$ are the greedy and the optimal seed set of size $\bmax$ respectively and $\sigma(\cdot)$ denotes the expected spread in graph $G$. For our social welfare algorithm to work properly, we further require 
	that the algorithm be prefix-preserving with respect to a budget vector $\bvec$, 
	as we formally define below.
} 

\eat{ 
\weic{
The old definition talks about a set satisfying the prefix order probability with high probability.
This is not accurate, because a set by itself has no associated probabilistic event.
We can only say an algorithm finds such a set with certain probability.
So I rephrased the following definition.} 
} 

Let $S_{b_i}$ denote the top-$b_i$ nodes chosen by the greedy algorithm for IM and let $OPT_{b_i}$ denote the optimal expected spread of $b_i$ nodes. We will assume that the nodes in $S_{b_i}$ are arranged in non-decreasing order of their marginal gain. 

\begin{definition}{\sc (Prefix Preserving Property).\ \ }\label{def:PRIMM}
Given $G = (V,E,p)$ and any budget vector $\bvec$, we say that an influence maximization algorithm $A$
	is {\em prefix-preserving} w.r.t. $\bvec$, 
	if for any $\epsilon>0$ and $\ell > 0$, 
	it returns an ordered set $\greedSeeds_{\bmax}$ of size $\bmax$, 
	such that  with probability  at least $1 - \frac{1}{|V|^{\ell}}$, 
	for every $b_i \in \bvec$, the top-$b_i$ nodes of $\greedSeeds_{\bmax}$, denoted $\greedSeeds_{b_i}$, satisfies $\sigma(\greedSeeds_{b_i}) \geq (1-\frac{1}{e} - \epsilon)OPT_{b_i}$, %\sigma(\optSeeds_{b_i})$, 
	where %$\optSeeds_{b_i}$ is the optimal seed set with $b_i$ seeds in the IC model.
$OPT_{b_i}$ is the optimal expected spread of $b_i$ nodes. 
\end{definition}

Unfortunately state-of-the-art IM algorithms \cite{tang15, Nguyen2016, Huang2017} are not
	prefix-preserving out-of-the-box. 
We present a non-trivial extension of IMM \cite{tang15}, called $\PRIMM$ (PRefix IMM), 
	to make it prefix-preserving.
We defer the presentation of $\PRIMM$ to Section~\ref{sec:PRIMM}.

%Specifically the rest of the section is organized as follows, first we prove the approximation guarantee of our algorithm under a simpler setting where we assume all items have same budget. Then we prove under non-uniform budget. Notice that our algorithm is same for both uniform and non-uniform cases. It does not require any modification for the non-uniform budget. However for the ease of understanding of the reader, we first present the simpler uniform budget case and then move onto general non-uniform budget. Finally we present our proposed extension, $\PRIMM$. 

%\SetAlgoSkip{}
\begin{algorithm}[t!]
%\begin{small}
\DontPrintSemicolon
\caption{  $\algo(\allitems, \bvec, G, \epsilon, \ell)$} \label{alg:greedy_allocation}
%Sort the items in non-increasing order of their budgets, i.e., $b_1 \geq ... \geq b_m$ \;
$\greedAlloc \leftarrow \emptyset$; \\ 
Let $\greedSeeds$ be the top $\bmax$ seeds selected using a 
	prefix-preserving influence maximization algorithm under the IC model over graph $G$
	and budget vector $\bvec$, 
	, i.e., $\greedSeeds \leftarrow \PRIMM(\bvec, G, \epsilon, \ell)$;  \label{alg:PRIMM} \\
\For{$i \in \allitems$}  {
	Assign the top $b_i$ nodes of $\greedSeeds$ to item $i$, i.e.,  $\greedSeeds_i \leftarrow \mbox{ top } b_i \mbox{ nodes from } \greedSeeds$  \;
	$\greedAlloc \leftarrow \greedAlloc \cup (\{i\} \cdot \greedSeeds_i)$ \;}	
%
\textbf{return} $\greedAlloc$ as the final allocation\;  
%\end{small}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{
In this paper we use state of the art IMM algorithm \cite{tang15}, to select the top $\bmax$ seeds. However, the nodes setlected by IMM does not have the prefix order property. Hence we extend the IMM algorithm for our purpose. Specifically the algorithm 2 of \cite{tang15} is modified as shown in algorithm \ref{alg:IMM_adopted}. Algorithm 1 and 3 of \cite{tang15} remains same. For brevity, we do not to repeat them in this paper.  

%\SetAlgoSkip{}
\begin{algorithm}[t!]
%\begin{small}
\DontPrintSemicolon
\caption{Greedy Allocation$(I, \bvec,G)$} \label{alg:IMM_adopted}
%Sort the items in non-increasing order of their budgets, i.e., $b_1 \geq ... \geq b_m$ \;
$\greedAlloc \leftarrow \emptyset$; \\ 
Let $\greedSeeds$ be the top $\bmax$ seeds selected using a influence maximization algorithm that preserves prefix order property, under the IC model over graph $G$, i.e., $\greedSeeds \leftarrow \texttt{IM}(G, \bmax)$; \\
\For{$j\in [\sizeofitems]$}  {
	Assign the top $b_j$ nodes of $\greedSeeds$ to item $i_j$, i.e.,  $\greedSeeds_j \leftarrow \mbox{ top } b_j \mbox{ nodes from } \greedSeeds$  \;
	$\greedAlloc \leftarrow \greedAlloc \cup (\{i_j\} \cdot \greedSeeds_j)$ \;}	
%
\textbf{return} $\greedAlloc$ as the final allocation\;  
%\end{small}
\end{algorithm}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Block Accounting} \label{sec:blocks} 

%\subsection{Uniform Budget Case} \label{sec:same_budget}

\eat{ 
In this section we assume that every item has the same budget, i.e., $b_i = k, \forall i \in [\sizeofitems]$, for some $k>0$. 
Thus the greedy allocation is simply $\greedAlloc = \greedSeeds \cdot \allitems$, where $\greedSeeds$ is the greedy seed node set of size $k$. 
} 
Recall the possible world model introduced in Section \ref{sec:possibleWorld}: 
in a possible world $W=(W^G,W^N)$, $W^N$ denotes a noise world where only the noise terms are sampled, and $W^G$ denotes an edge world where edges are sampled, and $W=(W^G,W^N)$ denotes a deterministic world where both noise terms and edges are sampled.

In the rest of the analysis, we fix the noise world $W^N$, and prove that
	$\sw_{\ow}(\greedAlloc) \geq (1 - \frac{1}{e} - \epsilon ) \cdot \sw_{\ow}(\optAlloc)$, where
	$\sw_{\ow}$ denotes the expected social welfare under the fixed noise world $\ow$.
We could then simply take another expectation over the distribution of $\ow$ to obtain
	the Inequality~\eqref{eq:approxsw} in our main theorem in Section~\ref{sec:overview}. %Theorem~\ref{thm:main}.
Let $\utilow$ be the utility function under the noise possible world $\ow$.
We first state the following simple result that $\utilow$ is supermodular. 

%%%%%%%%%%%%%%%%%% 
\eat{ 
\begin{lemma} \label{lem:utilowsupermod}
	Under the noise possible world $\ow$, $\utilow$ is supermodular.
\end{lemma}
\begin{proof}
We know that for any item set $A$,  $\utilow(A) = \val(A) - \price(A) + \noise(A) $.
Since $\val$ is supermodular, $\price$ is additive (i.e. modular) and this $-\price$ is
	also modular, and $\noise(A) = \sum_{i\in A} \noise(i)$
	is also modular, and $\noise(i)$ for all $i\in \allitems$ is fixed under $\ow$, so the summation of
	supermodular and modular functions is still supermodular.
Therefore, $\utilow$ is supermodular.
\end{proof}	
}
%%%%%%%%%%%%%%%%%% 

Given $W^N$, let $I_{\ow}^*$ be the subset of items that gives the largest utility across all subsets of $\allitems$ in $\ow$, with ties broken in favor of sets with larger cardinality. 
By Lemma~\ref{lem:itemunion}, $I_{\ow}^*$ must be unique.
This implies that the marginal utility of any subset of $\allitems \setminus I^*_{\ow}$ given $I_{\ow}^*$ is strictly
	negative.
By the supermodularity of the utility function $\utilow$ in the fixed noise world $\ow$ (Lemma~\ref{lem:utilowsupermod}), 
	it further follows that
	the marginal utility of any subset of $\allitems \setminus I^*_{\ow}$ given any subset of $I_{\ow}^*$ is strictly
	negative, which means no items in $\allitems \setminus I^*_{\ow}$ can ever be adopted by
	any user under the noise world $\ow$.
Thus, once we fix $\ow$, we can safely remove all items in $\allitems \setminus I^*_{\ow}$ from consideration.
For simplicity, we assume w.l.o.g. that $\allitems = I^*_{\ow}$ is the item set with the largest
utility for our analysis under a fixed $\ow$.\footnote{$\allitems$ may contain items not in $I^*_{\ow}$. Our assumption that $\allitems = I^*_{\ow}$ is only for analysis in a specific noise world $\ow$.}  

\eat{ 
Also notice that when budget is uniform, since there is only one budget, vanilla IM algorithms happen to be prefix preserving out-of-the box. } 

%%%%%%%%%%%%%%% BEGIN HUGE EAT 
\eat{  
We now discuss the block based accounting method for analyzing the social welfare. 
We divide items in $\allitems$ into a sequence of disjoint blocks such that each block has a non-negative marginal utility w.r.t. the union of all its preceding blocks.
 We next discuss how the blocks are generated. 

\subsubsection{Block generation process}\label{sec:block_acc}

Algorithm \ref{alg:blockset-ucomic} shows the pseudocode to generate the blocks from $\allitems$ for a given $\ow$. Note that this {\sl block generation process is solely used for our accounting analysis and 
	is not part of our allocation algorithm}. 

\eat{ 
\weic{I noticed that Algorithm \ref{alg:blockset-ucomic} had an issue, so revised it.
	The issue was that after finding a nonnegative block $B$, we should go back to the beginning of the 
	remaining sequence $\cal I$ to search again.	
}
} 

We first generate a global sequence $\cal I$ of all nonempty subsets of $\allitems$, starting
	from singletons, with increasing subset sizes.
For subsets with the same size, we can choose an arbitrary but the fixed order of these subsets.
Then, we scan through this sequence, with the purpose of generating a sequence of disjoint blocks $\allblocks$.
For each subset $B$ being scanned, if its marginal utility given all previously selected blocks is
	non-negative, i.e. $\utilow(B \mid \bigcup \allblocks) \geq 0$, where $\allblocks$ are currently selected
	sequence of blocks, and $\bigcup \allblocks$ is the union of all items in these selected blocks, 
	then we append $B$ to the end of selected sequence $\allblocks$, namely $\allblocks = \allblocks \oplus B$.
After selecting $B$, we remove all subsets in $\cal I$ that overlaps with $B$, and restart the scan from 
	the beginning of the remaining sequence.
If $\utilow(B \mid \bigcup \allblocks) < 0$, then we skip this block and go to the next one.
%	
%First singleton items are scanned, if any item has a non-negative utility then it
%	is selected as a block. If no such singleton item is found, then two item subsets are considered and so on. All subsets of smaller sizes are considered first before moving on to larger sizes. Subsets of same size can be ordered in any arbitrary but fixed order. 
%Once an item subset $B$ is selected as a block, every subset that intersects with $B$ in
%	sequence $\cal I$ is removed from consideration (lines $8$-$9$).

\weic{$\mathbf{B}$ represents a sequence of blocks, while $\mathcal{I}$ represents a sequence of all blocks,
	$\allitems$ represents set of all items.
	These notations are inconsistent in style, so I replace $\mathbf{B}$ with $\allblocks$, so that
	we use calligraphic capital letters to represent sequence of blocks.}

Let $B_1, B_2, \ldots, B_t$ be the sequence of blocks generated.
These blocks have the following properties.
We define the marginal gain of each block $B_i$ as
\begin{equation}
\Delta_i = \utilow(B_i \mid \cup_{j=1}^{i-1} B_j). \label{eq:Delta}
\end{equation}
We remark that the order of the blocks in $B_1, \ldots, B_t$ may not be the same as their corresponding
	subset orders in $\cal I$.
For example, the order of $\cal I$ for two items $a,b$ is $\{a\}, \{b\}, \{a,b\}$, but $\utilow(\{a\})<0$,
	$\utilow(\{b\}) > 0$, and $\utilow(\{a\} \mid \{b\}) > 0$, so the block order is $B_1 = \{b\}$ and
	$B_2 = \{a\}$.

\begin{property}\label{prop:block_disjoint}
	Blocks $B_1, B_2, \ldots, B_t$ forms a partition of $\allitems$, i.e. $B_i \cap B_j = \emptyset$ for
	all $1 \le i < j \le t$, and $\cup_{i\in [t]} B_i = \allitems$.
\end{property}
The disjointness of all blocks are clear from the construction. The fact that every item in $\allitems$ belongs
	to some block comes from our assumption that $\allitems$ has the maximum utility under $\ow$, because if
	$\allitems \setminus \cup_{i\in [t]} B_i$ is not empty, then this subset must have nonnegative marginal
	utility given $\cup_{i\in [t]} B_i$, so by the construction it will be appended to the block sequence.

\begin{property}\label{prop:block_utility}
For all $i\in [\numblocks]$, $\Delta_i \ge 0$ , and $\utilow(\allitems) = \sum_{i=1}^{\numblocks} \Delta_i$.
\end{property}

%\SetAlgoSkip{}
\begin{algorithm}[t!]
%\begin{small}
\DontPrintSemicolon
\caption{Generate Blocks($\allitems$, $\ow$)} \label{alg:blockset-ucomic}
%$B_0 \leftarrow \emptyset$ \;
%$\allblocks \leftarrow \{B_0\}$ \; 
Generate the $2^{|\allitems|} -1$ non-empty subsets of $\allitems$ \; 
Sort the subsets based on their sizes, and order subsets of the same size in an arbitrary fixed order. Put the sorted subsets in sequence $\mathcal{I}$ \; \label{line:I} 
$\allblocks \leftarrow \emptyset$; $B \leftarrow$ the first entry in $\mathcal{I}$\\ 
\While{\em $\mathcal{I}$ is not empty} {
	\If{$\utilow(B \mid \bigcup \allblocks) \geq 0$} {
	    $\allblocks \leftarrow \allblocks \oplus B$ // append $B$ at the end of sequence $\allblocks$ \;   
        remove all sets $B'$ from $\mathcal{I}$ with  $B' \cap B\ne \emptyset$ \;
      	$B \leftarrow$ the first entry in $\mathcal{I}$ \;
	}
	\Else{
		$B \leftarrow$ the next entry in $\mathcal{I}$ after $B$ \;
	}
}
\textbf{return} $\allblocks$ as the final sequence of blocks\;  
%\end{small}
\end{algorithm}

We now explain how these blocks are used in the accounting method to compute the social welfare of both greedy and any arbitrary allocation.

\subsubsection{Social welfare under greedy allocation}

In the uniform budget case where every item has budget $k$, 
	the $\algo$ algorithm (Algorithm \ref{alg:greedy_allocation}) allocates one copy of the full item set $\allitems$
	to each of the top $k$ nodes found by an influence maximization algorithm (note that in this case
	prefix-preserving is not needed since budgets are uniform).
Let $\greedSeeds \subseteq V$ be the top $k$ seeds found by the algorithm. 
Recall that $\sigma(S)$ denote the expected spread of seed set $S$ in the associated IC model.
Let $\greedAlloc = \greedSeeds \cdot \allitems$ be the greedy allocation. 
The following lemma shows that how the expected social welfare of the greedy allocation can be accounted for.
 
\begin{lemma}\label{lem:greedysw} 
The expected social welfare of $\greedAlloc$ in $\ow$, is $\sww(\greedAlloc) = \sigma(\greedSeeds) \cdot \utilow(\allitems)$.
%$ = \sum_{i\in [\numblocks]} \sigmaw(\greedSeeds_{B_i}) \cdot \Delta_i$, where $\greedSeeds_{B_i}$ are the seed nodes of block $B_i$ in allocation $\greedAlloc$, $\sigmaw(\greedSeeds_{B_i})$ is the expected spread of block $B_i$ in $\ow$ and $\Delta_i$ is as defined above. 
\end{lemma} 

\begin{proof} 
First, for every seed node $u\in \greedSeeds$, since $u$ is offered the full item set $\allitems$, and
	by our assumption $\allitems$ has the maximum utility under world $\ow$, $u$ would adopt the full
	set $\allitems$.
By Lemma \ref{lem:reachable}, for all nodes $v$ that $u$ could reach in the graph possible world $W^G$, 
	$v$ also adopts the full set $\allitems$.
Therefore, full set $\allitems$ always propagates together just like a single item, and the expected number of
	nodes adopting the full set $\allitems$ is exactly $\sigma(\greedSeeds)$, where the expectation is taken
	over the graph possible world $W^G$.
Since each node that adopts $\allitems$ contributes $\utilow(\allitems)$ to the social welfare, the
	expected social welfare is $\sww(\greedAlloc) = \sigma(\greedSeeds) \cdot \utilow(\allitems)$.
%	
%By construction, when any node is offered the itemset $\allitems$, it will adopt it, since among subsets of $\allitems$, the set $\allitems$ has the highest utility. 
%By supermodularity of utility, in $w$, a node $v$ adopts an itemset iff a seed node $u$ adopts that itemset and $v$ is reachable from $u$ (Lemma \ref{lem:reachable}). Thus the expected number of nodes that adopts $\allitems$ in $\ow$ is, $\sigmaw(\greedSeeds)$. From this, it follows that the expected social welfare of greedy allocation is $\sww(\greedAlloc) = \sigmaw(\greedSeeds) \cdot \utilow(\allitems)$. Now, $\utilow(\allitems) = \sum_{i\in [t]} \Delta_i$. Also, since blocks are pairwise disjoint, under greedy allocation $\sigmaw(\greedSeeds) = \sigmaw(\greedSeeds_{B_i})$, because all items are offered to every node in $\greedSeeds$.
\end{proof} 


\subsubsection{Utility under an arbitrary allocation}

We now analyze the social welfare for an arbitrary allocation $\allalloc$ under the noise possible world $\ow$.
Unlike the greedy allocation, 
	in an arbitrary allocation seed nodes may not necessarily be allocated the full item set $\allitems$, and
	the propagation behavior from the seeds could be more complicated.
Our idea is to use the blocks defined in Section~\ref{sec:block_acc} to partition any subset of items a node
	may become aware of, so that we can account for the social welfare of a node for each individual blocks.
The following is our technical treatment.

Let $A \subseteq \allitems$ be a subset of items. 
We partition $A$ using the blocks. Specifically we find partitions $A_i$'s such that, $A_i = A \cap B_i, \forall i \in [\numblocks]$. For a set $A_i$, if $A_i = B_i$, we call it a full block, if $A_i = \emptyset$, then it is an empty block, otherwise, we call it a partial block. 
Define $\Delta^A_i = \utilow(A_i \mid A_1 \cup \ldots \cup A_{i-1})$. 
It follows that $\utilow(A) = \sum_{i=1}^s \Delta^A_i$. 
From the above equation, we devise our accounting method such that each $A_i$ is accounted for $\Delta^A_i$ 
	in its social welfare contribution.
By supermodularity, 
We now show some important properties related to these blocks, especially partial blocks.

\begin{lemma} \label{lem:partialblock}
If $A_i$ is a partial block, then $\Delta^A_i < 0$.
\end{lemma}
\begin{proof}
If $\Delta^A_i \ge 0$, then by the supermodularity of $\utilow$ (Lemma~\ref{lem:utilowsupermod}), 
$\utilow(A_i \mid B_1 \cup \ldots \cup B_{i-1})) \ge \utilow(A_i \mid A_1 \cup \ldots \cup A_{i-1}) \ge 0
$.
Then in the block generation process (Algorithm~\ref{alg:blockset-ucomic}), set $A_i$ should be selected as
the $i$-th block instead of $B_i$, a contradiction.	
\end{proof}

The above lemma has the following immediate consequence, which is important in our analysis

\begin{lemma} \label{lem:marginalBound}
For any item set $A$, any block index $i$, $\Delta^A_i \le \Delta_i$.
\end{lemma}
\begin{proof}
By the definition of blocks, we know that $\Delta_i \ge 0$.
If $A_i$ is an empty block, then $\Delta^A_i = 0 \le \Delta_i$.
If $A_i$ is a partial block, then by Lemma~\ref{lem:partialblock}, $\Delta^A_i < 0 \le \Delta_i$.
If $A_i$ is a full block, then $A_i = B_i$.
We have $A_1 \cup \ldots \cup A_{i-1} \subseteq B_1 \cup \ldots B_{i-1}$, and by the supermodularity
	of $\utilow$ (Lemma~\ref{lem:utilowsupermod}), 
	$\Delta^A_i = \utilow(B_i \mid A_1 \cup \ldots \cup A_{i-1}) \le 
		\utilow(B_i \mid B_1 \cup \ldots \cup B_{i-1}) = \Delta_i$.
Therefore, the lemma holds.
\end{proof}

\eat{ %% The following part is related to the old padding technique, and is commented out
\weic{The following is used to be called a claim. But I don't see it necessary to separate claims from lemmas,
so unify it as a lemma.}

\begin{lemma}\label{lem:partial_adoption}
In any adoption set of any node, a partial block must be followed by a full block of higher index.
Technically, if $A$ is a set adopted by a node, and for some $i\in [t]$, $A_i$ is a partial block, then
	there must exists $j > i$ such that $A_j$ is a full block.
\end{lemma}
\begin{proof}

Suppose $A_s$ is the nonempty block with the highest index.  
Suppose, for a contradiction, that $A_s$ it is a partial block. 
Then from Lemma~\ref{lem:partialblock}, we know that $\Delta^A_s = \utilow(A_s \mid A_1 \cup \cdots A_{s-1})< 0$.
This means that $\utilow(A) < \utilow(A_1 \cup \cdots A_{s-1})$, but this contradicts to
	Lemma~\ref{lem:localmaximum2}, which says adopted set $A$ must be the local maximum.
\end{proof}

Lemma \ref{lem:partial_adoption} is true for any node, including the seed nodes. Hence a partial block cannot be adopted and consequently cannot propagate by itself unless it is followed by a full block. 
By Lemma~\ref{lem:partialblock}, a partial block $A_i$ only contribute negative marginal $\Delta^A_i$ to the social
	welfare, so when upper bounding the social welfare of an arbitrary seed allocation, we could ignore
	partial blocks like $A_i$.
However, we cannot completely ignore all partial blocks for their contribution to social welfare, because
	it is possible that via propagation several partial blocks merge at a node and becomes a full block, which
	provides positive marginal contribution to the social welfare.
This is illustrated by the following example.

\begin{example} \label{exp:merge}
Consider the network of Figure \ref{fig:blocks_fig}, and assume all edge probabilities to be $1$. 
Let there be three items $a,b,c$ in propagation with the following utilities $\utilow(a) = \utilow(b) =\utilow(c) = -1$, $\utilow(a,b) = \utilow(b,c) = \utilow(a,c) = 1$, $\utilow(a,b,c) =2$. Budget for all items $k=2$. Let the blocks be $B_1 = \{a,b\}$ and $B_2 = \{c\}$, thus $\Delta_1 = 1$ and $\Delta_2 =1$. Consider an allocation $\allalloc$ s.t., $\allalloc(a) = \{u,v\}$, $\allalloc(b) = \{u,w\}$ and $\allalloc(c) = \{v,w\}$. In this allocation both nodes $v$ and $w$ gets partial blocks $\{a\}$ and $\{b\}$ respectively. So at node $v$ and $w$ the partial blocks do not contribute
	 positively to the welfare. 
Thus the contribution of $v$ or $w$ towards welfare is only from full block $\{c\}$, $\Delta_2 =1$. But these partial blocks are followed by a full block $\{c\}$. Hence they get adopted and start propagating. Later at node $x$ the partial blocks merge to form the full block $\{a,b\}$ and starts contributing positively to the welfare at node
	$x$. In particular, node $x$ would adopt $\{a,b,c\}$ and block $\{a,b\}$ contributes $\Delta_1 = 1$ to
	the social welfare, where block $\{c\}$ contributes $\Delta_2 =1 $ to the welfare. 
\end{example}


\begin{figure}
\centering
\begin{small}
\includegraphics[width=.25\textwidth]{figs/eg.png}
\caption{An example network to illustrate the block propagation}
\label{fig:blocks_fig}
\end{small}
\end{figure}

To account for the propagation of partial blocks that can merge later to form full blocks and
	make positive contribution to social welfare, we introduce the following padding technique.

\spara{Padding technique}\label{sec:pad1}

The idea for the padding is to levy the contribution a partial block can potentially provide to social welfare. Notice that a partial block starts contributing to welfare only after becoming a full block. In other words it must contain all elements of the corresponding full block. 
Among all items in a block $B_i$, we call the item with the largest item index the {\em anchor item}.
Note that the choice of the anchor item for a block could follow other deterministic rules, and we simply use
	the item index for our convenience.
In our padding process, if a partial block at a seed node
	contains the anchor item of the corresponding full block $B_i$, 
	then we pad the partial block with the remaining items of $B_i$. 
Our padding thus converts only those partial blocks that contains the anchor item into the corresponding full block. 
After the padding, there is no longer the scenario of two partial blocks merge into a full block.
A partial block can only be merged with an already full block, and thus,
	we can then view the propagation only in terms of full blocks. 
Moreover, for each block $B_i$, the number of partial blocks that are padded can be at most $k$, because
	the anchor item of $B_i$ only has budget of $k$ and thus can only be allocated to $k$ seed nodes.
Finally, due to padding the contribution of the block to social welfare only increases because of
	the monotonicity of social welfare (Theorem~\ref{thm:monotoneSW}). 
We show that even the raised social welfare of an arbitrary allocation after padding is still within the desired bound. 
We next show an example of the padding process.

\begin{example}
Revisit the example of Figure \ref{fig:blocks_fig}. For the allocation $\allalloc$, the two partial blocks are $\{a\}$ and $\{b\}$ at nodes $v$ and $w$ respectively. 
For block $\{a,b\}$, $b$ is the anchor item.
Now the partial block of node $w$ contains the anchor item $b$. 
So we pad it with item $a$, to make it a full block, whereas partial block of node $v$ is not padded. Thus later when at node $x$ the partial blocks merge, we can still trace it back to a full block from a seed node which is $w$ in this case. Consequently we can view as if the propagation of full block $\{a,b\}$ started from seed node $w$ itself. 
\end{example}

After padding, for allocation $\allalloc$, we can view it as the propagation of full blocks $B_i$, whereas some of the full blocks are generated by padding. Each adoption of $B_i$ contributes
	at most $\Delta_i$ to the welfare (Lemma~\ref{lem:marginalBound}). 
Recall that $\Delta_i = \utilow(B_i \mid B_1 \cup ... \cup B_{i-1})$. 
We now need to formally argue that the merge of two partial blocks into a full block will not happen after the padding.
In other words, the full blocks can be viewed as always propagate from the seed nodes together.

\weic{
The following lemma is a new one.
I added it because it is needed to show that padding would indeed work, that is, after the padding at a seed node,
	the seed would always propagate the full block together.
However, I think the following lemma is not technically correct. 
That is, we cannot hope that after the padding, the full block $B_i$ would always be propagated together, if
	its anchor is adopted at the seed node.

In the following I will show such an example. 
But I believe we can still prove our main result without padding. 
So if you do not want to go through the rest of this note on the example, you can jump to the next note, 
	where I will explain how the proof still works without padding.

The following is an example that the seed node $u$ adopts a partial block with the anchor, but even after 
	we pad the partial block to a full block, $u$ would still adopt only the anchor, not the full block.
To construct such an example, we need at least one block $B_i$ with two items; we also need at least one block 
	in front of this block $B_i$, otherwise the full block would have nonnegative marginal and the proof would 
	go through.
We also need at lest one block behind $B_i$, otherwise $u$ would not adopt the anchor in the first place
	(by Lemma~\ref{lem:partialblock}).
So at the minimum, I need three blocks and four items. This is the counter example I constructed.

We have four items $\{a,b,c,d\}$, and we want to construct three blocks $\{a\}, \{b,c\}, \{d\}$.
Here are the utility functions I tried to satisfy all the requirements.
$\utilow(a) = 1; \utilow(b) = \utilow(c) = -2; \utilow(d) = -1;
\utilow(ab) = \utilow(ac) = \utilow(ad) = -1; \utilow(bc) = -3; \utilow(bd) = -2; \utilow(cd) = 2;
\utilow(abc) = 1; \utilow(abd) = 1; \utilow(acd) = 3; \utilow(bcd) = 1;
\utilow(abcd) = 5$.
By the block generation process, since $\utilow(a) = 1$, $\{a\}$ is the first block.
$\utilow(b | a) = \utilow(c | a) = \util(d | a) = -2 < 0$, so 
	we go to two-item sets, since $\util(bc\mid a) = 0$, 
the second block is $\{b,c\}$. Then the last block is $\{d\}$.
Note that $c$ is the anchor item for the block $\{b,c\}$.
One should verify that all marginals are correct for supermodularity.

For a seed node $u$, if we assign $c,d$ to $u$, then $u$ adopts $c, d$.
When we pad the second block with $b$, so now $u$ is assigned $b,c,d$, because $\utilow(bcd) = 1 < 2 = \utilow(cd)$,
	$u$ would still adopt $c,d$.
This means that padding may not make the seed node to adopt the full block even when the seed node still adopts
	the anchor item.

To make it a direct counter example for the following lemma, we also need to create a propagation so that
	some node $v$ adopts the full block $\{b,c\}$, but we cannot trace back $\{b,c\}$ to a seed node. 
Then we can use a graph with four nodes: $u, v, x, y$.
Node $u$ is above, assigned with $\{c,d\}$; node $x$ is another seed node assigned with $\{a, b, d\}$.
This looks like a nonuniform budget case, but we can certainly add another isolated node just to make the budget
	uniform if we want.
Now $x$ points to $v$ directly, and $u$ points to $y$ first, and then $y$ points to $v$.
By the above argument, $u$ adopts $\{c,d\}$, and then propagate to $y$ and $v$.
By the above utility function $x$ adopts $\{a,b,d\}$, and then propagate it to $v$.
Then at $v$, $v$ adopts all items $\{a,b,c,d\}$.
However, we cannot find a path $v$ to trace back to a seed set, because $x$ only adopts partial block $\{b\}$
	and $y$ only adopts partial block with $\{c\}$.
This is true even when we pad seed node $u$ with item $b$, but $u$ will still not adopt $b$.
}

\weic{
This is the note that will explain why we can still proceed without the padding.
The key observation is that, our intention for padding is to show that the full block will be propagated, so
	that we can properly account for their contribution.
However, it is not necessary that we really do the padding.
%What we really need to have is that when a node $v$ adopts a full block $B_i$, we can trace back its anchor item $a_i$;
%	that is, there is a path from some seed node $u$ to $v$, such that all nodes on the path adopts the anchor
%	item.
%For a single item, this is trivial and must be true.
%Then, we can argue that on this path, whether or not the anchor item $a_i$ is adopted together with its full 
%	block $B_i$, the marginal contribution of this partial or full block is at most $\Delta_i$
%	(by Lemma~\ref{lem:marginalBound}).
%
All we need to argue is that if some node $v$ adopts a full block $B_i$, then (a) the marginal
	contribution of this full block is at most $\Delta_i$, and (b) there must be a propagation path from 
	some seed node to this node $v$ such that
	all nodes on the path adopts the anchor $a_i$ of $B_i$.
(a) is true by Lemma~\ref{lem:marginalBound}.
(b) is true trivially, because when we look at a single item, there must be a propagation path for this
	single item from the seed.
	
Then, because of (b), it is enough to see that the expected number of nodes adopting the full block $B_i$ is
	at most $\sigma(S_{a_i})$, where $S_{a_i}$ is the seed nodes assigned the anchor $a_i$.
Then, together with (a), we know that the block $B_i$'s total contribution is at most
	$\sigma(S_{a_i}) \cdot \Delta_i$.
This is good enough to show our approximation because the budget of $a_i$ is $k$.
	
Note that we use the fact that if $v$ only adopts a partial block for $B_i$, then its marginal contribution is negative,
	so we do not count them, and thus it does not matter if those partial block adoptions cannot be traced back
	to some seed node with the anchor.
	
I believe the above argument also hold for the nonuniform case. There we only need to look at the anchor item
	again, and obtain the same bound $\sigma(S_{a_i}) \cdot \Delta_i$.
Then since the budget of $a_i$ is exactly the effective budget of block $B_i$, the rest would go through.

In a nutshell, we do not need the actual padding, since the diffusion of anchor item is already good enough to 
	limited the expected spread of a full block $B_i$.
}

\prith{
The counter example. Consider four items $a,b,c$ and $d$. Let the utilities be as follows in a noise possible world $W^N$.\\ $\utilow(a) = 1, \utilow(b) = -10, \utilow(c) = -5, \utilow(d) = -2$, \\$\utilow(a,b) = -9, \utilow(a,c) = -4, \utilow(a,d) = -1, \utilow(b,c) = -15, \utilow(b,d) = -12, \utilow(c,d) = 1$,\\ $\utilow(a,b,c) = 1, \utilow(a,b,d) = -11, \utilow(a,c,d) = 3 \utilow(b,c,d) = -6$, $\utilow(a,b,c,d) = 20$.

The blocks can therefore be, $B_1 = \{a\}, B_2=\{b,c\}$ and $B_3 = \{d\}$. Now consider a seed node $v$ where under some allocation, $\{c,d\}$ is allocated to $v$. $v$ will adopt $\{c,d\}$ as $\utilow(c,d) = 1 > 0$. If we convert the partial block $\{c\}$ to the corresponding full block $\{b,c\}$, then $v$ is allocated $\{b,c,d\}$. Even then $v$ ends up adopting $\{c,d\}$ and does not adopt the full block $\{b,c\}$.
}

\begin{lemma} \label{lem:atomicblocks}
During the propagation under a graph possible world $W^G$, if some node $v$ adopts
	a full block $B_i$, then there must be a path in $W^G$ from a seed node $u$ such that all nodes on the path
	(including the seed node $u$) adopts $B_i$.
\end{lemma}
\begin{proof}
Since $v$ adopts $B_i$, it must adopt the anchor item $a_i$ of $B_i$.
Then, there must be a path in $W^G$ from some seed node $u$ to $v$ such that all nodes on the path adopts $a_i$.
Since $a_i$ is assigned to the seed node $u$, then by our padding process the full block $B_i$ must be also padded
	at $u$, that is, $u$ is assigned the full block $B_i$ after the padding.
We now claim that $u$ must have adopted the full block $B_i$.
In fact, suppose, for a contradiction, that $u$ adopts an item set $A$ and $B_i \not \subseteq A$.
Let $A_i = A \cap B_i$ as defined before.
Then we have $\utilow(A) = \sum_{i\in [t]} \Delta^A_i$.
Let $A' = A \cup B_i$, and we also have $\util(A') = \sum_{i\in [t]} \Delta^{A'}_i$.
For all $j < i$, it is clear that $\Delta^A_j = \Delta^{A'}_j$.
For all $j > i$, we can see that, by supermodularity of $\utilow$ (Lemma~\ref{lem:utilowsupermod}),
	$\Delta^A_j \le \Delta^{A'}_j$.
\weic{However, I cannot show that for block $B_i$,  $\Delta^A_i \le \Delta^{A'}_i$.
If I could show this, then node $v$ should always adopt the set with larger utility, and tie-breaking with 
	the larger set, so $v$ would adopt $A'$, a contradiction.
Then if the seed node $u$ adopts the full block $B_i$, by reachability, all nodes on the path would adopt 
	the full block $B_i$.
}
\end{proof}
	
The remaining partial blocks only give negative contribution to the social welfare. Even after they merge with other partial blocks, cannot form any new full block. Consequently their contribution to social welfare are not counted. 
This above argument applies to all nodes including the seed nodes.
Therefore, for allocation $\allalloc$ we have the following lemma.  

} %% end of the commented part about the padding technique

The above two lemmas are crucial for our accounting method. 
To make our analysis closer to the later analysis for the nonuniform budget case, we do the accounting based on
	the presence of anchors of a block.
For a block $B_i$, the anchor $a_i$ of $B_i$ is the highest indexed item in $B_i$, where item indices in the uniform
	budget case can any total ordered indices.
Then we have the following lemma.

\begin{lemma}\label{lem:allsw}
For any arbitrary seed allocation $\allalloc$, 
	the expected social welfare in world $\ow$ is upper bounded as follows:
	$\sww(\allalloc) \leq \sum_{i\in [\numblocks]} \sigma(\allseeds_{a_i}) \cdot \Delta_i$, where $\allseeds_{a_i}$ are the seed nodes to which item $a_i$ is assigned in allocation $\allalloc$, and $\Delta_i$ is as defined 
	in Eq.~\eqref{eq:Delta}. 
\end{lemma}

\begin{proof}
For a graph possible world $W^G$, 
	suppose that after the diffusion process under $W^G$, every node $v$ adopts item set $A_v$.
Let $A_{v,i} = A_v \cap B_i$ for all $i \in [t]$, and
	$\Delta^{A_v}_i = \utilow(A_{v,i} \mid A_{v,1} \cup \ldots \cup A_{v,i-1})$.
Thus, we have 
\begin{align}
\sww(\allalloc) & = \E_{W^G} \left[\sum_{v\in V} \utilow(A_v) \right] 
	= \E_{W^G} \left[\sum_{v\in V} \sum_{i\in [t]} \Delta^{A_v}_i \right]  \nonumber \\
  &	= \sum_{i\in [t]} \E_{W^G} \left[ \sum_{v\in V} \Delta^{A_v}_i \right], \label{eq:welfareEquiv}
\end{align}
where the expectation is taken over the randomness of the graph possible worlds, and thus we use
	subscript $W^G$ under the expectation sign to make it explicit.
By switching the summation signs and the expectation sign in the last equality above, 
	we show that the expected social welfare can be
	accounted as the summation among all blocks $B_i$  of the expected marginal gain of block $B_i$ on all nodes.
We next bound $\E_{W^G} \left[\sum_{v\in V} \Delta^{A_v}_i \right]$ for each block $B_i$.

Under the graph possible world $W^G$, for each $v\in V$, there are three possible cases for $A_{v,i}$.
In the first case, $A_{v,i} = \emptyset$. In this case, $\Delta^{A_v}_i = 0$, so we do not need to count 
	the marginal gain $\Delta^{A_v}_i$.
In the second case, $A_{v,i}$ is not empty but 
	does not contain the anchor $a_i$, i.e. $a_i \not\in A_{v,i}$, and $A_{v,i} \ne \emptyset$.
In this case, $A_{v,i}$ is a partial block.
Then by Lemma~\ref{lem:partialblock}, $\Delta^{A_v}_i < 0$, which implies that we do not need to count 
	the marginal gain of $\Delta^{A_v}_i$ in this case too.
In the third case, $A_{v,i}$ contains its anchor $a_i$.
Under this case, by Lemma~\ref{lem:marginalBound}, $\Delta^{A_v}_i \le \Delta_i$, and so we relax
	$\Delta^{A_v}_i$ to $\Delta_i$.
This relaxation would occur only on nodes $v$ that adopts $a_i$.
By the EPIC model, for an individual item $a_i$, $v$ could adopt $a_i$ only when there is path in $W^G$ 
	from a seed node that adopts $a_i$ to node $v$. 
As defined in the lemma, $S_{a_i}$ is the set of seed nodes that are assigned $a_i$.
Let $\Gamma(S_{a_i}, W^G)$ be the set of nodes that are reachable from $S_{a_i}$ in $W^G$.
Then, there are at most $| \Gamma(S_{a_i}, W^G)|$ nodes at which we relax  $\Delta^{A_v}_i$ to $\Delta_i$ 
	for block $B_i$.
This means that 
\begin{align} \label{eq:marginalRelax}
\sum_{v\in V} \Delta^{A_v}_i \le | \Gamma(S_{a_i}, W^G)| \cdot \Delta_i.
\end{align}
Furthermore, notice that $\E_{W^G}[| \Gamma(S_{a_i}, W^G)| ] = \sigma(S_{a_i})$, by the live-edge representation of
	the IC model.
Therefore, together with Eq.~\eqref{eq:welfareEquiv} and~\eqref{eq:marginalRelax}, we have
\begin{align*}
\sww(\allalloc) & \le \sum_{i\in [t]} \E_{W^G} \left[  | \Gamma(S_{a_i}, W^G)| \cdot \Delta_i \right] \\
 & =  \sum_{i\in [t]} \sigma(S_{a_i}) \cdot \Delta_i.
\end{align*}
This concludes the proof of the lemma.
%	
%As discussed, after padding the propagation can be viewed only in terms of full blocks. For any node that adopts the full block contributes at most $\Delta_i$ to the social welfare
%	(by the supermodularity of $\utilow$, Lemma~\ref{lem:utilowsupermod}). The expected number of nodes that adopts a full block $B_i$ is $\sigmaw(\allseeds_{B_i})$. Thus we can rewrite the social welfare as, 
%$$\sww(\allalloc) \leq \sum_{i\in [\numblocks]} \sigmaw(\allseeds_{B_i}) \cdot \Delta_i. $$
\end{proof}

A direct consequence of the Lemmas \ref{lem:greedysw} and \ref{lem:allsw} is the following result,
	corresponding to the correctness part of Theorem~\ref{thm:main}.

\begin{lemma} {\sc (Correctness of $\algo$ under the Uniform Badget Case)\ \ }\label{lem:uniformbudget}
Let $\greedAlloc$ be the greedy allocation and $\allalloc$ be any arbitrary allocation. 
When the item budgets are uniform, 
	given $\epsilon$ and $\ell$, the expected social welfare $\sw(\greedAlloc) \geq (1 - \frac{1}{e} - \epsilon ) \cdot \sw(\allalloc)$ with at least $1 - \frac{1}{|V|^{\ell}}$ probability.
\end{lemma}

\begin{proof}
From Lemma \ref{lem:greedysw}, we have for a possible world $\ow = (W^G, W^N)$,
$\sww(\greedAlloc) =\sum_{i\in [\numblocks]} \sigma(\greedSeeds) \cdot \Delta_i $,
	where $|\greedSeeds| = k$. 

For an arbitrary allocation $\allalloc$, we know that $|\allseeds_{a_i}| \leq k$. 
%In the greedy allocation we again know that $|\greedSeeds_{B_i}| = k$. 
By the correctness of the influence maximization algorithm we use in line~\ref{alg:PRIMM} 
	(Definition~\ref{def:PRIMM}, e.g. the IMM algorithm \cite{tang15}), we have that 
	with probability at least $1 - \frac{1}{|V|^{\ell}}$, 
	$\sigma(\greedSeeds) \geq (1 - \frac{1}{e} - \epsilon) \sigma(\allseeds_{a_i})$, for all blocks $B_i$'s
	and their corresponding anchors $a_i$'s.
	
Let the distribution of world $\ow$ be $\dow$. Then we have that 
	with probability at least $1 - \frac{1}{|V|^{\ell}}$,
\begin{align*}
\sw(\greedAlloc) &= \mathbb{E}_{\ow \sim \dow} [\sww(\greedAlloc)] \\
&= \mathbb{E}_{\ow \sim \dow} \left[\sum_{i\in [\numblocks]} \sigma(\greedSeeds) \cdot \Delta_i \right]\\
&\geq \mathbb{E}_{\ow \sim \dow} \left[\sum_{i\in [\numblocks]}(1 - \frac{1}{e} - \epsilon) \sigma(\allseeds_{a_i}) \cdot \Delta_i \right]\\
& \geq (1 - \frac{1}{e} - \epsilon) \mathbb{E}_{\ow \sim \dow} [ \sww(\allalloc)]  \\
& = (1 - \frac{1}{e} - \epsilon) \sw(\allalloc).
\end{align*}
Therefore, the theorem holds.
\end{proof}

} 
%%%%%%%%%%%%%%%%%%%%%% END HUGE EAT 

%\subsection{Nonuniform Budget Case} \label{sec:nonuniformBudget}

\eat{ 
We now extend the block-based accounting for non uniform budget and show that our greedy allocation $\algo$ preserves the approximation ratio even in this case. 

We now discuss the block based accounting method for analyzing the social welfare. 
We divide items in $\allitems$ into a sequence of disjoint blocks such that each block has a non-negative marginal utility w.r.t. the union of all its preceding blocks.
 We next discuss how the blocks are generated. 

Let $\allitems = \{i_1, ..., i_s\}$. We order the items in non-increasing order of their budgets, i.e., assume that $b_1 \geq b_2 \geq \cdots \ge b_s$, with ties on budgets broken in an arbitrary but fixed manner. As discussed in the beginning of Section~\ref{sec:blocks}, we assume w.l.o.g. that 
% 
%where $t=|\allitems|$, and same as discussed at the beginning of Section~\ref{sec:same_budget}, we assume that 
% 
$\allitems$ has the largest utility among all subsets of $\allitems$ under the fixed noise world $\ow$. 
} 
\eat{ 
Recall that for the nonuniform budget case, 
	our algorithm $\algo$ is prefix preserving, and it selects $\bmax = b_1$ nodes in an order and 
	then allocates the top $b_i$ nodes as seeds for item $i \in \allitems$.
}  

%\subsubsection{Problem with existing block generation approach} \label{sec:issue}
\subsubsection{Block generation process} \label{sec:rbg}

%%%%%%%%%%%%%%%%%%%%%%% 
\eat{ 
Similar to the uniform budget case, we still fix the noise possible world $\ow$, and then apply the block-based
	accounting method to analyze the social welfare.
However, the block generation process of section \ref{sec:same_budget} does not directly
	work with the nonuniform budget, as shown
	in the following example. 

\weic{The follow example is not cleanly explained, and I have no idea what it is supposed to do.
The items and node ids are changed, and also if the two nodes have no edges, why there is the order of two nodes.
Please clarify.}

\begin{example}\label{exm:block_counter}

Consider a network with two nodes $u$ and $v$ with no edges, an item universe with two items $\allitems = \{a,b\}$, budget vector $\bvec =(2,1)$. Assume a world $\ow$ with following utilities, $\utilow(a) = \utilow(b) = 1$ and $\utilow(a,b) = 5$. Let the top two nodes be $v_1$ and $v_2$. Then, the greedy allocation assigns $(i_1,i_2)$ to $v_1$ and only $i_1$ to $v_2$. Since the individual utilities are positives, $v_2$ adopts $i_1$. Also since $i_1$ is a full block, as per our accounting we charge $\Delta_2$ towards welfare for this adoption. Note that $\Delta_2 = i_1 \mid i_2 \geq i_1 \mid \emptyset$. Hence we end up over estimating the social welfare of greedy allocation. 
\end{example}

To address this issue we revise our block generation process as follows. 
The basic idea is that in the block generation process we want to enforce an order based on budgets so that the items having higher budgets are considered as block candidates before the items with lower budget. 
The only change to the block generation process (Algorithm \ref{alg:blockset-ucomic}) is at line \ref{line:I},
	where we generate the sequence of subsets $\mathcal{I}$. 
The rest of the algorithm remains exactly the same.
} 
%%%%%%%%%%%%%%%%%%%%%%% 

%%%%% 
We now discuss the block based accounting method for analyzing the social welfare. 
We divide items in $\allitems$ into a sequence of disjoint blocks such that each block has a non-negative marginal utility w.r.t. the union of all its preceding blocks.
 We next discuss how the blocks are generated. 

Let $\allitems = \{i_1, ..., i_s\}$. We order the items in non-increasing order of their budgets, i.e., assume that $b_1 \geq b_2 \geq \cdots \ge b_s$, with ties on budgets broken in an arbitrary but fixed manner. As discussed in Section~\ref{sec:blocks}, we assume w.l.o.g. that $\allitems$ has the largest utility among all subsets of $\allitems$ under the fixed noise world $\ow$. 
Algorithm \ref{alg:blockset-ucomic} shows the pseudocode to generate the blocks from $\allitems$ for a given $\ow$. Note that this {\sl block generation process is solely used for our accounting analysis and 
	is not part of our allocation algorithm}. 

We first generate a global sequence $\cal I$ of all nonempty subsets of $\allitems$, following a specific enumeration order, defined as follows. 
For any two distinct subsets $S, S' \subseteq \allitems$, we use the following precedence order $\prec$ to place them in the sequence $\mathcal{I}$. 
% 
\begin{enumerate}
\item Arrange the sets $S, S'$ in decreasing order of item indices. Compare items in $S, S'$, starting from the highest indexed items of $S$ and $S'$.
 If they match then compare the second highest indexed items and so on until one of $S$ or $S'$ exhausts. If one of the sets, say $S$ exhausts first, then $S \prec S'$. 
\item If the current pair of items in $S$ and $S'$ do not match, then $S \prec S'$, if the current item of $S$ has a lower index than the current item of $S'$. 
\end{enumerate}

As an example if we have three items $\allitems = \{i_1, i_2, i_3\}$ in the universe with $b_1 \geq b_2 \geq b_3$, then we order the subsets in the following order: $\{i_1\}, \{i_2\}, \{i_1, i_2\}, \{i_3\}, \{i_1, i_3\}, \{i_2, i_3\}, \{i_1, i_2, i_3\}$. Between subsets $\{i_3\}$ and $\{i_1,i_3\}$, $\{i_3\}$ is inserted first 
	according to rule $1$, 
	whereas between $\{i_1,i_2\}$ and $\{i_3\}$, $\{i_1,i_2\}$ is ordered first according to rule $2$.

It is straightforward to see that this defines a total order on subsets of $\allitems$ and thus the sequence $\mathcal{I}$ is well defined. 
% 
% 
Then, we scan through this sequence, with the purpose of generating a sequence of disjoint blocks $\allblocks$.
For each subset $B$ being scanned, if its marginal utility given all previously selected blocks is
	non-negative, i.e. $\utilow(B \mid \bigcup \allblocks) \geq 0$, where $\allblocks$ are currently selected
	sequence of blocks, and $\bigcup \allblocks$ is the union of all items in these selected blocks, 
	then we append $B$ to the end of selected sequence $\allblocks$, namely $\allblocks = \allblocks \oplus B$, where $\oplus$ denotes ``append''. 
After selecting $B$, we remove all subsets in $\cal I$ that overlap with $B$, and restart the scan from the beginning of the remaining sequence.
If $\utilow(B \mid \bigcup \allblocks) < 0$, then we skip this set and go to the next one.

Let $B_1, B_2, \ldots, B_t$ be the sequence of blocks generated.
These blocks satisfy the following properties.
We define the marginal gain of each block $B_i$ as
\begin{equation}
\Delta_i = \utilow(B_i \mid \cup_{j=1}^{i-1} B_j). \label{eq:Delta}
\end{equation}

\eat{ 
We remark that the order of the blocks in $B_1, \ldots, B_t$ may not be the same as their corresponding
	subset orders in $\cal I$.
For example, the order of $\cal I$ for two items $a,b$ is $\{a\}, \{b\}, \{a,b\}$, but $\utilow(\{a\})<0$,
	$\utilow(\{b\}) > 0$, and $\utilow(\{a\} \mid \{b\}) > 0$, so the block order is $B_1 = \{b\}$ and
	$B_2 = \{a\}$.
} 

\begin{property}\label{prop:block_disjoint}
	Blocks $B_1, B_2, \ldots, B_t$ forms a partition of $\allitems$, i.e. $B_i \cap B_j = \emptyset$ for
	all $1 \le i < j \le t$, and $\cup_{i\in [t]} B_i = \allitems$.
\end{property}
The disjointness of blocks is clear from the construction. The fact that every item in $\allitems$ belongs
	to some block comes from our assumption that $\allitems$ has the maximum utility under $\ow$, because if
	$\allitems \setminus \cup_{i\in [t]} B_i$ is not empty, then this subset must have non-negative marginal
	utility given $\cup_{i\in [t]} B_i$, so by the construction it will be appended to the block sequence.

\begin{property}\label{prop:block_utility}
For all $i\in [\numblocks]$, $\Delta_i \ge 0$ , and $\utilow(\allitems) = \sum_{i=1}^{\numblocks} \Delta_i$.
\end{property}

%\SetAlgoSkip{}
\begin{algorithm}[t!]
%\begin{small}
\DontPrintSemicolon
\caption{Generate Blocks($\allitems$, $\ow$)} \label{alg:blockset-ucomic}
%$B_0 \leftarrow \emptyset$ \;
%$\allblocks \leftarrow \{B_0\}$ \; 
Generate the $2^{|\allitems|} -1$ non-empty subsets of $\allitems$ \; 
Sort the subsets based on their sizes, and order subsets of the same size in an arbitrary fixed order. Put the sorted subsets in sequence $\mathcal{I}$ \; \label{line:I} 
$\allblocks \leftarrow \emptyset$; $B \leftarrow$ the first entry in $\mathcal{I}$\\ 
\While{\em $\mathcal{I}$ is not empty} {
	\If{$\utilow(B \mid \bigcup \allblocks) \geq 0$} {
	    $\allblocks \leftarrow \allblocks \oplus B$ // append $B$ at the end of sequence $\allblocks$ \;   
        remove all sets $B'$ from $\mathcal{I}$ with  $B' \cap B\ne \emptyset$ \;
      	$B \leftarrow$ the first entry in $\mathcal{I}$ \;
	}
	\Else{
		$B \leftarrow$ the next entry in $\mathcal{I}$ after $B$ \;
	}
}
\textbf{return} $\allblocks$ as the final sequence of blocks\;  
%\end{small}
\end{algorithm}

%%%%%%%%%%%%%%%% 
\eat{ 
We now explain how these blocks are used in the accounting method to compute the social welfare of both greedy and any arbitrary allocation.
%%%%%

 
Recall that in our item set $\allitems$, items are indexed in non-increasing order of budgets.
Thus an item with a lower index has budget more than or equal to other items having higher indices. 
Between any two subsets of $\allitems$, we use the following rule to order them into the sequence $\mathcal{I}$.
\begin{enumerate}
\item Starting from the highest indexed item of the subsets, the index of the two items are compared.
 If they match then the second highest indices are compared  and so on until one of the subsets exhausts. 
 The subset that exhausts precedes the other subset in the order.
\item If they do not match then the subset having lower indexed item precedes the other subset in the order. 
\end{enumerate}

As an example if we have three items $\allitems = \{i_1, i_2, i_3\}$ in the universe with $b_1 \geq b_2 \geq b_3$, then we order the subsets in the following order: $\{i_1\}, \{i_2\}, \{i_1, i_2\}, \{i_3\}, \{i_1, i_3\}, \{i_2, i_3\}, \{i_1, i_2, i_3\}$. Between subsets $\{i_3\}$ and $\{i_1,i_3\}$, $\{i_3\}$ is inserted first 
	according to rule $1$, 
	whereas between $\{i_1,i_2\}$ and $\{i_3\}$, $\{i_1,i_2\}$ is ordered first according to rule $2$.

Note that, the sequence of item subsets in $\mathcal{I}$ has the following property: 
} 
%%%%%%%%%%%%%%%%% 

\begin{property} \label{prop:subset}
For any subset $S$ in the sequence $\mathcal{I}$, for any $T$ that is a proper subset of $S$, $T$ appears before $S$ in $\mathcal{I}$.
\end{property}

Now when a subset of items is chosen as the $i$-th block $B_i$, we know that $\utilow(B_i\mid B_1 \cup ... \cup B_{i-1})\geq 0$. Consider a proper subset $S$ of $B_i$. Notice that since blocks are disjoint, $ S \not\subseteq B_1 \cup ... \cup B_{i-1}$. 
As per Property \ref{prop:subset}, we also know that $S$ appears before $B_i$ in $\mathcal{I}$. Thus we can conclude $\utilw(S \mid B_1 \cup ...\cup B_{i-1})< 0$, otherwise $S$ would have been chosen as the $i$-th block instead of $B_i$. Hence partial blocks still produce negative marginal utility, which means Lemma~\ref{lem:partialblock} 
	still holds for the nonuniform budget case.


\subsubsection{Social welfare under greedy allocation}

We are now ready to analyze the social welfare of our greedy allocation (Algorithm \ref{alg:greedy_allocation}) using the accounting method under the new block partition. 
One key difference from the uniform budget is that, when budget is non uniform, even in greedy allocation we can have partial blocks allocated to seed nodes as the budget constraint can prevent allocation of full blocks to seeds. However we prove the following important result related to the seed nodes.

\begin{lemma}\label{lem:full_prefix}
In the greedy allocation, if $A_i$ is the first partial block assigned to a greedy seed node $v \in \greedSeeds$, 
	then at time step $1$ when propagation through edges has not yet started, $v$ can only
	adopt the set of full blocks $B_1 \cup ... \cup B_{i-1}$. 
That is, $\adoptw^{\greedAlloc}(v,1) = B_1 \cup ... \cup B_{i-1}$ for any possible world that is consistent with
	$\ow$.
\end{lemma}

\begin{proof}
Let $A_t$ be the highest indexed block assigned to $v$. We know that blocks $A_1,..., A_{i-1}$ are all full blocks, whereas if $t>i$, then $A_{i+1}, ..., A_t$ can be full or partial. We show that $v$ does not adopt any item from the set $A_i \cup ... \cup A_t$, when $A_i$ is a partial block.

Suppose this is not true. Let $M \subseteq A_i \cup ... \cup A_t$ be an item set that $v$ adopts. Then we know that $\utilw(M \mid A_1 \cup ... \cup A_{i-1})\geq 0$. Since all blocks from $A_1$ to $A_{i-1}$ are full blocks, we can rewrite it as $\utilw(M \mid B_1 \cup ... \cup B_{i-1})\geq 0$.
We can derive that $M$ must contain at least one item from the set $A_{i+1} \cup ... \cup A_t$, 
	otherwise, all items are only from $A_i$, then $M$ turns out to be a partial block having nonnegative marginal utility, contradicting to the nonuniform budget version of Lemma~\ref{lem:partialblock} . 



Let $B_i$ be the full block corresponding to the partial block $A_i$. 
We know that $M$ appears in the sequence $\mathcal{I}$, and $M$ cannot be $B_i$.
if $M$ appears before $B_i$ in $\mathcal{I}$, then as per our block construction process $M$ should be chosen as the $i$-th block, since $\utilw(M \mid B_1 \cup ... \cup B_{i-1})\geq 0$. This contradicts with the fact that $B_i$ is the $i$-th block.

If $M$ appears after $B_i$ in $\mathcal{I}$, then at least one item of $M$ has index at least as high
	as the highest indexed item in $B_i$. 
Let this item of $M$ be $i_0$ and its budget be $b_{i_0}$. 
We know from the correspondence of index and budget that all items of $B_i$ has budget at least $b_{i_0}$. 
Since $i_0$ is assigned to $v$, we know that $v$ is part of top $b_{i_0}$ greedy nodes. 
As all items of $B_i$ have budgets at least $b_{i_0}$, they should also be assigned to $v$, in the greedy allocation. 
Thus $B_i$ as a full block is assigned to $v$. This leads to a contradiction that $A_i$ is a partial block in 
	the greedy allocation.
Therefore the lemma holds.
\end{proof}


For a block $B_i$, we define its {\em proposed budget} $\bbud_i$ to be the minimum
	budget among its items, i.e. $\bbud_i = min_{j \in B_j} b_j $. 
Under the greedy allocation, 
	the proposed budget of $B_i$ is the same as the maximum number of seed nodes
	to which the full block $B_i$ is offered.
However some seed nodes may not adopt the block. From Lemma \ref{lem:full_prefix} we know a full block $B_i$ is not adopted by a seed node $v$ even after being assigned to, if and only if at least one of the blocks from $B_1, ..., B_{i-1}$ is not assigned to $v$. 
This could happen when some blocks in $B_1, ..., B_{i-1}$ actually appears after $B_i$ in the original
	sequence $\cal I$, so that they have a smaller budget than the proposed budget of $B_i$, namely $\bbud_i$.
To address this issue, we further define the {\em effective budget} of a block $B_i$, 
	$\bbude_i $, to be the minimum proposed budget among all blocks 
	$B_1, B_2, \ldots, B_i$, i.e. $\bbude_i = min_{j \in B_1 \cup ... \cup B_i} b_i$. 
Under the greedy allocation, the effective budget of $B_i$ corresponds to 
	the number of seed nodes that actually adopt the full block $B_i$ 
	after the seed assignment and without considering the effect of propagation. 
We use the notation $\greedSeeds_{B_i}$ to denote all the seed nodes that are assigned the full block $B_i$ and 
	$\greedESeeds_{B_i}$ to denote all the seed nodes that actually adopt $B_i$ at step $1$ without
	considering propagation under the greedy allocation, 
	and we call them the effective greedy seeds of $B_i$. 
%	$\greedESeeds_{B_i} \subseteq \greedSeeds_{B_i}$, where for every $v \in \greedESeeds_{B_i}$, $v$ adopts $B_i$. Whereas for every $v \in \greedSeeds_{B_i} \setminus \greedESeeds_{B_i}$, $v$ does not adopt $B_i$.  

We remark that the definitions of proposed budget and effective budget of a block is purely
	based on the block sequence $B_1, B_2, \ldots, B_t$, and they are also the key concepts
	to be used in the analysis of the social welfare of arbitrary allocations in the next
	section.
With these definitions, we are now ready to prove the following lemma for the social welfare of greedy allocation.

\begin{lemma}\label{lem:greedyasw} 
Let $\greedAlloc$ be the greedy allocation obtained using Algorithm \ref{alg:greedy_allocation}. Then the expected social welfare of $\greedAlloc$ in $\ow$ is $\sww(\greedAlloc) = \sum_{i\in [t]} \sigma(\greedESeeds_{B_i}) \cdot \Delta_i$, where $\greedESeeds_{B_i}$ are the effective seed nodes of block $B_i$ in allocation $\greedAlloc$ and $\Delta_i$ is as defined in Eq.~\eqref{eq:Delta}. 
\end{lemma} 

\begin{proof} 

By Lemma~\ref{lem:full_prefix}, in an effective seed node of block $B_i$, block $B_i$ is offered with all previous blocks $B_1,...,B_{i-1}$. Thus the seed node always adopts $B_i$ (together with $B_1, \ldots, B_{i-1}$). 
Moreover, by definition, no other seed nodes outside the set of effective seeds adopts $B_i$ or
	any other blocks $B_{i+1}, \ldots, B_t$.
In other words, seed nodes only adopt full blocks and there are no partial blocks adopted at any seed node.
Then by Lemma~\ref{lem:reachable}, we know that each adopted full block at the seed is propagated together.
In particular,  blocks $B_1, \ldots, B_t$ always propagate together, and there is no other way for a node
	to adopt block $B_t$.
Thus the expected number of nodes that are reached by block $B_i$ and consequently adopt $B_i$, is $\sigma(\greedESeeds_{B_i})$. 
Moreover, each adoption of $B_i$ by any node contributes exactly $\Delta_i$ to the social welfare
	because all $B_1,...,B_{i-1}$ must also be present.
Then we have $\sww(\greedAlloc) = \sum_{i\in [t]} \sigma(\greedESeeds_{B_i}) \cdot \Delta_i$.
\end{proof} 

\subsubsection{Social welfare under an arbitrary allocation}

We first categorize blocks into two types namely \em{over budgeted} and \em{properly budgeted}, based on their proposed and effective budgets.
A block $B_i$ is an over budgeted block, if its effective budget is strictly less than its proposed budget, i.e., $\bbude_i < \bbud_i$. Otherwise, if $\bbude_i = \bbud_i$, the block is said to be properly budgeted. 

For every block we define its corresponding \em{anchor block} and \em{anchor item}. 
Anchor block $B^a_i$, of an over budgeted block $B_i$ is the block from $B_1, ..., B_{i-1}$, that has minimum proposed budget. In case of a tie, the block having highest index is chosen as the anchor block. 
Anchor item $a_i$, for an over budgeted block $B_i$, is the highest indexed item in its corresponding anchor block $B^a_i$. 
On the other hand, for a properly budgeted block, the block itself is its anchor block, because if the block is properly budgeted then the block itself has the minimum budget among all its previous blocks. 
The anchor item is the highest indexed item of the block.
Notice that, by definition, if block $B_j$ is the anchor block of block $B_i$ with $j< i$, then
	block $B_j$ is also the anchor block for all blocks $B_j, B_{j+1}, \ldots, B_i$.
In particular, $B_j$ itself must be a properly budgeted block.
Moreover, the effective budget of block $B_i$ is the proposed budget of its anchor block.

\weic{The old version of the following lemma is problematic, and I revised it to be close to what I originally 
	wrote in the note, and commented out the old version.}
\begin{lemma}\label{lem:anchor}
Let $B_i$ be an over-budgeted block, $B_j$ ($j< i$) be the anchor block of $B_i$, 
	and $a_i$ be the anchor item of $B_i$ in $B_j$.
During the diffusion process from the seed allocation $\allalloc$, 
	let $A$ be the set of items in $B_{j} \cup \ldots \cup B_i$
	that has been adopted by $v$ by time $t$.
If $v$ has not yet adopted the anchor item $a_i$ by time $t$ and $A \ne \emptyset$, then 
	$\utilow(A \mid B_1 \ldots, B_{j-1}) < 0$.
%During the diffusion corresponding to allocation $\allalloc$, if a node $v$ adopts full block $B_i$ at time $t$, unless it already adopted the corresponding anchor item $a_i$ by time $t$, the marginal contribution $B_i$ 
%given the set of adopted items in $B_1, \ldots, B_{i-1}$ is negative.
\end{lemma}
\begin{proof}
Suppose, for a contradiction, that $\utilow(A \mid B_1 \ldots, B_{j-1}) \ge 0$.
By the definition of the anchor item, we know that all items in $A \setminus B_j $ has strictly larger budget than the budget
	of $a_i$, otherwise one of items in $A$ should be the anchor for $B_i$.
This means all items in $A \setminus B_j $ has index strictly lower than $a_i$.
By definition $a_i$ is not in $A$, and thus all items in $A \cap B_j$ also have index strictly lower than $a_i$.
Then by the block generation process, $A$ should appear before $B_j$ in sequence $\cal I$.
Since $\utilow(A \mid B_1 \ldots, B_{j-1}) \ge 0$, the block generation process should select $A$ as the
	$j$-th block instead of the current $B_j$, a contradiction.
%
%Now for an over budgeted block, suppose that the Lemma is not true. 
%That is, node $v$ has not adopted $a_i$ by time $t$. Instead it adopts an item set $A \supseteq B_i$ at time $t$, where $A \setminus B_i$ (possibly empty) contains some elements from $B^a_i, ..., B_i$. Also let $B_j = B^a_i$, for some $j < i$, because $B^a_i$ is a full block. Recall that $B_j$ is a full block which is picked after $B_{j-1}$ as per our block generation process. We now argue that if $A$ has positive contribution to utility, then that contradicts with the way blocks are generated.
%
%Items of $B_i$ has a budget strictly greater than budget of $a_i$ and items of $A \setminus B_i$ has budget at least same as budget of $a_i$. Thus $A$ appears before $B_j$ in $\mathcal{I}$. Since $A$ has positive contribution, we know that $\utilow(A \mid B_1, ..., B_{j-1}) \geq 0$. Hence $A$ should be chosen as the $j$-th block instead of $B_j$, a contradiction.
\end{proof}

From the above lemma, we notice that for an over-budgeted block $B_i$, as long as its anchor item $a_i$ is not adopted
	yet, $B_i$ together with other adopted items in $B_{j}, \ldots, B_{i-1}$  
	only contributes negative marginal social welfare. 
Therefore, we could ignore their propagation and marginal contribution in our accounting method. 
However, we cannot ignore block $B_i$ in the propagation when it co-occur with its anchored block $a_i$.
The following analysis is based on the above idea.

\eat{ %%% The following is commented out, which is about the old padding technique.



 This suggests the following additional padding process similar to that in Section~\ref{sec:pad1}.

\subsubsection{Revised Padding Process}

\weic{I noticed that the padding process for the nonuniform budget case does not need to be done in two steps.
We use to say that we first pad the partial blocks that contains its own highest indexed items, and then
pad the full block when its anchor item appears at the seed node.
The first step is  not needed. 
If a block is over-budgeted and its anchor item is not present, we don't have to pad it to a full block.
}

We extend the padding process for the uniform budget case as described in Section \ref{sec:pad1} to the
	nonuniform budget case.
Notice that in the uniform budget case, all blocks would be properly budgeted, and thus the anchor item of a block 
	is the highest indexed item in the block, so the definition of anchor item used in the uniform budget section is
	consistent with our definition here.
Then in the uniform budget case, if a partial block contains its anchor item, we pad the block to be the full block.

In the nonuniform budget case, each block $B_i$ has its anchor block $B^a_i$ and anchor item $a_i$.
We revise the padding process such that if a seed node $v$ is assigned the anchor item $a_i$, 
	then we pad the corresponding block to a full block $B_i$ (if it is not already full).
Note that if $B_i$ is a properly budgeted block, this means the block containing $a_i$ is padded, and this
	is consistent with the padding process in the uniform budget case.
The extension is on over-budgeted blocks, where we pad an over-budget block to full if its anchor item is
	present at the seed node.
Also note that one item could be the anchor item for more than one blocks, so more than one blocks may be padded
	due to the presence of this item.

The idea of the above padding process is in principle similar to the uniform budget case, and it follows from
	Lemma~\ref{lem:anchor}.
That is, by Lemma~\ref{lem:anchor}, an over-budgeted block not co-occurring with its anchor item only provides
	negative marginal social welfare, and thus we do not need to count them.
Then to avoid later that such a block merges with it anchor item to start generating positive social welfare,
	we pad the blocks already having the anchor items so that such a merge can be treated simply as the
	padded blocks propagating together with its anchor, and we never need to account for the new positive social welfare
	generated by a merge.
We now formalize this idea in the following analysis.

%For an arbitrary seed allocation $\allalloc$, we first 
%	follow the padding process described for the uniform budget in \ref{sec:pad1}. 
%Namely, for each partial block that contains the highest indexed item of its corresponding full block $B_i$,
%	the partial  block is padded to a full block. 
%Notice that in the nonuniform budget case, we pad all partial blocks containing its own highest indexed item, 
%	even if the block is an over-budgeted block.
%This is for the convenience of the discussion.
%By our assumption the highest indexed item has the least budget among all other items of $B_i$. Therefore, after this process, the number of full blocks $B_i$ assigned to seeds is at most the proposed budget of $B_i$. Then we perform an additional padding as described next.
%
%For an over-budgeted block $B_i$, every seed node $v$ that is assigned the anchor item $a_i$ but not the block $B_i$, we pad $v$ with the entire block $B_i$. 
%After the padding process, the following claims hold true.

\begin{lemma}\label{lem:effectiveseed}
After padding, the number of seeds containing both over budgeted block $B_i$ and its corresponding anchor item $a_i$ is at most the effective budget of $B_i$. 
\end{lemma}
\begin{proof}
By the definition of the anchor block and the anchor item, we can see that if $a_i$ is the anchor item for some 
	block $B_i$, then it must also be the anchor item for its own block, because it has the minimum budget 
	among all blocks preceding its own block.
This means that the block containing $a_i$ will not be padded due to the presence of some other item, and it 
	can only be padded to full due to the presence of $a_i$ itself. 
Therefore, item $a_i$ will never be padded at any seed node, and
	the number of seeds that can contain $a_i$ is at most the budget of $a_i$, which in turn is the effective budget of $B_i$. Hence the lemma follows.
\end{proof}

\weic{I am in the middle of revising the following lemma, so please leave it as is now.}

\begin{lemma}\label{lem:traceback}
During the propagation under a graph possible world $W^G$, 
	if a node $v$ adopts both an over budgeted block $B_i$ and its anchor item $a_i$, 
	then due to padding, there must be a path in $W^G$ from a seed node to $v$ such that
		all nodes on the path adopts both $a_i$ and $B_i$. 
\end{lemma}

\begin{proof}
Since $v$ adopts $a_i$, there must be a path from a seed node $u$ that adopts $a_i$ to $v$ in $W^G$.
Due to padding, seed node $u$ must have been padded with the full block $B_i$.
	
After the padding, item $a_i$ never appears alone and is always bundled together with block $B_i$. 
By Lemma~\ref{lem:reachable}, all nodes reachable in $W^G$ from a seed that adopts both $a_i$ and $B_i$ will
	also adopt $a_i$ and $B_i$ 

Thus when they reach a node an gets adopted, we can find the path to the padded seed node from where the propagation started.
\end{proof}

With the above claims, we now proceed to the account the social welfare of arbitrary seed allocation $\allalloc$. In particular, for an over budgeted block $B_i$, we will define $\allseeds_{B_i}$ as the set of seed nodes that contain both $a_i$ and $B_i$ after the padding. However for a properly budgeted block $B_i$, $\allseeds_{B_i}$ is simply the seed nodes to which $B_i$ is assigned. Then we have the following lemma.

} %%% this is the end of the commented out part about the old padding technique

\weic{
The proof of the following lemma is very similar to the proof of Lemma~\ref{lem:allsw}.
In fact, I copy/paste that proof and made minor changes.
I want to write the full proof here, since I feel that eventually perhaps we could remove the uniform budget
	section, since I don't see it providing much more benefit at the moment.
}

\begin{lemma}\label{lem:allasw}

For any arbitrary seed allocation $\allalloc$, the expected social welfare in $\ow$, is $\sww(\allalloc) \leq \sum_{i\in [t]} \sigma(\allseeds_{a_i}) \cdot \Delta_i$, where $\allseeds_{a_i}$ is the seed set assigned the anchor
	item $a_i$ of block $B_i$, and $\Delta_i$ is as defined before. 

\end{lemma}

\begin{proof}
For a graph possible world $W^G$, 
suppose that after the diffusion process under $W^G$, every node $v$ adopts item set $A_v$.
Let $A_{v,i} = A_v \cap B_i$ for all $i \in [t]$, and
$\Delta^{A_v}_i = \utilow(A_{v,i} \mid A_{v,1} \cup \ldots \cup A_{v,i-1})$.
Thus, we have 
\begin{align}
\sww(\allalloc) & = \E_{W^G} \left[\sum_{v\in V} \utilow(A_v) \right] 
= \E_{W^G} \left[\sum_{v\in V} \sum_{i\in [t]} \Delta^{A_v}_i \right]  \nonumber \\
&	= \sum_{i\in [t]} \E_{W^G} \left[ \sum_{v\in V} \Delta^{A_v}_i \right], \label{eq:welfareEquiv2}
\end{align}
where the expectation is taken over the randomness of the graph possible worlds, and thus we use
subscript $W^G$ under the expectation sign to make it explicit.
By switching the summation signs and the expectation sign in the last equality above, 
we show that the expected social welfare can be
accounted as the summation among all blocks $B_i$  of the expected marginal gain of block $B_i$ on all nodes.
We next bound $\E_{W^G} \left[\sum_{v\in V} \Delta^{A_v}_i \right]$ for each block $B_i$.

Under the graph possible world $W^G$, for each $v\in V$, there are three possible cases for $A_{v,i}$.
In the first case, $A_{v,i} = \emptyset$. In this case, $\Delta^{A_v}_i = 0$, so we do not need to count 
the marginal gain $\Delta^{A_v}_i$.
In the second case, $A_{v,i}$ is not empty but
	it does not co-occur with block $B_i$'s anchor $a_i$, that is $a_i \not\in A_v$, and $A_{v,i} \ne \emptyset$.
In this case, Let $A' = A \cap (B_j \cup \ldots \cup B_i)$, where $B_j$ is the anchor block of $B_i$.
Then $A'$ is not empty. 
By Lemma~\ref{lem:anchor}, $\utilow(A' \mid B_1 \cup \ldots \cup B_{j-1}) < 0$.
Since we have $\utilow(A' \mid B_1 \cup \ldots \cup B_{j-1})  
	= \sum_{s=j}^i \Delta^{A_v}_s$, 
This means that the cumulative marginal gain of $\Delta^{A_v}_s$ with $j\le s \le i$ is negative, so 
	we can relax them to $0$, effectively not counting the marginal gain of $\Delta^{A_v}_i$ either.

In the third case, $A_{v,i}$ is nonempty and co-occur with its anchor $a_i$, 
	i.e. $a_i \in A$ and $A_{v,i} \ne \emptyset$.
Under this case, by Lemma~\ref{lem:marginalBound}, $\Delta^{A_v}_i \le \Delta_i$, and so we relax
$\Delta^{A_v}_i$ to $\Delta_i$.
This relaxation would occur only on nodes $v$ that adopts $a_i$.
By the EPIC model, for an individual item $a_i$, $v$ could adopt $a_i$ only when there is path in $W^G$ 
from a seed node that adopts $a_i$ to node $v$. 
As defined in the lemma, $S_{a_i}$ is the set of seed nodes that are assigned $a_i$.
Let $\Gamma(S_{a_i}, W^G)$ be the set of nodes that are reachable from $S_{a_i}$ in $W^G$.
Then, there are at most $| \Gamma(S_{a_i}, W^G)|$ nodes at which we relax  $\Delta^{A_v}_i$ to $\Delta_i$ 
for block $B_i$.
This means that 
\begin{align} \label{eq:marginalRelax2}
\sum_{v\in V} \Delta^{A_v}_i \le | \Gamma(S_{a_i}, W^G)| \cdot \Delta_i.
\end{align}
Furthermore, notice that $\E_{W^G}[| \Gamma(S_{a_i}, W^G)| ] = \sigma(S_{a_i})$, by the live-edge representation of
the IC model.
Therefore, together with Eq.~\eqref{eq:welfareEquiv2} and~\eqref{eq:marginalRelax2}, we have
\begin{align*}
\sww(\allalloc) & \le \sum_{i\in [t]} \E_{W^G} \left[  | \Gamma(S_{a_i}, W^G)| \cdot \Delta_i \right] \\
& =  \sum_{i\in [t]} \sigma(S_{a_i}) \cdot \Delta_i.
\end{align*}
This concludes the proof of the lemma.
%
%
%
%
%------
%
%By Lemma \ref{lem:anchor}, we know that during the propagation process, if some node $v$ adopts an over budgeted block $B_i$ but not its anchor item $a_i$, we could ignore $B_i$'s contribution to social welfare, since its marginal on the previous $B_1, … B^a_i$ where $B^a_i$ is its anchor block, is strictly negative. So we only need to account for the marginals of $B_i$ when $B_i$ appears together with its anchor item $a_i$. By Property \ref{clm:traceback}, such adoption can always be traced back to a seed that is assigned both $a_i$ and $B_i$. Thus for an over budgeted block the marginal contribution of $B_i$ is at most $\sigmaw(\allseeds_{B_i}) \cdot \Delta_i$.
%
%For a properly budgeted block $B_i$, we can think of the last item of the block as its anchor item. Thus such block will always be adopted. Also every time such a block is adopted, we know that all blocks from $B_1, ..., B_{i-1}$ have already been adopted. Hence the marginal contribution of a single adoption of the block is again $\Delta_i$. Thus the total contribution to overall social welfare is $\sigmaw(\allseeds_{B_i}) \cdot \Delta_i$.
%
%Since blocks are pairwise disjoint, the total social welfare is just the sum of all individual contributions of the bocks. 
\end{proof}

We are now ready the state the main correctness result below.

\begin{lemma} {\sc (Correctness of $\algo$ under the Nonuniform Badget Case)\ \ }\label{lem:nonuniformbudget}
	Let $\greedAlloc$ be the greedy allocation and $\allalloc$ be any arbitrary allocation.
	When the item budgets are nonuniform, given $\epsilon$ and $\ell$, the expected social welfare $\sw(\greedAlloc) \geq (1 - \frac{1}{e} - \epsilon ) \cdot \sw(\allalloc)$ with at least $1 - \frac{1}{|V|^{\ell}}$ probability.
\end{lemma}

\begin{proof}
	From Lemma \ref{lem:greedyasw} , we have for a possible world $\ow = (W^G, W^N)$,
	$\sww(\greedAlloc) =\sum_{i\in [\numblocks]} \sigma(\greedESeeds_{B_i}) \cdot \Delta_i $,
	where the size of $\greedESeeds_{B_i}$ is the effective budget of $B_i$.
	
	For an arbitrary allocation $\allalloc$, 
	since $a_i$ is the anchor item of $B_i$, by its definition 
	we know that $|\allseeds_{a_i}| = |\greedESeeds_{B_i}|$. 
	%In the greedy allocation we again know that $|\greedSeeds_{B_i}| = k$. 
	By the correctness of the prefix-preserve influence maximization algorithm we use in line~\ref{alg:PRIMM} 
	(Definition~\ref{def:PRIMM}, to be instantiated in Section~\ref{sec:PRIMM}), we have that 
	with probability at least $1 - \frac{1}{|V|^{\ell}}$, 
	$\sigma(\greedESeeds_{B_i}) \geq (1 - \frac{1}{e} - \epsilon) \sigma(\allseeds_{a_i})$, for all blocks $B_i$'s
	and their corresponding anchors $a_i$'s.
	
	Let the distribution of world $\ow$ be $\dow$. Then we have that 
	with probability at least $1 - \frac{1}{|V|^{\ell}}$,
	\begin{align*}
	\sw(\greedAlloc) &= \mathbb{E}_{\ow \sim \dow} [\sww(\greedAlloc)] \\
	&= \mathbb{E}_{\ow \sim \dow} \left[\sum_{i\in [\numblocks]} \sigma(\greedESeeds_{B_i}) \cdot \Delta_i \right]\\
	&\geq \mathbb{E}_{\ow \sim \dow} \left[\sum_{i\in [\numblocks]}(1 - \frac{1}{e} - \epsilon) \sigma(\allseeds_{a_i}) \cdot \Delta_i \right]\\
	& \geq (1 - \frac{1}{e} - \epsilon) \mathbb{E}_{\ow \sim \dow} [ \sww(\allalloc)]  \\
	& = (1 - \frac{1}{e} - \epsilon) \sw(\allalloc).
	\end{align*}
	Therefore, the lemma holds.
\end{proof}





%\begin{theorem} \label{thm:arbitrarybudget}
%Let $\greedAlloc$ be the greedy allocation and $\allalloc$ be any arbitrary allocation, then in world $\ow$, for given $\epsilon$ and $\ell$, $\sigmaw(\greedESeeds_{B_i}) \geq (1 - \frac{1}{e} -\epsilon) \sigma(\allseeds_{B_i})$ with probability at least $1 - \frac{1}{|V|^{\ell}}$.
%\end{theorem}
%
%\begin{proof}
%For the greedy allocation $\greedAlloc$, from Claim \ref{clm:full_prefix}, we know that a block $B_i$ is adopted only when all of its previous blocks are also adopted. Thus it contributes to social welfare only for its effective greedy seeds $\greedESeeds_{B_i}$, the seeds that also contain all blocks of $B_1, ..., B_{i-1}$. The number of such seeds, i.e. $|\greedESeeds_{B_i}|$, is the minimum proposed budget that any of the blocks $B_1, ..., B_{i-1}$ has. Moreover this is exactly the effective budget $\bbude_i$, of block $B_i$. Thus $|\greedESeeds_{B_i}| = \bbude_i$. 
%
%By Claim \ref{clm:effectiveseed} and \ref{clm:traceback} we know in arbitrary allocation $\allalloc$, for an over budgeted block $B_i$, its contribution to social welfare comes only from the effective budget of the block as effective budget is the number of time its anchor item $a_i$ can appear in a seed node. Thus for over budgeted block $|\allseeds_{B_i}| = \bbude_i = |\greedESeeds_{B_i}|$. For a properly budgeted block $B_i$, $|\greedESeeds_{B_i}| = |\greedSeeds_{B_i}| = |\allseeds_{B_i}| = \bbude_i$ trivially holds. Now since $\PRIMM$ has item wise prefix order property \ref{prop:prefix}, for budget $\bbude_i$, which is the budget of item $a_i$, $\sigmaw(\greedESeeds_{B_i}) \geq (1 - \frac{1}{e} -\epsilon) \sigmaw(\allseeds_{B_i})$ with probability at least $1 - \frac{1}{|V|^{\ell}}$.
%\end{proof}

%Lemma \ref{lem:greedyasw}, \ref{lem:allasw} and Theorem \ref{thm:arbitrarybudget} together shows that Theorem \ref{thm:uniformbudget} is true even when items' budgets are non uniform.

\eat{
\begin{theorem}\label{thm:arbitrarybudget}
Let $\greedAlloc$ be the greedy allocation and $\allalloc$ be any arbitrary allocation, then the expected social welfare $\sw(\greedAlloc) \geq (1 - \frac{1}{e} ) \cdot \sw(\allalloc)$
\end{theorem}

\begin{proof}
From Lemma \ref{lem:greedyasw} we have for outer world $\ow$,
$\sww(\greedAlloc) =\sum_{i\in [t]} \sigmaw(\greedESeeds_{B_i}) \cdot \Delta_i $.\\
From the equivalent classes of possible worlds, we have,
$\sw(\greedAlloc) = \sum_{OW \in \mathbf{OW}} Pr[OW] \cdot \sww(\greedAlloc)$, where $\mathbf{OW}$ is set of all distinct classes of outer worlds.

Now for any allocation $\allalloc$, consider an over budgeted block $B_i$. From property \ref{clm:full_prefix}, we know that its effective greedy seeds $\greedESeeds_{B_i}$ are those seeds that contains all blocks of $B_1, ..., B_{i-1}$. The number of such seeds, i.e. $|\greedESeeds_{B_i}|$, is the minimum proposed budget that any of the blocks $B_1, ..., B_{i-1}$ has. Moreover this is exactly the effective budget $\bbude_i$, of $B_i$. Thus $|\greedESeeds_{B_i}| = \bbude_i$. By property \ref{prop:effectiveseed} we know in arbitrary allocation $\allalloc$, $|\allseeds_{B_i}| = \bbude_i$. For a properly budgeted block $B_i$, $|\greedESeeds_{B_i}| = |\greedSeeds_{B_i}| = |\allseeds_{B_i}|$.


Consequently for any block $B_i$, we can say that $\sigmaw(\greedESeeds_{B_i}) \geq (1 - \frac{1}{e}) \sigmaw(\allseeds_{B_i})$. Thus
\begin{align*}
\sw(\greedAlloc) &= \sum_{OW \in \mathbf{OW}} Pr[OW] \cdot \sum_{i\in [t]} \sigmaw(\greedESeeds_{B_i}) \cdot \Delta_i \\
&\geq \sum_{OW \in \mathbf{OW}} Pr[OW]\cdot (1 - \frac{1}{e})  \sum_{i\in [t]} \sigma(\allseeds_{B_i}) \cdot \Delta_i \\
& \geq (1 - \frac{1}{e}) \sum_{OW \in \mathbf{OW}} Pr[OW]\cdot \sww(\allalloc) \text{, by virtue of Lemma \ref{lem:allasw}} \\
& = (1 - \frac{1}{e}) \sw(\allalloc)
\end{align*}
\end{proof}
}

\subsection{Item wise prefix preserving IMM} \label{sec:PRIMM}

IMM \cite{tang15} is one of the state of the art algorithm for influence maximization involving single item. In presence of multiple items, however it is not prefix preserving (Definiton \ref{def:PRIMM}). In this section we present an extension of the vanilla IMM, called $\PRIMM$ (\em{PR}efix \em{IMM}), that is prefix preserving. The Algorithm is shown in Algorithm \ref{alg:IMM_adopted}. Notice that $\nodeselect(\mathcal{R},k)$, is the standard greedy algorithm to find a seed set of size $k$ by solving maximum coverage on RR set $\mathcal{R}$. The $\nodeselect$ algorithm is same as Alg $1$ of IMM, which we donot repeat for brevity.  

\begin{algorithm}[t!]
%\begin{small}
\DontPrintSemicolon
\caption{$\PRIMM$ $(\bvec, G, \epsilon, \ell)$} \label{alg:IMM_adopted}
Initialize $\mathcal{R} = \emptyset$; \\
$s = 1$, $n = |V|$, $i = 1$, $\ell = \ell \cdot (1 + \log 2 / \log n )$ ; \\ \label{lin:ellb}
$\ell^\prime = \log_n(n^{\ell} \cdot |\bvec|)$; \\ \label{lin:ell}
$\epsilon^\prime = \sqrt{2} \cdot \epsilon$; \\
\While{$i \leq \log_2(n) - 1$ and $s \leq |\bvec|$} {
	$k = \bvec_s$, $LB =1$; \\
	Let $x = \frac{n}{2^i}$ and $\theta_i = \lambda^\prime_k/x$, where $\lambda^\prime_k$ is defined in Eq. \ref{eq:lambdap}; \\
	\While{$|\mathcal{R}| \leq \theta_i$} {
		Generate an RR set for a randomly selected node $v$ of $G$ and insert in $\mathcal{R}$; \\
	}
	Let $S_k =\nodeselect(\mathcal{R}, k)$; \\
	\If{$n \cdot F_{\mathcal{R}}(S_k) \geq (1 + \epsilon^\prime)\cdot x$} { \label{lin:cov}
		$LB = n \cdot F_{\mathcal{R}(S_k)} / (1+\epsilon^\prime) $; \\
		Let $\theta_k = \lambda^\ast_k / LB$, where $\lambda^\ast_k$ is defined in Eq. \ref{eq:lambdaa}; \\
		\While{$|\mathcal{R}|<\theta_k$} {
			Generate an RR set for a randomly selected node $v$ of $G$ and insert in $\mathcal{R}$; \\
		}
		$s = s + 1 $; \\	
	}
	\Else{ $i= i+1$; \\}
	
}
$\theta_k = \lambda^\ast_{\bvec_s}/LB$; \\
\While{$|\mathcal{R}|<\theta_k$} {
	Generate an RR set for a randomly selected node $v$ of $G$ and insert in $\mathcal{R}$; \\
}	
$S_{\bmax} = \nodeselect(\mathcal{R}, \bmax)$; \\ \label{lin:nodes}
\textbf{return} $S_{\bmax}$ as the final seed set;
\end{algorithm}

$\PRIMM$, ingests four inputs, namely the budget vector $\bvec$, graph $G$, $\epsilon$ and $\ell$. $\bvec$ is sorted in nonincreasing order as stated earlier in section \ref{sec:nonuniformBudget}. Given $\ell^\prime$ for a budget $k$ IMM generates RR set $\mathcal{R}$, such that $|\mathcal{R}|\geq \lambda^\ast_k / OPT_k$ with probability at least $1 - 1/n^{\ell^\prime}$. We will reason about our choice of of $\ell^\prime$ (line \ref{lin:ell}) in Theorem \ref{thm:primm}. Before that we present a brief description of $\PRIMM$.
\begin{equation}\label{eq:lambdap}
\lambda^\prime_k = \frac{(2+\frac{2}{3}\epsilon^\prime) \cdot (\log {n \choose k} + \ell^\prime \cdot \log \ n+\log\log_{2} \ n )\cdot n}{\epsilon^{\prime 2}}
\end{equation} 

\begin{gather}\label{eq:lambdaa}
\lambda^\ast_k = 2n \cdot ((1 - 1/e)\cdot \alpha + \beta_k)^2 \cdot \epsilon^{-2} \\
\text{where, $\alpha$ is constant, }\beta_k = \sqrt{(1 - 1/e) \cdot (\log \tbinom{n}{k}+\ell^\prime \log \ n+ \log \ 2)} \nonumber
\end{gather} 

The basic idea of $\PRIMM$ is to generate enough RR sets such that for any budget $k \in \bvec$, $|\mathcal{R}| \geq \lambda^\ast_k / OPT_k$, with probability at least $1 - 1/n^{\ell^\prime}$. Since $OPT_k$ is unknown, we rely on the lower bound of $OPT_k$, i.e., $LB_k$ as proposed in IMM. Specifically $\PRIMM$ starts from the highest budget. For a given budget $k$ and $i$ it samples enough RR sets in $\mathcal{R}$ first (line $8-9$) and then checks the coverage condition on the sampled RR set (line $11$). Note if $\mathcal{R}$ already had enough number of RR sets (generated at a previous budget), then it skips RR set generation and moves directly to coverage check. If coverage condition succeeds, then $LB$ for the budget $k$ is found. It uses the $LB$ to find required number of RR sets (line $13-15$) for $k$ and moves to next budget. Else it increments $i$ to sample more RR set for budget $k$ (line $18$). 

If for any budget all possible $i$ values are tested, $\PRIMM$ breaks the for loop and generates RR set using $LB=1$ (line $19$), which is the lowest possible value of $LB$. Further since budgets are sorted in nonincerasing order and $\lambda^\ast_k$ is monotone in $k$ (eq. \ref{eq:lambdaa}), there cannot be any remaining budget $k^\prime$ for which $\lambda^\ast_{k^\prime} /LB$ (line $19$) is higher. Hence the RR set generation process terminates. Finally $\PRIMM$ selects the top $\bmax$ seeds. For any budget $k$ we therefore have the following lemma.

\begin{lemma}\label{lem:primm}
For any budget $k \in \bvec$ and the RR set $\mathcal{R}$ returned by $\PRIMM$, $|\mathcal{R}|\geq \lambda^\ast_k / OPT_k$ holds with probability at least $1 - 1/n^{\ell^\prime}$.
\end{lemma}

\begin{proof}
Given $x \in [1,n]$, $\epsilon^\prime$ and $\delta_3 \in (0,1)$ and a budget $k$. Let $S_k$ be the seed set of size $k$ obtained by invoking $\nodeselect(\mathcal{R},k)$, where,
\begin{equation}\label{eq:rrsize}
|\mathcal{R}| \geq \frac{(2+\frac{2}{3}\epsilon^\prime)\cdot (\log {n \choose k} + \log (1/\delta_3))}{\epsilon^\prime} \cdot \frac{n}{x} 
\end{equation} 
Then, from Lemma $6$ of \cite{tang15}, if $OPT_k < x$, $n \cdot F_{\mathcal{R}}(S_k) < (1+\epsilon^\prime) \cdot x$ with probability at least $(1-\delta_3)$. Now let $j = \ceil{\log_2 \frac{n}{OPT_k}}$. By union bound we have that the $\PRIMM$ has probability at most $(j-1) / (n^{\ell^\prime} \cdot \log_2 n)$ to satisfy the coverage condition of line \ref{lin:cov} for the budget $k$. Then by lemma $7$ of \cite{tang15} and the union bound, $\PRIMM$ will have $LB_k \leq OPT_k$ with probability at least $1 - n^{\ell^\prime}$. We know that for any $k \in \bvec$, $|\mathcal{R}| \geq \lambda^\ast_k / LB_k$, hence the lemma follows.
\end{proof}

We are now ready to prove the correctness of $\PRIMM$ in following theorem.

\begin{theorem} \label{thm:primm}
$\PRIMM$ returns a prefix preserving $(1 - 1/e - \epsilon)$ approximate solution to influence maximization with at least $1 - 1/n^\ell$ probability. 
\end{theorem}

\begin{proof}

We know from Lemma \ref{lem:primm} that the RR set sampling for any budget can fail with probability at most $1/n^{\ell^\prime}$. By applying union bound over all the budgets, we have that the failure probability of $\PRIMM$ is at most $\sum_{k \in \bvec} 1/n^{\ell^\prime} = |\bvec| \cdot 1/n^{\ell^\prime}$. By setting $\ell^\prime = \log_n(n^{\ell} \cdot |\bvec|)$, we bound failure probability of $\PRIMM$ to at most $1/n^\ell$. Also by using $\ell^\prime$, for computing $\alpha$ and $\beta$ in Eq. \ref{eq:lambdaa}, we know from Theorem $1$ of \cite{tang15}, that node selection of $\PRIMM$ (line \ref{lin:nodes}) returns a $(1 - 1/e - \epsilon)$ solution with at least $1 - 1/n^{\ell}$ probability. Notice that node selection works in a greedy manner, which by definition is prefix preserving. Hence by union bound $\PRIMM$ returns $(1 - 1/e - \epsilon)$ approximate prefix preserving solution with at least $1 - 2/n^{\ell}$ probability.

Finally by increasing $\ell$ by a factor of $1 + \log 2/ \log n$ in line \ref{lin:ellb}, we raise $\PRIMM$'s probability of success to $1 - 1/n^\ell$. 
\end{proof}

\subsubsection{Running time}

The running time of $\PRIMM$ mostly involves two parts: the time needed to generate the RR set $\mathcal{R}$ and the total time of invoking all $\nodeselect$. From Lemma $9$ of \cite{tang15}, we have for any budget $k$, RR set generated for that budget $\mathcal{R}_k$

\begin{align*}
\mathbb{E}[|\mathcal{R}_k|] &\leq \frac{3 max\{ \lambda^\ast_k, \lambda^\prime_k\} \cdot (1+\epsilon^\prime)^2}{(1 - 1/e)\cdot OPT_k}
\end{align*}

Since $\lambda^\prime_k$ and $\lambda^\ast_k$ are both monotone in $k$ (Eq. \ref{eq:lambdap} and Eq \ref{eq:lambdaa}), we know their maximums are achieved for $k = \bmax$. Further let $OPT_{min}$ be the minimum $OPT$ across all budgets, then for any $\mathcal{R}_k$,

\begin{align*}
\mathbb{E}[|\mathcal{R}_k|] &\leq \frac{3 max\{ \lambda^\ast_{\bmax}, \lambda^\prime_{\bmax}\} \cdot (1+\epsilon^\prime)^2}{(1 - 1/e)\cdot OPT_{min}} \\
& = O((\bmax+\ell^\prime)n\log \ n \cdot \epsilon^{-2} / OPT_{min})
\end{align*}

Further since $\PRIMM$ reuses the RR sets instead of generating them from scratch for every budget, for the RR set $\mathcal{R}$ generated by $\PRIMM$,

\begin{align}\label{eq:rsize}
\mathbb{E}[|\mathcal{R}|] &= max_{k \in \bvec}\{ \mathbb{E}[|\mathcal{R}_k|] \} \nonumber \\ 
& = O((\bmax+\ell^\prime)n\log \ n \cdot \epsilon^{-2} / OPT_{min})
\end{align}

Let for a RR set $R \in \mathcal{R}$, $w(R)$ denote the number of edges in $G$ pointing to nodes in $R$. If $EPT$ is the expected value of $w(R)$, then we know, $n \cdot EPT \leq m \cdot OPT_{min}$ \cite{tang14}. Hence using Equation \ref{eq:rsize}, the expected total time to generate $\mathcal{R}$,

\begin{align}\label{eq:rtime}
\mathbb{E}[\sum_{R \in \mathcal{R}}w(R)] &= \mathbb{E}[|\mathcal{R}|] \cdot EPT \nonumber \\
& = O((\bmax+\ell^\prime)(n+m)\log \ n \cdot \epsilon^{-2})
\end{align}

Using Theorem \ref{thm:primm} and Eq. \ref{eq:rtime} we now prove the following theorem,
\begin{theorem}
$\PRIMM$ is prefix preserving and returns a $(1 - 1/e - \epsilon)$-approximate solution with at least $1 - 1/n^\ell$ probability in $O(|\bvec|(\bmax+\ell^\prime)(n+m)\log \ n \cdot \epsilon^{-2})$ expected time .
\end{theorem}

\begin{proof}
From Theorem \ref{thm:primm}, we have that $\PRIMM$ returns a prefix preserving $(1 - 1/e - \epsilon)$-approximate solution with at least $1 - 1/n^\ell$ probability. In that process $\PRIMM$ invokes $\nodeselect$, $\log_2 \ n -1 + |\bvec|$ times in the while loop and once to find the final seed set $S_{\bmax}$. Let $\mathcal{R}_i$ be the susbset of $\mathcal{R}$ used in the $i$-th iteration of the loop. Since $\nodeselect$ involves one pass over all RR set, on a given input $\mathcal{R}_i$, it takes $O(\sum_{R \in \mathcal{R}_i} |R|)$ time. Recall $|\mathcal{R}_i|$ doubles with every increment of $i$. Hence it is a geometric sequence with a common ratio of $2$. Now from Theorem $3$ of \cite{tang15} and the fact that across the while loop $\nodeselect$ is called an additional $|\bvec|$ times, we have total cost of invoking all $\nodeselect$ is $O(|\bvec| \cdot \mathbb{E}[\sum_{R \in \mathcal{R}}|R|])$.

Since $|R| \leq w(R)$, for any $R \in \mathcal{R}$, then using Eq. \ref{eq:rtime} we have,
\begin{align*}
O(|\bvec| \cdot \mathbb{E}[\sum_{R \in \mathcal{R}}|R|]) &= O(|\bvec| \cdot \mathbb{E}[\sum_{R \in \mathcal{R}}w(R)]) \\
& = O(|\bvec|(\bmax+\ell^\prime)(n+m)\log \ n \cdot \epsilon^{-2})
\end{align*}

Hence the theorem follows.
\end{proof}


==> sec-app.tex <==
\appendix


\section{Proofs and additional theoretical analysis}

We include missing proofs in the main text in this section.
The theorems and lemmas are restated with the original numbering
	for convenience.

\subsection{Proofs for Properties of \model (Section \ref{sec:prop})} \label{sec:app4}


{\lemitemunion*}
\begin{proof}
For any subset $C \subseteq A\cup B$, we have
	\begin{align*} 
	\util_W(C) & = \util_W(C\setminus B \mid B \cap C) + \util_W(B \cap C) \le \util_W(C\setminus B \mid B) + \util_W(B) \\
	& = \util_W(C \cup B) = \util_W(B \mid C\setminus B) + \util_W(C \setminus B) \\
	& \le \util_W(B \mid A) + \util_W (A) = \util_W(A \cup B).
	\end{align*} 
%	Inequality~\eqref{eq:CB} follows from applying supermodularity of $\util_W$
%	on the first term, and applying local maximum of $B$ on the second term.
%	Inequality~\eqref{eq:AB} follows applying supermodularity of $\util_W$
%	on the first term, and applying local maximum of $A$ on the second term.
\end{proof}
\vspace{-6mm}
\eat{
{\lemitemunion*}
\begin{proof}
For any subset $C \subseteq A\cup B$, we have
	\begin{align} 
	\util_W(C) & = \util_W(C\setminus B \mid B \cap C) + \util_W(B \cap C)  \nonumber \\
	& \le \util_W(C\setminus B \mid B) + \util_W(B)   \label{eq:CB} \\
	& = \util_W(C \cup B) \nonumber \\
	& = \util_W(B \mid C\setminus B) + \util_W(C \setminus B) \nonumber \\
	& \le \util_W(B \mid A) + \util_W (A)  \label{eq:AB} \\
	& = \util_W(A \cup B). \nonumber 
	\end{align} 
%	Inequality~\eqref{eq:CB} follows from applying supermodularity of $\util_W$
%	on the first term, and applying local maximum of $B$ on the second term.
%	Inequality~\eqref{eq:AB} follows applying supermodularity of $\util_W$
%	on the first term, and applying local maximum of $A$ on the second term.
\end{proof}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\lemlocalmaximum*}
\begin{proof}
We prove by an induction on $t$.
The base case of $t=1$ is true because by the model, node $u$ adopts the local maximum among
	all subsets of items allocated to it.
For the induction step, suppose for a contradiction that $\adoptws(u,t)$ is not a local maximum
	but $\adoptws(u,t-1)$ is a local maximum.
Then there must exist a $C\subset \adoptws(u,t)$ that is a local maximum and
	$\util_W(C) > \util_W(\adoptws(u,t))$.
By Lemma~\ref{lem:itemunion}, $C \cup \adoptws(u,t-1)$ is also a local maximum, and thus
	$C \cup \adoptws(u,t-1)$ cannot be $\adoptws(u,t)$.
But since $\util_W(C \cup \adoptws(u,t-1)) \geq \util_W(C) > \util_W(\adoptws(u,t))$, $u$
	should adopt $C \cup \adoptws(u,t-1)$ instead of $\adoptws(u,t)$, a contradiction.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{
{\lemitemunion*}
\begin{proof}
	First, observe that $\util_W(A) = \val(A) - \price(A) + \noise_W(A)$, where $-\price(\cdot)$ and $\noise_W(\cdot)$ are both modular functions. Since $\val(\cdot)$ is supermodular, it follows that $\util_W(\cdot)$ is supermodular as well. 
	For any subset $C \subseteq A\cup B$, we have
	\begin{align} 
	\util_W(C) & = \util_W(C\setminus B \mid B \cap C) + \util_W(B \cap C)  \nonumber \\
	& \le \util_W(C\setminus B \mid B) + \util_W(B)   \label{eq:CB} \\
	& = \util_W(C \cup B) \nonumber \\
	& = \util_W(B \mid C\setminus B) + \util_W(C \setminus B) \nonumber \\
	& \le \util_W(B \mid A) + \util_W (A)  \label{eq:AB} \\
	& = \util_W(A \cup B). \nonumber 
	\end{align} 
	In the above derivation, Inequality~\eqref{eq:CB} follows from applying supermodularity of $\util_W$
	on the first term, and applying local maximum of $B$ on the second term, with the fact that
	$B\cap C \subseteq B$; and
	Inequality~\eqref{eq:AB} follows from  applying supermodularity of $\util_W$
	on the first term, and applying local maximum of $A$ on the second term, with the fact that
	$C \setminus B \subseteq A$.
	%
	%The first and third equality follow from the definition of $\util_W(\cdot)$. The first inequality follows from supermodularity of $\util_W(\cdot)$, while the last inequality follows from the fact that $\util_W(B)$ is the maximum among its subsets, which implies $\util_W(B) \geq \util_W(A\cap B)$. 
	%$\util_W(A\cup B) \ge \util_W(B)$ could be proved symmetrically.  
	%%
\end{proof}

{\lemlocalmaximum*}
\begin{proof}
	We prove this lemma by an induction on time $t$.
	
	\noindent
	\underline{Base Case}: $t=1$. Clearly, $\adoptws(u,1) \neq \emptyset$ only for seed nodes $u$.
	By the diffusion model, $\adoptws(u,1)$ must have the maximum utility among all subsets of the desire set $\awarews(u,1)$, so $\adoptws(u,1)$ is a  local maximum w.r.t. $\util_W$. 
	
	\noindent
	\underline{Induction}:	
	Assume the claim is true for $t-1$, i.e., the adoption set $\adoptws(u,t-1)$ is a local maximum w.r.t. $\util_W$. Assume that $\adoptws(u,t)$ is not a local maximum. Then, $\exists C \subset \adoptws(u,t)$, s.t. $\util_W(C) > \util_W(\adoptws(u,t))$.
	
	W.l.o.g., assume $C$ is local maximum. If it is not, we can always select the subset of items of $C$ that has the highest utility. By definition, that subset is a local maximum and it will also be a subset of $\adoptws(u,t)$. Clearly its utility is higher than that of $C$, and hence higher than $\util_W(\adoptws(u,t))$ as well.
	
	Now since $\adoptws(u,t-1)$  and $C$ are both local maxima, by Lemma \ref{lem:itemunion},  $\adoptws(u,t-1) \cup C$ is also a local maximum and $\util_W(\adoptws(u,t-1) \cup C) > \util_W(\adoptws(u,t))$. This contradicts the adoption behavior of node $u$ defined by our model: since $\adoptws(u,t-1) \subseteq \adoptws(u,t-1) \cup C \subset \adoptws(u,t)$ and $\util_W(\adoptws(u,t-1) \cup C) > \util_W(\adoptws(u,t))$, then $u$ at time $t$ should adopt $\adoptws(u,t-1) \cup C$, instead of adopting $\adoptws(u,t)$.
	% 
	%%%%%%%%%%%%%%%%% 
	\eat{ 
		\weic{However, $u$ may have some other items in its desired set, but not in the adoption set.
			Those items complicated the situation, and make lead to an adoption set of $u$ that is
			not local maximum.
			
			This situation leads me to find the counter example of the reachability explained above.
			For now, I think that if we assume that at every seed node, the full desired set is adopted, then
			the reachability holds.
		}
	} 
	%%%%%%%%%%%%%%%%%%% 
\end{proof}


{\lemreachable*}
\begin{proof} 
	Consider a possible world $W$ and a node $u$ that adopts item $i$. Consider any node $v$ reachable from $u$ in $W$ that does not adopt $i$. Let $(u, v_1, ..., v_k, v)$ be a path in $W^E$. Assume w.l.o.g. that $v$ is the first node on the path that does not adopt $i$. $\adoptws(v_k,t)$ and $\adoptws(v,t+1)$ respectively are the itemsets adopted by $v_k$ at time $t$ and by $v$ at time $t+1$. 
	%We have $i \in \adoptws(v_k,t)$ and $i\not\in \adoptws(v,t+1)$. Also 
	Let $J = \adoptws(v_k,t) \cup \adoptws(v,t+1)$. Clearly $i \in J$ and $J \subset \awarews(v,t+1)$, desire set of $v$ at $t+1$.
	By Lemma \ref{lem:localmaximum2}, we know that both $\adoptws(v_k,t)$ and $\adoptws(v,t+1)$ are local maxima. Then by Lemma \ref{lem:itemunion}, $J$ is also a local maximum, hence $\utilw(J) \geq \utilw(\adoptws(v,t+1))$, as $\adoptws(v,t+1) \subset J$. Also, $|J|> |\adoptws(v,t+1)|$, as $J$ contains at least one more item $i$. Thus as per our diffusion model $v$ at time $t$ should adopt the larger cardinality set $J$. Consequently $i$ should be adopted by $v$.
\end{proof}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\lemreachable*}
\begin{proof}
Consider a possible world $W$ and a node $u$ that adopts item $i$. Consider any node $v$ reachable from $u$ in $W$ that does not adopt $i$. Let $(u, v_1, ..., v_k, v)$ be a path in $W^E$. Assume w.l.o.g. that $v$ is the first node on the path that does not adopt $i$. $\adoptws(v_k,t)$ and $\adoptws(v,t+1)$ respectively are the itemsets adopted by $v_k$ at time $t$ and by $v$ at time $t+1$. 
	%We have $i \in \adoptws(v_k,t)$ and $i\not\in \adoptws(v,t+1)$. Also 
	Let $J = \adoptws(v_k,t) \cup \adoptws(v,t+1)$. Clearly $i \in J$ and $J \subset \awarews(v,t+1)$, desire set of $v$ at $t+1$.
	We know that both $\adoptws(v_k,t)$ and $\adoptws(v,t+1)$ are local maximums 
		by Lemma~\ref{lem:adoptmax}. 
	Then by Lemma \ref{lem:itemunion}, $J$ is also a local maximum, hence $\utilw(J) \geq \utilw(\adoptws(v,t+1))$, as $\adoptws(v,t+1) \subset J$. Also, $|J|> |\adoptws(v,t+1)|$, as $J$ contains at least one more item $i$. Thus as per our diffusion model $v$ at time $t$ should adopt the larger cardinality set $J$. Hence $i$ is adopted by $v$.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{ 
{\thmmonotoneSW*}
\begin{proof}
	 
	% 
	
		Assume that for any time $t\le \tau$, $\adopt_W^{\allalloc}(v,t) \subseteq \adopt_W^{\allalloc}(v,t)$. It immediately follows that $\aware_W^{\allalloc}(v,\tau) \subseteq \aware_W^{\allalloc'}(v,\tau)$. By an argument similar to that for the base case, 
		
		When allocation is changed from $\allalloc^1$ to $\allalloc^2$, the adoption set of a seed node monotonically increases. Formally speaking, $\forall v \in S^2, \adopt_W^{\allalloc^2}(v,1) \supseteq \adopt_W^{\allalloc^1}(v,1)$. Suppose this is not true. Then there exists a non-empty set $J = \adopt_W^{\allalloc^1}(v,1) \setminus \adopt_W^{\allalloc^2}(v,1)$. Since $J$ is adopted by $v$ under allocation $\allalloc^1$, we know that $\util_W(J \mid \adopt_W^{\allalloc^1}(v,1) \setminus J)\geq 0$. We also know that $\util_W(J \mid \adopt_W^{\allalloc^2}(v,1) \setminus J) = \util_W(J \mid \{\adopt_W^{\allalloc^1}(v,1) \setminus J\} \cup \{\adopt_W^{\allalloc^2}(v,1)\setminus \adopt_W^{\allalloc^1}(v,1)\})$. Further, $\{\adopt_W^{\allalloc^1}(v,1) \setminus J \cup \adopt_W^{\allalloc^2}(v,1)\setminus \adopt_W^{\allalloc^1}(v,1) \} \supseteq \adopt_W^{\allalloc^1}(v,1) \setminus J$. Hence by supermodularity of utility (property \ref{prop:sup_sm}), $\util_W(J \mid \adopt_W^{\allalloc^2}(v,1) \setminus J) \geq 0$. Hence under $\allalloc^2$, $v$ should also adopt $J$.
		
		Now from claim \ref{clm:reachable} we have that, once a node adopts an item, all nodes reachable will also adopt the same item. Since reachability is also monotone, combined with the fact that adoption at seed nodes is monotone, we have that adoption at any node is monotone. Since adoption is monotone, and by definition of adoption, every adoption has nonnegative contribution to welfare, we have,
		\begin{align*}
		\rho_W(\allalloc^2) = \sum_{v \in V} \util(\adopt_W^{\allalloc^2}(v))\\
		&\geq \sum_{v \in V} \util(\adopt_W^{\allalloc^1}(v)) \\
		= \rho_W(\allalloc^1)
		\end{align*}
		
		Since this is true in every world $W$, we can say for the expected social welfare
		\begin{align*}
		\rho(\allalloc^2) &= \mathbb{E} ( \rho_W(\allalloc^2)) \\
		& \geq \mathbb{E} ( \rho_W(\allalloc^1)) \\
		& =  \rho(\allalloc^1)
		\end{align*}
	
	% 
\end{proof}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\thmnotsubsuper*}
\vspace{-4mm}
\begin{proof} 

To prove monotonicity, we show by induction on propagation time that the social welfare in any world $W$ is monotone. The result follows upon taking expectation. Consider allocations $\allalloc \subseteq \allalloc'$ and any node $v$.  
	
	\noindent 
	\underline{Base Case}: At $t=1$, desire happens by seeding. By assumption, ${\bf I}_v^{\allalloc} \subseteq {\bf I}_v^{\allalloc'}$. Thus, $\aware_W^{\allalloc}(v,1)\subseteq \aware_W^{\allalloc'}(v,1)$, where $\aware_W^{\allalloc}(v,1)$ denotes the desire set of $v$ in world $W$ under allocation $\allalloc$. Suppose $J := \adopt_W^{\allalloc}(v,1) \setminus  \adopt_W^{\allalloc'}(v,1)$ is non-empty. From the semantics of adoption of itemsets, we have $\util_W(J\mid \adopt_W^{\allalloc}(v,1) \setminus J) \ge 0$. Now, $\adopt_W^{\allalloc}(v,1) \setminus J \subseteq \adopt_W^{\allalloc'}(v,1)$. By supermodularity of utility, $\util_W(J\mid \adopt_W^{\allalloc'}(v,1)) \ge 0$.
	Since $J \subseteq \adopt_W^{\allalloc}(v,1) \subseteq \aware_W^{\allalloc}(v,1)
	\subseteq \aware_W^{\allalloc'}(v,1)$,
	by the semantics of itemset adoption, the set $J \cup \adopt_W^{\allalloc'}(v,1)$ will be adopted by $v$ at time $1$, a contradiction to the assumption that
	$\adopt_W^{\allalloc'}(v,1)$ is the adopted itemset by $v$ at time $1$.
	
	\noindent
	\underline{Induction}: By Lemma~\ref{lem:reachable}, we know that once a node adopts an item, all nodes reachable from it in $W^E$ also adopt that item. Furthermore, reachability is monotone in seed sets. From this, it follows that $\adopt_W^{\allalloc}(v,\tau+1) \subseteq \adopt_W^{\allalloc'}(v,\tau+1)$. Define $\adopt_W^{\allalloc}(v) := \bigcup_t \adopt_W^{\allalloc}(v,t)$. By definition, an adopted itemset has a non-negative utility, so we have $\rho_W(\allalloc) = \sum_{v\in V} \util_W(\adopt_W^{\allalloc}(v))\le \sum_{v\in V} \util_W(\adopt_W^{\allalloc'}(v)) = \rho_W(\allalloc')$. This shows that the social welfare in any possible world is monotone, as was to be shown.
	
	For submodularity and supermodularity, we give counterexamples. 
	Consider a network with single node $u$ and two items $i_1$ and $i_2$. Let $\price(i_1) > \val(i_1)$ and $\price(i_2) > \val(i_2)$. However $\val(\{i_1,  i_2\}) > \price(i_1) + \price(i_2)$. Assume that noise terms are bounded random variables, i.e., $|\noise(i_j)| \le |\val(i_j) - \price(i_j)|$, $j=1,2$. 
	Thus expected individual utility of $i_1$ or $i_2$ is negative, but when they are offered together, the expected utility is positive. Now consider two seed allocations $\allalloc = \emptyset$ and $\allalloc' = \{(u,i_1)\}$. Let the additional allocation pair be $(u,i_2)$. Now 
	$\rho(\allalloc \cup \{(u,i_2)\}) - \rho(\allalloc) = 0 - 0 =0$: for $\allalloc$, no items are adopted and for $\allalloc \cup \{(u, i_2)\}$ the noise $\noise(i_2)$ cannot affect adoption decision in any possible world, so $i_2$ will not be adopted by $u$ in any world. 
	
	However, $\rho(\allalloc' \cup \{(u,i_2)\}) - \rho(\allalloc') > 0$, as under allocation $\allalloc'$, $i_1$ is not adopted by $u$ in any world, while under allocation $\allalloc' \cup \{(u,i_2)\}$, $u$ will adopt $\{i_1, i_2\}$ in every world, resulting in positive social welfare and breaking submodularity. 
	
	\eat{ 
	\end{proof}
	
	\spara{Supermodularity of social welfare}
	
	We next show that welfare is not supermodular either via another counter example.
	
	\begin{theorem}
		Social welfare is not supermodular.
	\end{theorem}
	
	\begin{proof}
	} 
	
	For supermodularity, consider a network consisting of two nodes $v_1$ and $v_2$ with a single directed edge from $v_1$ to $v_2$, with probability 1. Let there be one item $i$ whose deterministic utility is positive, i.e., $\val(i) > \price(i)$. Again, assume that the noise term $\noise(i)$ is a bounded random variable, i.e., $|\noise(i)| \le |\val(i) - \price(i)|$. 
	Now consider two seed allocations $\allalloc = \emptyset$ and $\allalloc' = \{(v_1, i)\}$. Let the additional pair be $(v_2, i)$. Under allocation $\allalloc'$, both nodes $v_1$ and $v_2$ will adopt $i$ in every possible world. Hence adding the additional pair $(v_2, i)$ does not change item adoption in any world and consequently the expected social welfare is unchanged. Thus we have,
	\vspace{-2mm}
	\begin{align*}
	\rho(\allalloc \cup \{(v_2, i)\}) - \rho(\allalloc) &= \mathbb{E}[\util(i_1)] >0  \\
	&= \rho(\allalloc' \cup \{(v_2, i)\}) - \rho(\allalloc')
	\end{align*} 
	which breaks supermodularity. 
\end{proof}

\subsection{Proofs for Block Accounting (Section \ref{sec:blocks})} \label{sec:app5}




\subsection{Proofs for Item-wise prefix preserving IMM (Section \ref{sec:PRIMM})}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{
\subsection{Proofs for Experiments (Section \ref{sec:exp})}
\begin{lemma}
The value function of Configuration 10 is supermodular.
\end{lemma}
\begin{proof}
First we show that for an itemset $A_t$ at level $t$, and an item $i \notin A_t$, $\val(i \mid A_t) \geq \val(i \mid B)$, where $B \subset A_t$ is any  subset of $A_t$. We prove this claim by induction on level.

\noindent 
	\underline{Base Case}: Let $t=1$ and $A_1$ be any singleton itemset.  Then $\val(i \mid A_1) = \val(i \mid \emptyset) + \epsilon \geq \val(i \mid \emptyset)$.
	
	\noindent 
	\underline{Induction}: Suppose the claim is true for all levels $t \leq l$. We show it holds for $t = l+1$. From our method of assigning values we have, $\val(i \mid A_{l+1}) = \max_{B_l \in \power(\allitems, l)} \{\val(i \mid B_l)\} + \epsilon$, where $\power(\allitems, l)$ is the set of all itemsets at level $l$. Thus $\val(i \mid A_{l+1}) \geq \val(i \mid B_l)$. By induction hypothesis,  $\val(i\mid B_l) \geq \val(i \mid B)$, for any 
subset $B \subset B_l$, and thus 
%we therefore have that for any $l^\prime < l+1$, 
$\val(i \mid A_{l+1}) \geq \val(i \mid B)$.
	
It then follows that  for any itemsets $B \subset A \subset \allitems$ and item $i \in \allitems \setminus A$, $\val(i \mid A) \geq \val(i \mid B)$. Hence value is supermodular. 
\end{proof}

\begin{lemma}
The value function of Configuration 10 is well defined.
\end{lemma}
\begin{proof}
We show that for an itemset $A_t$ at level $t$, $\val(i \mid A_t \setminus \{i\}) + \val(i) = \val(j \mid A_t \setminus \{j\}) + \val(j) $, for any $i , j \in A_t$.

Let $\val(A_t) = max_{k \in A_t} \{\val(A_t \setminus \{k\}) + \val(k|A_t \setminus \{k\})\} = m$. Then according to our configuration  $\val(i \mid A_t \setminus \{i\}) = m - \val(i)$. Similarly $\val(j \mid A_t \setminus \{j\}) = m - \val(j)$. Hence $\val(i \mid A_t \setminus \{i\}) + \val(i) = m - \val(i) + \val(i) = m - \val(j) + \val(j) = \val(j \mid A_t \setminus \{j\}) + \val(j)$.
\end{proof}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\eat{
\section{Additional experiments}

First we show the social welfare produced by $\RRSIM$, $\RRCIM$, $\id$, $\bd$ and $\algo$ in the configurations we omitted in Section \ref{sec:two_items}. Fig. \ref{fig:missing} (a) and (b) shows the results for Configurations $1$ and $4$ respectively. The trend is similar to Fig. \ref{fig:welfare} of Section \ref{sec:two_items}.

Fig. \ref{fig:missing} (c) shows the effect of budget skew on Configuration $7$. The three different budget distributions are same as that of Section \ref{sec:real_data}, namely (i) Uniform: each item has the same budget $50$, (ii) Large skew: one item has $82\%$ of the total budget (i.e. $500$) and the remaining $18\%$ is divided evenly among the remaining $9$ items; and (iii) Moderate skew: Budgets of the $10$ items are given by the budget vector $\bvec = [10,20,30,40,50,50,60,70,80,90]$. Again the welfare is the highest under uniform and worst under large skew, with moderate skew in between. Running time-wise uniform is the fastest and large skew is the slowest. The findings are consistent with the observation on real parameter experiment in Section \ref{sec:real_data}. With large skew, the number of seeds to be selected increases and the allocation cannot take full advantage of supermodularity.

\begin{figure*}[ht]
\begin{small}
\centering
\begin{tabular}{cc}
\hspace{-12mm}\includegraphics[height=3cm,width=.75\textwidth]{figs/pdf/appendix.pdf} &
\hspace{-5mm}\includegraphics[height=3cm,width=.35\textwidth]{figs/pdf/budgetskew.pdf}\\
%\hspace{-2mm}\includegraphics[width=.25\textwidth]{figs/pdf/tsw.pdf} \\
\hspace{-15mm} (a) Configuration 1  \hspace{30mm} (b) Configuration 4   & \hspace{6mm} (c) Effect of budget distribution on $\algo$
\end{tabular}
\caption{Additional experiments}\label{fig:missing} 
\vspace{-2mm}
\end{small}
\end{figure*}


}

==> sec-competition.tex <==

In this section, we focus on a setting where the items are mutually competing. We will present different degree of competitions, however the core essence of competition is captured by modeling user valuation for itemsets as a \emph{submodular} function. A function $f: 2^U \rightarrow \mathbb{R}$ is submodular if for any subsets $S \subset T \subset U$ and item $x \in U \setminus T$, $f(S\cup\{x\}) - f(S) \geq f(T\cup\{x\}) - f(T)$. 
The intuition is that between competing items, the marginal value-gain of an item w.r.t. a set of items decreases as the set grows, which submodularity captures well. E.g., the value gain of owning a second smart-phone drops when a user already owns a smart-phone. 
Use of submodular function to model competition is a well established practice in the economics literature (e.g., see \cite{vetta2002nash,alos2005evolutionary}). 
Like \textsection\ref{sec:complementary}, in this section we study the propagation of competing items, by combining a basic stochastic diffusion model with the utility model for item adoption. This work is still in progress. Hence we will mostly be focusing on the unique challenges that competing items poses, answers to those challenges are what we are currently working on. The summary of our research findings so far are as follows:

1. Recall that for complementary items, our objective, namely maximizing the expected social welfare was monotone. However, for competing items the same objective is not even monotone. It is neither submodular nor supermodular as well. In \textsection\ref{sec:prop_sub} we show specific counterexamples. Lack of monotone property makes designing efficient approximation algorithms even harder for competing items.

2. Unlike complementary items since the value function is submodular, the power of bundling does not exist for competing items. In fact, since the marginal gain diminishes for the value being submodular, intuitively, offering more than one item to a single node may seem counterproductive to maximizing social welfare. However we will show in section \textsection\ref{sec:challenges} that this is not always true, which in turn makes designing a simple greedy more difficult.

3. For competing items, we found that bundling is not the only challenge, the specific network structure poses a great difficulty as well. Depending on the structure the order of arrival of different items to a node differs. Hence a node may adopt an inferior item first and due to competition cannot adopt a better item later. For complementary items we proved the reachability lemma (Lemma \ref{lem:reachable}) to solve this issue. However, under competitive setting reachability lemma does not hold.

We next prove the properties of \model model under competition.

\subsection{Properties Of \model Under Submodular Valuations}\label{sec:prop_sub}

\input{sec-sub_prop}

\subsection{Approximation Algorithm}\label{sec:challenges}

\input{sec-sub_algo}


==> sec-exp-1.tex <==
\begin{table}[t!]
	\scriptsize
	\centering
	\begin{tabular}{rccccc}
	 & \flix & \dbBook & \dbMovie & \twit \\ \hline
	{ \# nodes}			& $12.9$K & $23.3$K	& $34.9$K & $41.7$M  \\ 
	{ \# edges} 		& $192$K  & $141$K	& $274$K & $1.47$G   \\ 
	 { avg. degree}     & $14.8$ & $6.5$ & $7.9$	& $70.5$  \\ 
	 { type}            &  undirected  & directed & directed  &  directed   \\ \hline
	\end{tabular}
	\caption{Network Statistics}
	 \label{tab:datasets}
\end{table}
\subsection{Experiment Setup}

\begin{figure*}[ht]
\begin{small}
\hspace*{-30mm}\includegraphics[height=3.5cm,width=1.32\textwidth]{figs/pdf/sw1.pdf}
\begin{tabular}{cccc}
%\hspace{-6mm}\includegraphics[width=.25\textwidth]{figs/pdf/flxt.pdf} &
%\hspace{-2mm}\includegraphics[width=.25\textwidth]{figs/pdf/dbt.pdf} &
%\hspace{-2mm}\includegraphics[width=.25\textwidth]{figs/pdf/dmt.pdf} &
%\hspace{-2mm}\includegraphics[width=.25\textwidth]{figs/pdf/twt.pdf} \\
 \hspace{2mm} (a) Configuration $2$  \hspace{26mm} &  (b) Configuration $3$ \hspace{23mm} &  (c) Configuration $5$ \hspace{21mm} &  (d)  Configuration $6$
\end{tabular}
\caption{Expected social welfare in four configurations (on \dbMovie network)} \label{fig:welfare}
\vspace{-3mm}
\end{small}
\end{figure*}

 
We perform extensive experiments on four real social networks.
	% to evaluate our algorithms: \flix, \douban, and \lastfm. 
% and also conduct scalability tests on larger synthetic graphs.
We first experiment with synthetic utility (value and price) functions. 
To experiment with real utility functions, we learn the values and noise distributions of items from the bidding data of \ebay; %, using the method 
%proposed by Jiang et. al. in \cite{Albertbidding07}. We 
and obtain item prices from \cgl and \fb groups. All experiments are performed on a Linux machine with Intel Xeon $2.6$ GHz CPU and $128$ GB RAM.

\spara{6.1.1 Networks} 
Table \ref{tab:datasets} summarizes the networks and their characteristics. 
\flix is mined in \cite{lu2015} from a social movie site and a strongly connected component is extracted. \db is a Chinese social network~\cite{yuan2013we}, where users rate  books, movies, music, etc.
In \cite{lu2015} all movie and book ratings of the users in the graph are crawled separately to derive two datasets from book and movie ratings: \dbBook and \dbMovie. \twit is one of the largest network datasets, which is publicly available at \cite{twitter}. 


\spara{6.1.2 Algorithms compared}
We compare $\algo$ against four baselines -- $\RRSIM$, $\RRCIM$, $\id$ and $\bd$. $\RRSIM$ and $\RRCIM$, proposed in \cite{lu2015}, are two state-of-the art algorithms designed for complementary products in the context of IM. However, they work only with two items. Extending the \comic framework and the $\RRSIM$ and $\RRCIM$ algorithms for more than two items is highly non-trivial as that requires dealing with a NLA with exponentially many states. 
Hence in comparing the performance of $\algo$ against $\RRSIM$ and $\RRCIM$, we  limit the number of items to two. Later we experiment with more than two items. Below, by deterministic utility of an itemset $I$, we mean $\val(I) - \price(I)$, i.e., its utility with the noise term ignored. 

{\bf 6.1.2.1 \comic baselines.} For two items $\ia$ and $\ib$, given seed set of item $\ib$ (resp. $\ia$), $\RRSIM$ (resp. $\RRCIM$) finds seed set of item $\ia$ (resp. $\ib$) such that expected number of adoptions of $\ia$ is maximized. Initial seeds of $\ib$ (resp. $\ia$) is chosen using IMM \cite{tang15}. 

{\bf 6.1.2.2 Item-disjoint.} Our next baseline is $\id$, which allocates only one item to every seed node. Given the set of items $\allitems$, $\id$ finds $\sum_{i \in \allitems} b_i$ nodes, say $L$,  using IMM \cite{tang15}, where $b_i$ is the budget of item $i$. Then it visits items in $L$ in non-increasing order of budgets, assigns item $i$ to first $b_i$ nodes and removes those $b_i$ nodes from $L$. By explicitly assigning every item to different seeds, $\id$ does not leverage the effect of supermodularity. However it benefits from the \textit{network effect}: since the utilities are supermodular, if more neighbors of a node adopt some item, it is more likely that the node will also adopt an item. Thus, when individual items have positive utility and hence can be adopted and propagate on their own, by choosing more seeds,  $\id$ makes use of the network effect to encourage more adoptions.

{\bf 6.1.2.3 Bundle-disjoint.} The last baseline, $\bd$, aims to leverage both supermodularity and network effect. It first orders the items $\allitems$ in non-increasing budget order and determines successively minimum sized subsets with non-negative deterministic utility, maintaining these subsets (``bundles'') in a list. Items in each bundle $B$ are allocated to a new set of $b_B := {\it min\/}\{b_i\mid i\in B\}$ seed nodes. The budget of each item in $B$ is decremented by $b_B$, and items with budget $0$ are removed. When no more bundles can be found, we revisit each item $i$ with a positive unused budget and repeatedly allocate it to the seeds of the first existing bundle $B$ which does not contain $i$. If $b_B > b_i$ (where $b_i$ is the current budget of $i$ after all deductions), then the first $b_i$ seeds from the seed set of $B$ are assigned to $i$. If an item $i$ still has a surplus budget, we select $b_i$ fresh seeds using IMM and assign them to $i$.
\begin{table}[t!]
\scriptsize
\centering
\caption{Two item configurations}
\label{tab:configs}
\begin{tabular}{|c|c|c|c|c|l|}
\cline{1-6}
                                                                      No     & Price                                                                                           & Value                                                               & Noise                                                                                                             & GAP                                                                                & Budget     \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\ \\ 1 \\ \ \end{tabular}}        & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}} \ \\ \ \\ \ \\ \ \\ \ \\ $\ia = 3$\\ $\ib = 4$\\ $\{\ia,\ib\} = 7$ \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\ia = 1.7$\\ $\ib = 2.7$ \\ $\{\ia,\ib\} = 8$ \end{tabular}} & \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}} \ \\ \ \\ \ \\ \ \\ \ \\ $\ia : N(0,1)$ \\ $\ib : N(0,1)$ \\ $\{\ia,\ib\} : N(0,2)$ \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} $\qao = 0.1$\\ $\qbo = 0.1$\\ $\qab = 0.99$ \\ $\qba = 0.99$ \end{tabular}} & Uniform    \\ \cline{1-1} \cline{6-6} 
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\ \\ 2 \\ \ \end{tabular}}        &                                                                                                                      &                                                                                          &                                                                                                                                        &                                                                                                         & Nonuniform \\ \cline{1-1} \cline{3-3} \cline{5-6} 
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\ \\ 3 \\ \ \end{tabular}} &                                                                                                                      & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\ia = 3$\\ $\ib = 4$ \\ $\{\ia,\ib\} = 8$\end{tabular}}     &                                                                                                                                        & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\qao = 0.5$\\ $\qbo = 0.5$\\ $\qab = 0.84$ \\ $\qba = 0.84$\end{tabular}} & Uniform    \\ \cline{1-1} \cline{6-6} 
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\ \\ 4 \\ \ \end{tabular}} &                                                                                                                      &                                                                                          &                                                                                                                                        &                                                                                                         & Nonuniform \\ \cline{1-1} \cline{3-3} \cline{5-6} 
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\ \\ 5 \\ \ \end{tabular}}                                                    &                                                                                                                      & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\ia = 3$\\ $\ib = 3$ \\ $\{\ia,\ib\} = 8$\end{tabular}}     &                                                                                                                                        & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$\qao = 0.5$\\ $\qbo = 0.16$\\ $\qab = 0.98$ \\ $\qba = 0.84$\end{tabular}} & Uniform    \\ \cline{1-1} \cline{6-6} 
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\ \\ 6 \\ \ \end{tabular}}                                                    &                                                                                                                      &                                                                                          &                                                                                                                                        &                                                                                                         & Nonuniform \\ \hline
\end{tabular}
\end{table} 

\begin{figure*}[ht]
\begin{small}
\hspace*{-30mm}\includegraphics[height=3.5cm,width=1.32\textwidth]{figs/pdf/test.pdf}
\begin{tabular}{cccc}
%\hspace{-6mm}\includegraphics[width=.25\textwidth]{figs/pdf/flxt.pdf} &
%\hspace{-2mm}\includegraphics[width=.25\textwidth]{figs/pdf/dbt.pdf} &
%\hspace{-2mm}\includegraphics[width=.25\textwidth]{figs/pdf/dmt.pdf} &
%\hspace{-2mm}\includegraphics[width=.25\textwidth]{figs/pdf/twt.pdf} \\
 \hspace{-5mm} (a) \flix  \hspace{27mm} &  (b) \dbBook \hspace{27mm} &  (c) \dbMovie \hspace{25mm} &  (d)  \twit
\end{tabular}
\caption{Running times of $\algo$, $\RRSIM$, $\RRCIM$, $\id$ and $\bd$ (on Configuration $3$)} \label{fig:time}
\vspace{-3mm}
\end{small}
\end{figure*}

\begin{figure*}[ht]
\begin{small}
\hspace*{-30mm}\includegraphics[height=3.5cm,width=1.32\textwidth]{figs/pdf/mem.pdf}
\begin{tabular}{cccc}
%\hspace{-6mm}\includegraphics[width=.25\textwidth]{figs/pdf/flxt.pdf} &
%\hspace{-2mm}\includegraphics[width=.25\textwidth]{figs/pdf/dbt.pdf} &
%\hspace{-2mm}\includegraphics[width=.25\textwidth]{figs/pdf/dmt.pdf} &
%\hspace{-2mm}\includegraphics[width=.25\textwidth]{figs/pdf/twt.pdf} \\
 \hspace{-5mm} (a) \flix  \hspace{27mm} &  (b) \dbBook \hspace{27mm} &  (c) \dbMovie \hspace{25mm} &  (d)  \twit
\end{tabular}
\caption{Memory counsumption of $\algo$, $\RRSIM$, $\RRCIM$, $\id$ and $\bd$ (on Configuration $3$)} \label{fig:mem}
\vspace{-3mm}
\end{small}
\end{figure*}


\spara{6.1.3 Parameters}
Following previous work \cite{tang14,tang15,Huang2017,Nguyen2016} we set the  probability of edge $e = (u,v)$ to $1/\ind(v)$. 
Unless otherwise specified, we use $\epsilon = 0.5$ and $\ell = 1$ as our default values for all five methods as recommended in \cite{tang15,lu2015}. %Further we are the first to introduce the concept of utility in the context of IM. 
The \comic algorithms $\RRSIM$ and $\RRCIM$ use GAP parameters (adoption probabilities) to model the interaction between items. We explain how the corresponding GAP parameters can be simulated within the \model framework using utilities, which we use in our comparison.

Let $\ia$ and $\ib$ be the two items. Suppose the desire set of a node $u$ only has item $\ia$. The condition that $u$ adopts $\ia$ is
	$\val(\ia)-\price(\ia)+\noise(\ia) \ge 0$.
Thus the GAP parameter $\qao$ is given by:
\begin{equation*}
\qao = \Pr[ \val(\ia)-\price(\ia)+\noise(\ia) \ge 0] = \Pr[ \noise(\ia) \ge \price(\ia) - \val(\ia)].
\end{equation*}

Now suppose $\ia$ has been adopted by $u$, and $\ib$ enters the desire set. 
The GAP parameter $\qba$ is the probability of adopting $\ib$ given that $\ia$ has been adopted. So we have
\begin{align*}
\qba & = \Pr[\val(\{\ia,\ib \})-\price(\ia) - \price(\ib) + \noise(\ia) + \noise(\ib) \ge \\
	& \ \  \hspace*{2ex}  \val(\ia) - \price(\ia) + \noise(\ia)
\mid \noise(\ia) \ge \price(\ia) - \val(\ia) ] \\
 & = \Pr[  \noise(\ib) \ge \price(\ib) - (\val(\{\ia,\ib \} ) - \val(\ia)) \mid \noise(\ia) \ge \\ 
 & \ \hspace*{2ex} \price(\ia) - \val(\ia) ].
\end{align*}
Since noise $\noise(\ib)$ is independent of noise $\noise(\ia)$, we can remove the above condition in the
	conditional probability, and obtain
\begin{equation*}
\qba =  \Pr\{  \noise(\ib) \ge \price(\ib) - (\val(\{\ia,\ib \} ) - \val(\ia))\}.
\end{equation*}
The other two GAP parameters, $\qbo$ and $\qab$ can be obtained similarly.
To summarize, we have
% 
\begin{align} \label{eq:gaputil}
\qao & = \Pr[ \noise(\ia) \ge \price(\ia) - \val(\ia)], \nonumber \\ 
\qab & = \Pr[  \noise(\ia) \ge \price(\ia) - (\val(\{\ia,\ib \} ) - \val(\ib))], \\ \nonumber
\qbo & = \Pr[ \noise(\ib) \ge \price(\ib) - \val(\ib)], \\ \nonumber
\qba & =  \Pr[  \noise(\ib) \ge \price(\ib) - (\val(\{\ia,\ib \} ) - \val(\ia))].
\end{align}


\subsection{Experiments on two items} \label{sec:two_items}
\begin{figure*}[h!t!]
\begin{small}
%\centering
\hspace*{-25mm}\includegraphics[height=3.5cm,width=1.32\textwidth]{figs/pdf/synsw.pdf} 
\begin{tabular}{cccc}
 \hspace*{5mm} (a) Configuration $7$ & \hspace*{25mm} (b) Configuration $8$   & \hspace*{21mm} (c) Configuration $9$  & \hspace*{23mm} (d) Configuration $10$
\end{tabular}
\caption{Expected social welfare on four configurations}\label{fig:synsw} 
\vspace{-2mm}
\end{small}
\end{figure*}
To enable comparison with the \comic algorithms $\RRSIM$ and $\RRCIM$, in our first set of experiments, we limit number of items to two. We explore six different configurations corresponding to the choice of the values, prices, noise distribution parameters, and item budgets (see Table \ref{tab:configs}). While \model does not assume any specific distribution for noise, in our experiments we use a gaussian distribution for illustration.


Configurations $1$ and $2$ signify a utility setting where the individual items $\ia$ and $\ib$ have negative deterministic utility, while $\{\ia, \ib\}$ has a non-negative utility. Notice under this setting, $\algo$ and $\bd$ are equivalent, because the only possible bundle is $\{\ia, \ib\}$. In Configurations  $3$ and $4$, individual items have non-negative deterministic utility. In this setting $\id$ and $\bd$ are equivalent. Finally, in Configurations $5$ and $6$ one item has a negative deterministic utility while the other item has a non-negative one. In this setting, again $\algo$ and $\bd$ are equivalent.

For every parameter setting, we consider two budget settings, namely \textit{uniform} (e.g., Configuration $1$) and \textit{non-uniform} (resp. Configuration $2$). In case of uniform budget, both items have same the same budget $k$, where $k$ is varied from $10$ to $50$ in steps of $10$. For non-uniform budget, $\ia$'s budget is fixed at $70$, and $\ib$'s budget is varied from $30$ to $110$ in steps of $20$.

\spara{6.2.1 Social Welfare}
We compare the social welfare achieved by all algorithms on all six configurations. However, in Fig. \ref{fig:welfare}, we show the results only for \dbMovie network on Configurations $2,3,5$ and $6$. The trend of the results is similar on other networks and configurations, hence they are omitted. In terms of social welfare, $\algo$ outperforms all the baselines consistently. The social welfare produced by $\id$ and $\bd$ depends on the specific configurations. E.g., when individual items have negative deterministic utility (Configuration $2$), $\id$ produces $0$ expected social welfare as expected (Fig. \ref{fig:welfare}(a)). Even when the welfare is non-zero for $\id$ %(similarly when $\bd$ and $\algo$ are not equivalent), 
$\algo$ achieves an expected social welfare which is upto $5$ times higher (Fig. \ref{fig:welfare}(d)). A similar remark applies when $\bd$ and $\algo$ are not equivalent (e.g., Fig. \ref{fig:welfare}(b)). Further, notice that $\RRSIM$ and $\RRCIM$ produce welfare similar to $\algo$. It follows from %what is noted in 
Table $4$ of \cite{lu2015arxiv} that under this configuration, $\RRSIM$ and $\RRCIM$ end up copying the seeds of other item. Hence their allocations are similar to $\algo$.  However, as shown next, $\algo$ runs much faster than the other two and unlike them, easily supports more than two items, which makes $\algo$ more usable in practice for multiple items over large networks.

\spara{6.2.2 Running time}
We study the running time of all algorithms using Configuration $1$. The results are shown in Fig. \ref{fig:time}. As can be seen, $\algo$ and $\bd$ are equivalent and hence have the same running time. However, $\algo$ significantly outperforms all other baselines on every dataset. $\RRSIM$ and $\RRCIM$ are particularly slow. In fact, on the large $\twit$ network, they could not finish even after $6$ hours. We had to time them out, hence they are omitted from Fig. \ref{fig:time}(d). In comparison with the baselines, $\algo$ is upto $5$ orders of magnitude faster than $\RRCIM$ and upto $1.5$ times than $\id$. Running times on other configurations show a similar trend, and are omitted. 

\subsection{More than two items}\label{sec:mtsyn}

\begin{figure}[ht]
\begin{minipage}[b]{0.45\linewidth}
%\centering
\includegraphics[width=1.28\textwidth]{figs/pdf/numvstime.pdf}
\caption{Effect of number of items}
\label{fig:multiitemrun}
\end{minipage}
\hspace{0.5cm}
\begin{minipage}[b]{0.45\linewidth}
%\centering
\begin{small}
\begin{tabular}{|c|c|c|} \hline
  No & Value & Budget \\ \hline 
  7 & Additive & Uniform \\ \hline
  8 & Cone-max & Non-uniform \\ \hline
  9 & Cone-min & Non-uniform \\ \hline
  10 & Level-wise & Uniform \\ \hline
  \end{tabular}
  
\end{small}
  \caption{Multiple item configurations.}
\label{tab:configs-2+items}
\end{minipage}
\end{figure}


\eat{
\begin{figure}
\begin{floatrow}
\ffigbox{%
	\includegraphics[width=.58\textwidth]{figs/pdf/numvstime.pdf}
}{%
  \caption{Effect of number of items} \label{fig:multiitemrun}
}
\capbtabbox{%
\scriptsize
  \begin{tabular}{|c|c|c|} \hline
  No & Value & Budget \\ \hline 
  7 & Additive & Uniform \\ \hline
  8 & Cone-max & Non-uniform \\ \hline
  9 & Cone-min & Non-uniform \\ \hline
  10 & Level-wise & Uniform \\ \hline
  \end{tabular}
}{%
  \caption{Multiple item configurations.} \label{tab:configs-2+items}
}
\end{floatrow}
\end{figure}
}

\spara{6.3.1 The configurations}  
Having established the superiority of $\algo$ for two items, we now consider more than two items. 
Recall that $\RRSIM$ and $\RRCIM$ cannot work with more than two items, so we confine our baselines to $\id$ and $\bd$. 
% 
\eat{Again several interesting configurations can be obtained based on the budgets and the utilities of the items. We devise four such specific configurations. Unless otherwise stated, in every configuration the number of items is assumed to be $10$.
} 
% 
We gauge the performance of the algorithms on social welfare and running time. We also study the effect of budget distribution on social welfare. We design four configurations corresponding to the choice of budget and utility (see Table~\ref{tab:configs-2+items}). For all configurations, we sample noise terms from $N(0,1)$. Price and value are set in such a way as to achieve certain shapes for the set of itemsets in the lattice that have a positive utility (see below). 


{\bf 6.3.1.1 Configurations 7-9.} Configuration 7 is the simplest one for multiple items: every item has the same budget; price and value are set such that every item has the same utility of $1$ and utility is additive. Thus, by design, this configuration gives minimal advantage to any algorithm that tries to leverage supermodularity.  The next two configurations (8 and 9) model the situation where a single ``core'' item is necessary in order to make an itemset's utility positive. E.g., a smartphone may be a core item, without which its accessories do not have a positive utility. We set the core item's utility to $5$. The addition of any other item increases the utility by $2$. Thus, all supersets of the core item have a positive utility, while all other subsets have a negative utility. Thus, the set of subsets with positive utility forms a ``cone'' in the itemset lattice. In Configuration 8 (resp. 9), the core item is the item with maximum (resp. minimum) budget. Finally, we design a more general configuration where the set of itemsets with positive utility forms an arbitrary shape. Specifically we design Configuration 10 as follows. 

{\bf 6.3.1.2 Configuration 10.} We consider the itemset lattice, with level $t$ having subsets of size $t$. We randomly set the prices and values of items in level 1 such that a random subset of items have a non-negative utility. Let $A_t$ be any itemset at level $t > 1$ and $i \in A_t$ any item. We choose a value uniformly at random, $\epsilon \sim U[1,5]$, and define 
%
\begin{equation}\label{eq:mar_val}
\val(i|A_t \setminus \{i\}) = max_{B \in \power(A_t \setminus \{i\}, t-2)} \{\val(i|B) + \epsilon\}
\end{equation}
% 
where $\power(A, q)$ denotes the set of subsets of $A$ of size $q$. That is, the marginal gain of an item $i$ w.r.t. $A_t\setminus \{i\}$ is set to be the maximum marginal gain of $i$ w.r.t. subsets of $A_t$ of size $t-2$, plus a randomly chosen boost ($\epsilon$). 
E.g., let $A_4=\{i,j,k,l\}$, $t = 4$ then, $\val(i|\{j,k,l\}) = max\{\val(i|\{j,k\}), \val(i|\{k,l\}), \val(i|\{j,l\})\} + \epsilon$.

Recall that the value computation proceeds level-wise starting from level $t=0$. Thus, for any itemset $A_t$ in Equation \ref{eq:mar_val}, $\val(i|B)$ for subsets $B$ is already defined. 

Finally, we set 
$\val(A_t) = max_{i \in A_t} \{\val(A_t \setminus \{i\}) + \val(i|A_t \setminus \{i\})\}$. We can show that this way of assigning values ensures that the value function is well-defined and supermodular \cite{fullpaper}.

\spara{6.3.2 Social welfare}
First, we study the social welfare achieved by the algorithms, in each of the the above configurations, with the total budget varied from $500$ to $1000$ in steps of $100$. For Configurations 7 and 10, we set the budget uniformly for every item. %Thus when total budget is $500$ every item has a budget of $50$. 
For other configurations, the max budget is set to $20\%$ of the total budget,  min budget to $2\%$, and the remaining budget is split uniformly. The results are shown in Fig. \ref{fig:synsw}. Under Configurations 8 and 9, $\algo$ and $\bd$ produces the same allocation, hence the welfare is the same. However in general $\algo$ outperforms every baseline in all the four configurations by producing welfare upto $4$ times higher than baselines.


\spara{6.3.3 Running time vs number of items}
Next, we study the effect of the number of items on the running time of the algorithms. For this experiment, we use Configuration 7. We set the budget of every item to $k=50$ and vary the number of items $s$, from $1$ to $10$. Fig. \ref{fig:multiitemrun} shows the running times on the $\twit$ dataset. As the number of items increases the number of seed nodes to be selected for $\id$ and $\bd$ increases. Notice both $\id$ and $\bd$ select the same number of seeds, which is $k \times s$. $\id$ selects it by one invocation of IMM, with budget $ks$, while $\bd$ invokes IMM $s$ times with budget $k$ for every invocation. So their overall running times differ.  By contrast, the running time of $\algo$ only depends on the maximum budget and is independent of the number of items. E.g., when number of items is $10$, $\algo$ is about $8$ times faster than $\bd$ and $2.5$ times faster than $\id$. 

\eat{
\spara{6.3.4 Effect of budget distribution}
Our final experiment in this section is not a comparison of algorithms. Rather, it studies the following question. Suppose we have a fixed total budget which we must divide it up among various items. How would the social welfare and running time vary for different splits? Since we have seen that in terms of social welfare $\algo$ dominates all baselines, we use it to measure the welfare. 
We adapt Configuration 7: keeping the utility additive with positive utility for each individual items, given a total budget of $500$, we split it across $10$ items. Specifically, we consider three different budget distributions, namely (i) Uniform: each item has the same budget $50$, (ii) Large skew: one item has $82\%$ of the total budget and the remaining $18\%$ is divided evenly among the remaining $9$ items; and (iii) Moderate skew: Budgets of the $10$ items are given by the budget vector $\bvec = [10,20,30,40,50,50,60,70,80,90]$.

Fig. \ref{fig:multiitemskew} shows the expected social welfare and the running time of $\algo$ under the three budget distributions. The welfare is the highest under uniform and worst under large skew, with moderate skew in between. Running time shows the opposite trend, with uniform being the fastest and large skew being the slowest. The findings are consistent with the observation that with large skew, the number of seeds to be selected increases and the allocation cannot take advantage of supermodularity.  
}
\eat{ 
When the distribution is uniform $\algo$ performs the best, even for arbitrary budget the social welfare does not reduce much. However when budget is skewed the social welfare significantly reduces. In contrast, the running time is highest for the skewed budget and lowest when budget is uniform. This is because that the number of seed nodes to be selected is $491$ for skewed, as compared to $50$ for uniform budget.
} 


\subsection{Experiment with real parameters} \label{sec:real_data}
In this section, we conduct experiments on parameters (value, price, and noise) learned from real data. We consider the following 5 items: (1) Playstation $4$, $500$ GB console, denoted $\ps$, (2) Controller of the Playstation, denoted $\cs$, and (3-5) Three different games compatible with $\ps$, denoted $\ga$, $\gb$ and $\gc$ respectively. We next describe the method by which we learn their parameters from real data. 



\begin{figure*}[h!t!]
\begin{small}
\centering
\begin{tabular}{cc}
\hspace{-12mm}\includegraphics[height=3cm,width=1.05\textwidth]{figs/pdf/real_sw_t.pdf} &
\hspace{-63mm}\includegraphics[height=3cm,width=.31\textwidth]{figs/pdf/real_skew.pdf}\\
%\hspace{-2mm}\includegraphics[width=.25\textwidth]{figs/pdf/tsw.pdf} \\
\hspace{-55mm} (a) Social welfare  \hspace{30mm} (b) Running time   & \hspace{-70mm} (c) Effect of budget distribution on $\algo$
\end{tabular}
\caption{Results on real dataset}\label{fig:real} 
\vspace{-2mm}
\end{small}
\end{figure*}

\spara{6.4.1 Learning the price, value, and noise}
Predicting a user's bid in an auction is a widely studied problem in auction theory. Jian et al. \cite{Albertbidding07} showed that learning user's valuations of items improves the prediction accuracy. Given bidding history of an item, their method learns a value distribution of the item, by taking into account hidden/unobserved bids. %in the process. 
Their experiments show that their method significantly improves upon the existing baselines in accurately learning valuation and estimating the bids.

We use their method to learn the values of itemsets from bidding histories. Recall that in our model we do not use value as a random variable, instead using noise to model the randomness in valuations. Hence we take the mean of the learned distribution to be the value and the noise is set to have $0$ mean and the same variance as the learnt distribution. While \model does not assume specific noise distributions, we fit a gaussian distribution to noise for concreteness. 
\eat{ 
As noted in \cite{Albertbidding07}, although the learnt value functions are close to gaussian distributions, they do not exactly follow the exact gaussian shape (e.g., see Fig. $6$ of \cite{Albertbidding07}). To mitigate that we
} 
We take $10,000$ independent random samples from the learnt distribution and fit a gaussian distribution on the sampled values.

\begin{table}[t!]
	\scriptsize
	\centering
	\begin{tabular}{|c|c|c|c|c|}
 \hline
 Itemset & Price & Value & Noise & Clickable eBay bidding link \\
 \hline
 $\{\ps\}$ & $260$ & $213$ & $N(0,4)$ & \href{https://www.ebay.com/itm/SONY-PS4-Console-500-GB-PlayStation-4-Original-model-CUH-1001A/163109688891?epid=1465054404&hash=item25fa18563b:g:LK4AAOSwNrFbK~Nt}{link}  \\
 \hline
 $\{\ps,\cs\}$ & $280$ & $220$ & $N(0,6)$ & \href{https://www.ebay.com/itm/Sony-Playstation-4-500GB-with-2-controllers/232815848520?hash=item3634e7ec48:g:EqEAAOSwhEVbICmq}{link}  \\
 \hline
 $\{\ps,\ga,\gb,\gc\}$ & $275$ & $258$ & $N(0,4)$ & \href{https://www.ebay.com/itm/Sony-PlayStation-4-500GB-Black-Console-With-3-Games-Included-Working/153067119731?epid=167317351&hash=item23a382e473:g:KRcAAOSwukVbKI1c}{link}  \\
 \hline
 $\{\ps,\ga,\gb,\cs\}$ & $290$ & $292.5$ & $N(0,5)$ & \href{ https://www.ebay.com/itm/PlayStation-4-Slim-500GB-Uncharted-4-Bundle-Console-PS4-NBA2k18-Fast-Furious-7/253697656780?hash=item3b118f07cc:g:wZUAAOSwDrVbKJcG}{link}  \\
 \hline
 $\{\ps,\ga,\gb,\gc,\cs\}$ & $295$ & $302$ & $N(0,7)$ & \href{ https://www.ebay.com/itm/Sony-PlayStation-4-Game-Console-Bundle/232813673454?hash=item3634c6bbee:g:J14AAOSwf5BbKqhq}{link}  \\
 \hline
	\end{tabular}
	\caption{Learned parameters}
	 \label{tab:realp}
\end{table}

We mine the bidding histories of different itemsets from \ebay. The prices of items are mined from \cgl and \fb groups of used products. Since the items bade in \ebay are typically used products, to match them with the right price information, we use \cgl and \fb groups. 

The price obtained for $\ps$ is C\$$260$, for $\cs$ is C\$$20$ and for $\ga,\gb$ and $\gc$ it is C\$$5$ each. We show some of the learned parameters of different itemsets and links to the corresponding bidding histories used in learning, in Table \ref{tab:realp}. We describe the parameters of the rest of the itemsets here. Firstly, any of $\cs,\ga,\gb,\gc$, without the core item $\ps$, is useless. Hence values of those items are set to $0$. Secondly, we did not find any bidding record for an itemset consisting of $\ps,\cs$ and a single game. This is perhaps because typically owners of $\ps$ own multiple games and while selling they sell all the games together with $\ps$. Hence, we consider the itemset with $\ps,\cs$ and a single game to have negative deterministic utility. However, as the table shows, itemsets with $\ps,\cs$ and two games have non-negative deterministic utility. Finding the bidding history for the exact same games is difficult, so since games $g_1$--$g_3$ are priced similarly and valued similarly by users, we assume that any itemset with $\ps,\cs$ and any two games has the same utility as shown in the fourth row of Table \ref{tab:realp}. Lastly, notice that the only itemsets that have positive deterministic utility are itemsets with $\ps,\cs$ and at least two games. All other itemsets including the singleton items, have negative deterministic utility. Consequently, we know that the allocation produced by $\id$ will have $0$ expected social welfare, so we omit $\id$ from our experiments, discussed next. 

\spara{6.4.2 Results}
As stated 
\eat{ 
earlier since individual item has negative deterministic utility, we compare $\algo$ against $\bd$ in the following experiments.
} 
above, we compare $\algo$ with $\bd$ in the following experiments. First we study the effect of total budget on the expected social welfare produced. Given a total budget, we assign $30\%,30\%,20\%,10\%,10\%$ of that to $\ps,\cs,\ga,\gb,\gc$ respectively. Then we vary the total budget from $100$ to $500$ in steps of $100$. Fig. \ref{fig:real}(a) shows the welfare: as can be seen, $\algo$ outperforms $\bd$ in both high and low budgets. In fact with higher budget, $\algo$ produces welfare $2$ times more than $\bd$. Next we report the running time of the two algorithms in Fig. \ref{fig:real}(b). Since $\bd$ makes multiple calls to IMM, its running time is $1.5$ times higher than $\algo$.

Our final experiment is not a comparison of algorithms. Rather, it studies the following question. Suppose we have a fixed total budget which we must divide it up among various items. How would the social welfare and running time vary for different splits? Since we have seen that in terms of social welfare $\algo$ dominates all baselines, we use it to measure the welfare. 
Given a total budget of $500$, we split it across $10$ items following three different budget distributions, namely (i) Uniform: each item has the same budget $50$, (ii) Large skew: one item has $82\%$ of the total budget and the remaining $18\%$ is divided evenly among the remaining $9$ items; and (iii) Moderate skew: Budgets of the $10$ items are given by the budget vector $\bvec = [10,20,30,40,50,50,60,70,80,90]$.

Fig. \ref{fig:real}(c) shows the expected social welfare and the running time of $\algo$ under the three budget distributions. The welfare is the highest under uniform and worst under large skew, with moderate skew in between. Running time shows the opposite trend, with uniform being the fastest and large skew being the slowest. The findings are consistent with the observation that with large skew, the number of seeds to be selected increases and the allocation cannot take full advantage of supermodularity.


==> sec-model-laks.tex <==

%%%%%%%%%%%%%%%%%%%%%% 
\eat{ 
%and \comic models.}\label{sec:IC} 
The independent cascade (IC) model~\cite{kempe03} assumes that there is a single item (e.g., idea or product) propagating through the network. 
%We use ``product'' in our description of the model for concreteness and simplicity. 
An instance of the IC model consists of a directed graph $G=(V,E,p)$ where % with nodes $V$, edges $E\subset V\times V$, and function 
$p:E \to [0,1]$ is an assignment of influence probabilities to edges, %specifies pairwise influence probabilities between nodes,
and a seed set $S\subset V$.
For convenience, we use $p_{u,v}$ for $p(u,v)$.
At time $t = 0$, the seeds are {\em active} and all other nodes are {\em inactive}.
Propagation proceeds in discrete time steps.
At time $t > 0$, every node $u$ that became active at $t-1$ makes one attempt to activate each of its inactive out-neighbors $v$, i.e., it tests 
whether the edge $(u,v)$ is ``live'' or ``blocked''.
The out-neighbor $v$ becomes active at $t$ w.p. $p_{uv}$. 
The propagation ends when no new nodes become active. 
} 
%%%%%%%%%%%%%%%%%%% 

%%%%%%%%%%%%%%%%%%% 
\eat{ 
\comic extends IC for multiple items. The set of items be $\allitems$. To enable arbitrary adoption decision making for items in $\allitems$, \comic~\cite{lu2015} introduces a separate decision-making automata, called node level automaton (NLA) at every individual node. Edges become live following IC like process. However, a node does not necessarily become active when one of its live in-neighbor becomes active at a previous state. Rather moves to a state based on its current state and NLA. The state transition of an NLA is governed by a set of global adoption probability (GAP) parameters. Finally \comic puts an explicit order on the items arriving simultaneously at an user. Parameter $\pi_v$ denotes the order for node $v$.
} 
%%%%%%%%%%%%%%%%%%%% REMOVING DESCRIPTION OF COMIC INCLUDE A BRIEF SUMMARY IN THE RELATED WORK SECTION. 

In this section, we describe a novel model called \emph{economically postulated independent cascade} model (\model for short) that combines the diffusion dynamics of the classic IC model with an item adoption framework where decisions are governed by utility. 
 
\subsection{Utility based adoption}

\eat{ 
Whereas NLA was necessary to capture users' decision making process in presence of multiple items, it is a postulatory contrivance. On the other hand, } 

%RETAIN THE ORIGINAL UNCOMMENTED VERSION OF THIS PARAGRAPH FOR THE ARXIV VERSION. 
Utility is a widely studied concept in economics \cite{myerson1981optimal,hirshleifer1978,feige-vondrak-demand-2010} and is commonly used to model item  adoption decisions by users. 
%We next briefly review utility and provide the  specific formulation we use in this paper. 
We refer the reader interested in %more 
general definitions related to utility to \cite{rasmusen1994,nisan2007,feige-vondrak-demand-2010}.

%\subsubsection{Utility of items}

We let $\allitems$ denote a finite universe of items. The utility of a set of items $\itemset \subseteq \allitems$ for a user is the pay-off of $I$ to the user and 
	depends on aggregate effect of three components: the price $\price$ that the user needs to pay, the valuation $\val$ that the user has for $\itemset$ and a random noise term $\noise$, used to model the uncertainty in our knowledge of the user's valuation on items, where $\price$, $\val$ and $\noise$ are all set functions over items.
%
For an item $i \in \allitems$, $\price(i) > 0$ denotes its price. We assume that price is additive, i.e., for an itemset $\itemset \subseteq \allitems$, $\price(I) = \sum_{i \in \itemset} \price(i)$. 
%
Although \model can handle any generic valuation function, in this paper we focus on complementary products, and hence assume that $\val$ is supermodular
(definition in \textsection\ref{sec:related}). 
%RETAIN THE DEF. FOR THE ARXIV VERSION. 
% 
\eat{
: for two itemsets $I_1$ and $I_2$ such that $I_1 \subseteq I_2 \subset \allitems$, and for $i \in \allitems \setminus I_2$, we have $\val(I_1 \cup \{i\}) - \val(I_1) \leq \val(I_2 \cup \{i\}) - \val(I_2)$.} 
We also assume $\val$ is monotone since it is a natural property for values. 
%\weic{I think we need $\val$ to be monotone, right?}
%
%In order to model the uncertainty in our knowledge of a user's valuation, we add random noise. Specifically, 
For $i \in \allitems$, $\noise(i) \sim \mathcal{D}(\mu_i = 0, \nu_i^2)$ denotes the noise term associated with item $i$, %The noise is assumed to be Gaussian with zero mean and $\nu_i^2$ variance. 
where the noise may be drawn from any distribution $\mathcal{D}$ having a zero mean. Every item has an independent noise distribution. For a set of items $I \subseteq \allitems$, we assume the noise is additive, i.e., the noise of $I$, $\noise(I) := \sum_{i \in I} \noise(i)$. \eat{ 
Since the noise distributions are independent, $\noise(I) \sim N(\sum_{i \in I} \mu_i, \sum_{i \in I} \nu_i^2)$. Such characterization of 
} 
Similar assumptions on additive noise are used in economics theory \cite{hirshleifer1978,Albertbidding07}. 
%%%%%%%%%%%%%% 
\eat{ 
\weic{Why do we restrict the noise to be Gaussian? I think we only need to assume the noise is additive
	and zero-mean, right? If we need Gaussian for the experiments, we can defer to the experimental
	section. The general framework should be as general as possible.}
\prit{I used Gaussian because I saw Gaussian being used in those econ papers, including Kevin LB paper where they derive value distribution from bidding history which turns out to be Gaussian. But you are right our theory does not need the Gaussian distribution, just the two properties you mentioned should be fine.}
\laks{changed to allow any distribution.} 
} 
%%%%%%%%%%%%%% 
Notice that all the three parameters -- value, price and noise are user independent and depend only on items. %We discuss alternative design choices and their implications in Section~\ref{sec:design}. 
%\weic{Why only talking about valuation noise? price is also user independent right?}
%\prit{True. I added that. Although not sure if price is ever personalized in any business.}

%%%%%%%%%%% 
\eat{ 
Also notice that in this characterization, noise is user independent. An alternative characterization can make noise to be user dependent \cite{nisan2007}. However providing approximation algorithm under such model is extremely difficult, as we shall show later in section \ref{sec:local_noise}.
} 
%%%%%%%%%%% 

%RETAIN THE ORIGINAL UNCOMMENTED PARAGRAPH FOR THE ARXIV VERSION. 
%    
Finally, the utility of an itemset $\itemset$ is $\util(\itemset) = \val(\itemset) - \price(\itemset) + \noise(\itemset)$. Since noise is %a 
random,  
%variable, 
utility is also random. However this randomness solely arises from the noise. 
%
\eat{
We use $\util^D(\itemset) = \val(\itemset) - \price(\itemset)$ to denote the deterministic part of the utility. 
} 
% 
<<<<<<< .mine
Also because noise is drawn from a zero mean distribution, $\mathbb{E}[\util(I)] = \val(\itemset) - \price(\itemset)$. Further, for the empty itemset $\emptyset$, we assume $\val(I) = 0$. %, making $\util(\emptyset) = \val(\emptyset) - \price(\emptyset) + \noise(I) = 0$.
=======
Also because noise is drawn from a zero mean distribution, $\mathbb{E}[\util(I)] = \val(\itemset) - \price(\itemset)$. 
For the empty itemset $\emptyset$, we assume $\val(I) = 0$. %, making $\util(\emptyset) = \val(\emptyset) - \price(\emptyset) + \noise(I) = 0$.
>>>>>>> .r859


\subsection{Diffusion Dynamics}\label{sec:decomic} 


%\subsubsection{Seed allocation}

\noindent
{\bf Seed allocation.\ \ }
%For every item a budget specifies the number of seeds that can be chosen for that item. 
Let $\vec{b} = (b_1, ..., b_{|\allitems|})$ be a vector of natural numbers representing the budgets associated with the items. An item's budget specifies the number of seed nodes that may be assigned to that item. We sometimes abuse notation and write $b_i \in \bvec$ to indicate that $b_i$ is one of the item budgets. We denote the maximum budget as $\bmax := max\{b_i\mid b_i\in \bvec\}$. We define an \emph{allocation} as a relation $\allalloc \subset V \times \allitems$ such that $\forall i\in\allitems: |\{(v,i)\mid v\in V\}| \le b_i$, i.e., each item is assigned a set of nodes whose size is under the item's budget. We refer to the nodes $S_i^{\allalloc} := \{v \mid (v,i) \in \allalloc\}$ as the \emph{seed nodes} of $\allalloc$ for item $i$ and to the nodes $S^{\allalloc} := \bigcup_{i\in\allitems} S_i^{\allalloc}$ as the \emph{seed nodes} of $\allalloc$. We denote the set of items allocated to a node $v\in V$ as ${\bf I}_v^{\allalloc} := \{i\in\allitems \mid (v,i) \in \allalloc\}$. 

%\subsubsection{Desire and adoption}

\noindent
{\bf Desire and adoption.\ \ }
Every node maintains two sets of items called desire set and adoption set. Desire set is the set of items that the node has been informed about (and thus potentially desires), via propagation or seeding. Adoption set, is the subset of the desire set, that the node adopts.  
%
%Unlike previous models, %~\cite{kempe03,lu2015}, 
%awareness does not necessarily imply adoption. In particular, 
%the seed nodes do not necessarily adopt the items allocated to them. 
%%Instead, adoption decision is driven . Items that are offered to a seed node, goes to the awareness set.
%A node adopts a subset of items in its awareness set that maximizes its utility. 
%
At any time a node selects, from its desire set at that time, the subset of items that maximizes the utility and adopts it. \chgins{W.l.o.g.}, we assume that any ties between itemsets are broken in favor of larger itemsets.  
%Thus, the adoption set of a node is a subset of its desire set. 
Following previous literature, we consider a progressive model: once a node desires an item, it remains in the node's desire set forever; similarly, once an item is adopted by a node, it cannot be unadopted later. 

For a node $u$, $\aware^{\allalloc}(u,t)$ denotes its desire set and $\adopt^{\allalloc}(u,t)$ denotes its adoption set at the time $t$, pertinent to an allocation $\allalloc$. We omit the time to refer to the adoption (desire) set at the end of diffusion: e.g., $\adopt^{\allalloc}(u)$ denotes the final adoption set of node $u$ at the end of diffusion for node $u$. 
%RETAIN THIS IN THE ARXIV VERSION. 
\eat{We are now ready to present the diffusion process of \model.}

%\subsubsection{The diffusion model}

<<<<<<< .mine
In the beginning of any diffusion, the noise term of every item is sampled,  which are then used till the diffusion terminates. The diffusion then proceeds in discrete time steps, starting from $t=1$. 
=======
\noindent
{\bf Diffusion model.\ \ }
In the beginning of any diffusion, the noise term of every item is sampled. These noise values are used till the diffusion terminates. The diffusion then proceeds in discrete time steps, starting from time $t=1$. 
>>>>>>> .r859
Given an allocation $\allalloc$ at $t=1$, the seed nodes have their desire sets initialized : $\forall v \in S^{\allalloc}$, $\awares(v,1) = {\bf  I}_v^{\allalloc}$. Seed nodes then adopt the subset of items from the desire set that maximizes the utility, breaking ties, if any, in favor of sets of larger cardinality. 
As a result, a seed node may not adopt all items allocated to it.

Once a seed node $u$ adopts an item $i$, its neighbor $u^\prime$ is influenced with probability $p_{u, u^\prime}$ (as in the IC model). 
%\chgins{Notice that the probability of influence $p_{u, u^\prime}$ remains same for every new adoption by $u$.} 
If the influence succeeds then $i$ is added to the desire set of $u^\prime$ at time $t =2$. The rest of the diffusion process is described in Figure~\ref{fig:ecomicmodel}.

%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{figure}[h]

\begin{framed}
\begin{small}


    \begin{description}[style=unboxed,leftmargin=8pt]

\item[1.]
\textbf{Edge transition.} At every time step $t > 1$, for a node $u'$ that has adopted at least one new item at $t-1$, its outgoing edges are tested for transition.
For an untested edge $(u',\ua)$, flip a biased coin independently: $(u',\ua)$ is {\em live} w.p.\ $p_{u',\ua}$ and {\em blocked} w.p.\ $1-p_{u',\ua}$. Each edge is tested {\em at most once} in the entire diffusion process and its status is remembered for the duration of a diffusion process. 

%\end{description}

Then for each node $\user$ that has at least one in-neighbor $u'$ (with a live edge $(u', \user)$) which adopted at least one item at $t-1$, $\ua$ is tested for possible item adoption (2-3 below).

%\begin{description}[style=unboxed,leftmargin=8pt]



\item[2.]
\textbf{Generating desire Set}
The desire set of node $\user$ at time $t$, $\awares(\user,t) = \awares(\user, t-1)   \cup_{u' \in N^-(\user)} (\adopts(u',t-1) )$, where $N^-(\user) = \{u' \mid (u', \user) \mbox{ is live}\}$ denotes the set of in-neighbors of $\user$ having a live edge connecting to $\user$. 

\item[3.]
\textbf{Node adoption.}
Node $\user$ determines the utilities for all subsets of items of the desire set  $\awares(\user,t)$. $\user$ then adopts a set $T^* \subseteq \awares(\user,t)$ such that  $T^* = \argmax_{T \in 2^{\awares(\user,t)}} \{\util(T) \mid T \supseteq \adopts(\user,t-1)\;\wedge\;\util(T)\ge 0\}$. $\adopts(\user, t)$ is set to $T^*$. 

    \end{description}
%\end{description}

\end{small}
\end{framed}
\caption{Diffusion dynamics under \model model}
\label{fig:ecomicmodel}
\end{figure} 
%%%%%%%%%%%%%%%%%%%%%%%%%%% 


\subsection{Definition of Social welfare Maximization}\label{sec:sw} 

Let $G = (V,E,p)$ be a social network, $\allitems$ the universe of items under consideration. 
\eat{
We denote by $\parameterset$ the set of model parameters, which includes price, value information and the noise distributions of items.
For an allocation $\allalloc$, $\phi(S_i)$ denotes the random set of $i$-adopted nodes as determined by the stochastic process of the diffusion model and randomness of valuations of itemsets, at the end of the propagation.  Let $\sigma(S_i) = \mathbb{E}(|\phi(S_i)|)$ be  the expected number of nodes that adopt item $i$. Note that $\phi(S_i)$ denotes a (random) set of nodes adopting $i$, whereas $\sigma(S_i)$ denotes the (expected) size of the set.

\weic{I am not sure we need this paragraph. Adoption is not the problem we want to study, so why define
	these terms here?}
	
\prit{True, but adoption is used heavily in the proofs later. Because of reachability property the most of the analysis on social welfare is actually about the adoptions. For completeness we defined it here itself.}

\weic{If adoptions are only used in the proofs, then I think it is better to defer the notations to the proofs when they are needed. There are already many terminologies and notations for readers to absorb.}
}
<<<<<<< .mine
%In this paper, 
We consider a novel objective driven by the utilities
earned from adoptions. We call it social welfare, which is the
sum of all users' utilities of itemsets adopted by users after the propagation converges. Formally, let $\E(\util(\adopt^{\allalloc}(u)))$ be the expected utility that a user $\user$ enjoys for a seed allocation $\allalloc$ after the propagation ends. Then the \emph{expected social welfare} \chgins{\footnote{In other communities such as algorithmic game theory, this is known as ``consumer surplus''.}} for $\allalloc$,  $\rho(\allalloc) = \E[\sum_{u \in V}\util(\adopt^{\allalloc}(\user))]$, where the expectation is over both the randomness of propagation and the randomness due to noise. 
=======
In this paper, we consider a novel utility-based objective  called {\em social welfare}, which is the
sum of all users' utilities of itemsets adopted by users after propagation converges. Formally, $\E(\util(\adopt^{\allalloc}(u)))$ is the expected utility that a user $\user$ enjoys for a seed allocation $\allalloc$ after the propagation ends. Then the \emph{expected social welfare} \chgins{\footnote{In other communities such as algorithmic game theory, this is also called as ``consumer surplus''.}} for $\allalloc$,  $\rho(\allalloc) = \E[\sum_{u \in V}\util(\adopt^{\allalloc}(\user))]$. Notice that the expectation is over both the randomness of propagation and the randomness due to noise. 
>>>>>>> .r859

%%%%%%%%%%%%%%%%%%%% SEE IF THIS NEEDS TO BE SAID ANYWHERE. 
\eat{ 
\spara{Key features of \model} 

Our utility driven model has several benefits over existing models. 

Firstly, the seed users in our model are treated as rational users. Thus they also go through the same utility based decision making like every other user of the network.

Secondly, \comic cannot handle the arrival of a set of items together. It had to use arbitrary tie-breaking in a case when a node becomes aware more than one items simultaneously, to put an order in the adoption. In \model, we treat this by creating an explicit desire set for nodes first. The utility is a set function as opposed to the point probability of GAP. Therefore even if more than one items arrive at the same time instance, the utility can treat them as a set, without the need of enforcing an explicit order.

Third, the notion of utility opens up a whole new objective of social welfare maximization, where instead of maximizing just the adoption, the utility earned from the adoptions is aimed to be maximized. No other model reported to date, has been able to study social welfare maximization. \model is the first framework which enables the study of utility in IM context.

Fourth, for complimentary products under \model, a greedy allocation algorithm that preserves $1 - \frac{1}{e}$ approximation guaranty with respect to optimal social welfare, although social welfare is not submodular in seed size. This greedy algorithm is independent of the model parameters. Hence it can be easily extended to multiple items, whereas for \comic extending the algorithm beyond two items was difficult due to parameter explosion.
} 
%%%%%%%%%%%%%%%%%%%%%%%% 

\eat{
\subsection{The Metrics} 

In this section, we define the metrics of item adoption and social welfare, as governed by the diffusion and item adoption model described in the earlier sections. Let $\allitems$ be the universe of items. For a user to adopt a set of items, two conditions must be satisfied: (i) the user must be aware of the items; (ii) the itemset should lead to the maximum possible utility, which should be non-negative. The parameters associated with our model are as follows. First, there is a probabilistic graph $G = (V,E, p)$, where for every link $(u,v) \in E$, $p_{uv} := p(u,v)$ specifies the influence probability from $u$ to $v$. Second, associated with every subset $I\subseteq \allitems$, there is a random variable $\eta_I$, representing the noise term that is used to model the uncertainty in our knowledge of the user's valuation of $I$. We define a \emph{possible world} associated with our model as a pair $W = (W^G, W^N)$, where $W^G \sim G$ is a sample drawn from the distribution associated with $G$ by sampling edges, and $W^N$ is a sample of noise terms for every subset of $\allitems$. For nodes $u, v \in V$, we say $v$ is reachable from $u$ in $W$ if there is a directed path from $u$ to $v$ in the deterministic graph $W^G$. Let $\vec{b} = (b_1, ..., b_{|\allitems|})$ be a vector of natural numbers representing the budgets associated with the items. We define an \emph{allocation} as a mapping $\allalloc: \allitems \rightarrow 2^{V}$, such that $|\allalloc(i)| \le b_i$, $1\le i \le |\allitems|$. In words, an allocation assigns a number of nodes to each item, and the number is no more than the item's budget. We refer to the nodes $S_i := \allalloc(i)$ as the seed nodes of $\allalloc$ for item $i$ and to the nodes $S := \bigcup_{i\in\allitems} \allalloc(i)$ as the seed nodes of $\allalloc$. We denote the set of items allocated to a node as $\allalloc^{-1}(v) := \{i\in\allitems \mid v \in \allalloc(i)\}$. 

Given an allocation, the adoption of items by nodes is governed by the diffusion described earlier. It is equivalent to the following possible world characterization. Given a possible world $W = (W^G, W^N)$ and an allocation $\allalloc$, a node $v \in V$ adopts a set of items as follows: (i) if $v$ is a seed node, then it adopts an itemset $\adopt_W(v) := \argmax \{util(I) \mid I\subseteq \allalloc^{-1}(v)\}$; when there are ties, we assume for convenience that itemsets with larger cardinality are preferred; (ii) if $v$ is a non-seed node, then it adopts an itemset $\adopt_W(v) := \argmax \{util(I) \mid I\subseteq \bigcup_{u\in S}\adopt_W(u) \;\wedge\; v \mbox{ is reachable from } u \mbox{ in } W \}$.  

The \emph{social welfare} of an allocation $\allalloc$ in a possible world $W = (W^G, W^N)$ is defined as the sum of utilities of itemsets adopted by nodes, i.e., $\rho_W(\allalloc) := \sum_{v\in V} util(\adopt_W(v))$. The \emph{adoption count} of $\allalloc$ in $W$ is defined as $\alpha_W(\allalloc) := \sum_{v\in V} |\adopt_W(v)|$. Their expectations are defined in the obvious manner. Specifically, the \emph{expected social welfare} of an allocation $\allalloc$ is $\rho(\allalloc) := \mathbb{E}_{W^G}[\mathbb{E}_{W^N}[\rho_W(\allalloc)]] = \mathbb{E}_{W^N}[\mathbb{E}_{W^G}[\rho_W(\allalloc)]]$. The \emph{expected adoption count} of $\allalloc$ is defined similarly. 
}
%%%%%%%%%%%%%%%%%%%%  

%\subsection{Problem}

\eat{Many interesting problems can be formulated around the framework of \model. However in this paper we focus on the novel roblem of welfare maximization (WelMax). We define the problem formally next.
} 

\eat{
 We denote by $\parameterset$ the set of model parameters, which includes price, value information and the noise distributions of items. 
} 
We define the problem of maximizing expected social welfare (\emph{WelMax}) as follows. We refer to $\val, \price, \noise$,  as the model parameters and denote them collectively as $\parameterset$. 

\begin{problem}
[WelMax]
Given $G = (V,E,p)$, the set of model parameters $\parameterset$, and budget vector $\bvec$, find a seed allocation $\allalloc^*$, such that $\forall i \in \allitems$, $|\alliseeds^*| \leq b_i$ and $\allalloc^*$ maximizes the expected social welfare, i.e., $\allalloc^* = \argmax_{\allalloc} \rho(\allalloc)$.
\end{problem}

%Unfortunately, WelMax is NP-hard. 

\begin{proposition}
WelMax is NP-hard.
\end{proposition}

\begin{proof}[(Sketch)]
It is easy to check that the classical influence maximization in the IC model, an
	NP hard problem, is a special case
	of WelMax.
%
%The result follows from the fact that the IM problem under the IC model is a special case of WelMax: let $\allitems = \{i\}$, set $\val(i) = 1$, $\price(i) = 0$ and set the noise term for item $i$ to $0$. This makes $\util(i) = 1$ so any influenced node will adopt $i$. Thus, the expected social welfare is simply the expected spread. We know maximizing expected spread under the IC model is NP-hard \cite{kempe03}.
\end{proof} 

\eat{ 
We show that IM problem under IC is a special case of WelMax. For that consider $\allitems = \{i\}$, that is there is only one item in the item set. Set the value of the item as $1$ and price as $0$. Noises for the item for all users are $0$. Hence the utility of adopting the item is always $1$ for any user. Thus the social welfare is simply the size of the set of nodes that adopts $i$. So maximizing social welfare translates to maximizing adoption. Thus for any set of nodes $S \subseteq V$, $\sigma_{IC}(S) = \rho(S)$.
\end{proof}
} 

%\subsection{Function Types} 
%\label{sec:fun-types} 

\noindent
{\bf Function types.\ \ }
Notice that the functions $\val$ and $\util$ are functions over sets of items, whereas $\sigma$ is a function over sets of network nodes, and $\rho$ is a function over allocations, which are sets of (node, item) pairs. When we speak of a certain property (e.g., monotonicity, submodularity, etc.) of a function of a given type, the property is meant w.r.t. the applicable type. E.g., $\sigma$ is well-known to be monotone and submodular w.r.t. sets of nodes. Similarly, we assume that $\val$ is a monotone supermodular function over sets of items. 


==> sec-proofs.tex <==
%\section{Remarks on Com-IC Model}
%
%\spara{Special Cases of Com-IC}
%We remark that \comic encompasses previously-studied single-entity and pure-competition models as special cases.
%When $\qao = \qbo = 1$ and $\qab = \qba = 0$, \model reduces to the (purely) competitive Influence Cascade model~\cite{infbook}.
%If, in addition, $\qbo$ is $0$, the model further reduces to the classic IC model.



\note[Laks]{The appendix looks a bit messy. We should order the material in the same order as the section of the main paper it pertains to. E.g., proofs before additional experiments.} 

\section{Remarks on Com-IC Model}



\subsection{Unreachable States}
Recall that in the \comic model, before an influence diffusion starts,
	all nodes are in the initial joint state ($\calA$-idle, $\calB$-idle).
According to the diffusion dynamics defined in Figure~\ref{fig:model}, 
	there exist five unreachable joint states, {\sl which are not material
	to our analysis and problem-solving, since none of these
	is relevant to actual adoptions}, the objectives studied in \SIM and \CIM.
For completeness, we list these states here.
\begin{enumerate}
\item ($\calA$-idle, $\calB$-rejected)
\item ($\calA$-suspended, $\calB$-rejected)
\item ($\calA$-rejected, $\calB$-idle)
\item ($\calA$-rejected, $\calB$-suspended)
\item ($\calA$-rejected, $\calB$-rejected)
\end{enumerate}

\begin{lemma}
In any instance of the \comic model (no restriction on GAPs), no node can reach
	the state of ($\calA$-idle, $\calB$-rejected), from its initial state
	of ($\calA$-idle, $\calB$-idle).
\end{lemma}
\begin{proof}
Let $v$ be an arbitrary node from graph $G=(V,E,p)$.
Note that for $v$ to reject $\calB$, it must be first be informed of $\calB$ (otherwise it remains $\calB$-idle, regardless of its state w.r.t.\ $\calA$), and then becomes $\calB$-suspended (otherwise it will be $\calB$-adopted, a contradiction).
Now,  note that $v$ is never informed of $\calA$, and hence it will not be triggered  to reconsider $\calB$, the only route
	to the state of $\calB$-rejected, according to the model definition.
Thus, ($\calA$-idle, $\calB$-rejected) is unreachable.
\end{proof}

The argument for ($\calA$-rejected, $\calB$-idle) being unreachable is symmetric,
	and hence omitted.

\begin{lemma}\label{lemma:unreach}
In any instance of the \comic model (no restriction on GAPs), no node can reach
	the state of ($\calA$-suspended, $\calB$-rejected), from its initial state
	of ($\calA$-idle, $\calB$-idle).
\end{lemma}
\begin{proof}
Let $v$ be an arbitrary node from graph $G=(V,E,p)$.
Note that for $v$ to reject $\calB$, it must be first be informed of $\calB$ (otherwise it remains $\calB$-idle, regardless of its state w.r.t.\ $\calA$), and then becomes $\calB$-suspended (otherwise it will be $\calB$-adopted, a contradiction).
Now,  $v$ transits from $\calA$-idle to $\calA$-suspended, meaning that $v$ does not adopt $\calA$.
This will not further trigger reconsideration, and hence $v$ stays at $\calB$-suspended.
This completes the proof.
\end{proof}

The argument for ($\calA$-rejected, $\calA$-suspended) being unreachable is symmetric,
	and hence omitted.
Finally, it is evident from the proof of Lemma~\ref{lemma:unreach} that, the joint state
	of ($\calA$-suspended, $\calA$-suspended) is a {\em sunken} state, meaning the node
	will not get out it to adopt or reject any product.
This implies that  ($\calA$-rejected, $\calB$-rejected) is also unreachable.


\subsection{Additional Counter-Examples}

The first two counter-examples show that self-monotonicity and
	cross-monotonicity may not hold in general for the \comic model when there is
	no restriction on GAPs.

\begin{figure}[h!]
 \centering
   \includegraphics[width=0.3\textwidth]{graphics/ex-non-mono}
 \caption{The graph for Example \ref{exp:non-mono}}
\label{fig:counter-mono}
\end{figure}

\begin{example}[Non-Self-Monotonicity] 
\label{exp:non-mono}
{\em
Consider Figure \ref{fig:counter-mono}.
All edges have probability $1$.
GAPs are $\qao = q \in (0,1)$, $\qab = \qbo = 1$, $\qba = 0$, which means that
	$\calA$ competes with $\calB$ but $\calB$ complements $\calA$.
Let $S_\calB = \{y\}$.
If $S_\calA$ is $S = \{s_1\}$, the probability that $v$ becomes $\calA$-adopted is $1$,
	because $v$ is informed of $\calA$ from $s_1$, and even if it does not adopt
	$\calA$ at the time, later it will surely adopt $\calB$ propagated from $y$,
	and then $v$ will reconsider $\calA$ and adopt $\calA$.
If it is $T = \{s_1, s_2\}$, that probability is $1-q+q^2 < 1$: $w$ gets $\calA$-adopted w.p. $q$ blocking $\calB$ and then $v$ gets $\calA$-adopted w.p. $q$; $w$ gets $\calB$-adopted w.p. $(1-q)$ and then $v$ surely gets $\calA$-adopted. 
Replicating sufficiently many $v$'s, all connected to $s_1$ and $w$, will lead to
	$\sigma_\calA(T,S_\calB) < \sigma_\calA(S,S_B)$. %, hence non-monotone. 
The intuition is that the additional $\calA$-seed $s_2$ ``blocks'' $\calB$-propagation
	as $\calA$ competes with $\calB$ ($\qba < \qbo$) but $\calB$ complements
	$\calA$ ($\qab > \qao$).
Clearly $\sigma_\calA$ is not monotonically decreasing in $S_\calA$ either (e.g., in a graph when all nodes are isolated).
Hence, $\sigma_\calA$ is not monotone in $S_\calA$.
\qed
}
\end{example}

\begin{figure}[h!]
 \centering
   \includegraphics[width=0.45\textwidth]{graphics/ex-cross-mono}
 \caption{The graph for Example \ref{exp:non-cross-mono}}
\label{fig:counter-cross-mono}
\end{figure}

\begin{example}[Non-Cross-Monotonicity] 
\label{exp:non-cross-mono}
{\em
We use the example shown in Figure \ref{fig:counter-cross-mono}.
All edges have probability $1$.
Nodes $y_1$ and $y_2$ are the two fixed $\calA$ seeds, and we want to grow
	$\calB$ seed set from $S=\{s_1\}$ to $T=\{s_1, s_2\}$.
GAPs satisfy $0 < \qab < \qao < 1$ and $0 < \qbo < \qba < 1$, 
	which means that
	$\calA$ complements $\calB$ but $\calB$ competes with $\calA$.
Since $\calB$ competes with $\calA$, it is straightforward to have examples in which
	the $\sigma_\calA$ decreases when $\calB$ seed set grows.
We use Figure~\ref{fig:counter-cross-mono} to show a possible world
	in which the growth of $\calB$ seed sets leads to $v$ adopting $\calA$,
	indicating that $\calA$ spread may also increase.
Even though we do not have a direct example showing that 
	$\sigma_\calA$ increases when $\calB$ seed set grows, 
	we believe the possible world example is a good indication that
	$\sigma_\calA$ is not cross-monotone in $S_\calB$.

Figure~\ref{fig:counter-cross-mono} uses Figure~\ref{fig:counter-mono}
	as a gadget.
Intuitively, when $\calB$ seed set grows from $S$ to $T$, 
	the probability that $z$ adopts $B$ decreases as shown in Example~\ref{exp:non-mono}.
Then we utilize this and the fact that $\calB$ competes with $\calA$ 
	to show that when $S$ is the $\calB$ seed set, due to $\calB$'s competition from
	$x$ node $v$ will not adopt $\calA$, but when $T$ is the $\calB$ seed set,
	there is no longer $\calB$'s competition from $x$ and thus $v$ will adopt $\calA$.

The node thresholds in the possible world are as follows:
$\qab < \alpha^w_\calA \le \qao$, $\qbo < \alpha^x_\calB \le \qba$, $\qao < \alpha^z_\calA$,
	$\qab < \alpha^v_\calA \le \qao$, and all other non-specified $\alpha$ values
	take value $0$, meaning that they will not block diffusion.

Consider first that $S$ is the $\calB$ seed set.
Since $\qbo < \alpha^x_\calB$, $x$ is informed about $\calB$
	from $s_1$ but will not adopt $\calB$ directly from $s_1$.
From $y_1$, we can see that $\calA$ will pass through $u$, $w$ and reaches $x$.
After $x$ adopts $\calA$, it reconsiders $\calB$, and since $\alpha^x_\calB \le \qba$,
	$x$ adopts $\calB$.
Node $x$ then informs $z$ about $\calA$ and $\calB$, in this order.
However, since $\qao < \alpha^z_\calA$, $z$ does not adopt $\calA$, but it adopts
	$\calB$ ($\alpha^z_\calB = 0 \le \qbo$).
Next $z$ informs $v$ about $\calB$, which adopts $\calB$ since $\alpha^v_\calB=0\le \qbo$.
This happens one step earlier than $\calA$ reaches $v$ from $y_2$, but since
	$\qab < \alpha^v_\calA$, $v$ will not adopt $\calA$.


Now consider that $T$ is the $\calB$ seed set.
In this case, $w$ definitely adopts $\calB$ from $s_2$.
Since $\qab < \alpha^w_\calA$ and $w$ adopts $\calB$ first, $w$ will not adopt
	$\calA$ from $y_1$.
Because $\qbo < \alpha^x_\calB$ and $w$ blocks $\calA$ from reaching
	$x$, $x$ will not adopt $\calA$ or $\calB$.
Then $z$ will not adopt $\calA$ or $\calB$ either.
This allows $\calA$ to reach $v$ from $y_2$, and since $\qab < \alpha^v_\calA \le \qao$,
	$v$ adopts $\calA$.


We can certainly duplicate $v$ enough times so that when $\calB$ seed set grows from
	$S$ to $T$, the $\calA$-spread in this possible world also increases, even though
	$\calB$ is competing with $\calA$. \qed
	
% The following is my failed attempt trying to come up with an example with GAP parameters.
%\red{We use the example shown in Figure \ref{fig:counter-cross-mono}.
%All edges have probability $1$.
%Nodes $y_1$ and $y_2$ are the two fixed $\calA$ seeds, and we want to grow
%	$\calB$ seed set from $S=\{s_1\}$ to $T=\{s_1, s_2\}$.
%GAPs are set as: $\qao=p \in (0,1)$, $\qab=0$, $\qbo=q\in (0,1)$, and $\qba=1$, 
%	which means that
%	$\calA$ complements $\calB$ but $\calB$ competes with $\calA$.
%Since $\calB$ competes with $\calA$, it is straightforward to have examples in which
%	the $\sigma_\calA$ decreases when $\calB$ seed set grows.
%We use Figure~\ref{fig:counter-cross-mono} to show a case that $\sigma_\calA$ 
%	also increases, and thus $\sigma_\calA$ is not cross-monotone in $S_\calB$.}
%
%\red{Figure~\ref{fig:counter-cross-mono} uses Figure~\ref{fig:counter-mono}
%	as a gadget.
%Intuitively, when $\calB$ seed set grows from $S$ to $T$, 
%	the probability that $z$ adopts $B$ decreases as shown in Example~\ref{exp:non-mono}.
%Then we utilize this and the fact that $\calB$ competes with $\calA$ such that
%	$v$ has less probability to adopt $\calB$ and thus $v$ has an increased probability
%	of adopting $\calA$. The actual calculation is as follows.}
%	
%\red{Consider the first case where $z$ adopts $\calB$ directly from $\calB$ seed $s_1$
%	which occurs with probability $q$.
%In this case, $z$ will definitely block $\calA$ propagating from $y_1$ since
%	$\qab=0$.
%The only chance that $v$ adopts $\calA$ is $z$ fails to activate $v$ in adopting $\calB$
%	(with probability $1-q$) and then $\calA$ passes through four intermediate nodes
%	from $y_2$ and activate $v$ (with probability $p^5$).
%This is the same whether we have $s_2$ as a $\calB$ seed, and thus, in this case
%	$\calA$ adoption probability at $v$ is the same for the two possible $\calB$
%	seed sets.}
%
%\red{Consider the second case where $z$ fails to adopt $\calB$ directly from 
%	$s_1$ (with probability $1-q$).
%Let $S$ be the $\calB$ seed set first. 
%Then, with probability $(1-p^3)$, $\calA$ from $y_1$ does not activate $z$,
%	in which case the only possibility that $v$ adopts $\calA$ is that
%	$\calA$ from $y_1$ activates $v$ (with probability $p^5$).
%On the other hand, if $z$ adopts $\calA$ coming from $y_1$ (with probability $p^3$),
%	by reconsideration $z$ will then also adopts $\calB$ (since $\qba=1$).
%Then $v$ may adopt $\calA$ either because $z$ activates $v$ (with probability $p$),
%	or $z$ fails to activate $v$ for $\calA$ and then for $\calB$
%	(with probability $(1-p)(1-q)$), and then $\calA$ from $y_2$ activates $v$
%	(with probability $p^5$).
%Here if $z$ would activate $v$ for $\calB$, $\calB$ would reach $v$ one step earlier than
%	$\calA$ coming from $y_2$ and thus blocking $\calA$.
%This is the key step in the setup.
%Together, under the second case, when $S$ is the $\calB$ seed set, 
%	$v$ adopts $\calA$ with probability $(1-p^3)p^5 + p^3(p+(1-p)(1-q)p^5)$.
%}
%
%\red{
%Finally, consider the above second case, but now $T$ is the $\calB$ seed set.
%If $w$ adopts $\calB$ from $s_2$ directly (with probability $q$), $w$ will certainly block
%	$\calA$ from $y_1$.
%In this case, $z$ will not adopt $\calA$ or $\calB$ and
%	$v$ adopts $\calA$ only when $\calA$ from $y_2$ reaches $v$ (with probability $p^5$).
%If $w$ does not adopt $\calB$ from $s_2$ directly (with probability $1-q$), 
%	we claim that under this condition $v$'s adoption of $\calA$ is exactly the same
%	as if $s_2$ is not a $\calB$ seed.
%The reason is as follows.
%First, if $\calA$ from $y_1$ does not reach $w$, then $w$ will not adopt
%	$\calA$ or $\calB$, same as the corresponding case when $s_2$ is not a $\calB$ seed.
%Second, if $w$ adopts $\calA$ from $y_1$, in this case by reconsideration $w$ will
%	adopts $\calB$.
%Superficially this looks different from the case when $s_2$ is not a $\calB$ seed.
%However, consider the next step, when $w$ tries to activate $z$ for $\calA$.
%If this activation succeeds, then $z$ adopts $\calA$ first and then by reconsideration
%	$z$ adopts $\calB$.
%This behavior is exactly the same as $w$ would activate $z$ even when $s_2$ is not a
%	$\calB$ seed.
%If $w$ fails to activate $z$ for $\calA$, then $w$ will not try to activate $z$ for
%	$\calB$ again, since $s_1$ already tried and failed activating $\calB$.
%Thus $w$ adopting $\calB$ via reconsideration is not essential for $z$'s adoption status,
%	and thus we show that in this case the $v$'s adoption of $\calA$ is exactly the
%	same as if $s_2$ is not a $\calB$ seed.
%Borrowing the result for the case of $S$ as $\calB$ seed, we have that when
%	$T$ is the $\calB$ seed set, under the second case condition the probability that
%	$v$ adopts $\calA$ is $q p^5+(1-q)((1-p^3)p^5 + p^3(p+(1-p)(1-q)p^5))$.
%}
}
\end{example}


\begin{figure}[h!]
 \centering
   \includegraphics[width=0.3\textwidth]{graphics/ex-non-self-submod}
 \caption{The graph for Example \ref{exp:complement1} and \ref{exp:complement2}}
\label{fig:counter-sub}
\end{figure}

The following two examples show that even when two items are mutually complementary,
	self-submodularity and cross-submodularity in general may not hold.

\begin{example}[Non-Self-Submodularity]
\label{exp:complement1}
{\em
Consider the possible world in Figure~\ref{fig:counter-sub}.
All edges are live.
The node thresholds are:
for $w$: $\alpha_\calA^w \leq \qao$, $\qbo < \alpha_\calB^w \leq \qba$;
for $z$: $\alpha_\calA^z > \qab$, $\alpha_\calB^z < \qbo$;
for $v$: $\qao < \alpha_\calA^v \leq \qab$, $\alpha_\calB^v \leq \qbo$;
Then fix $S_\calB = \{y\}$.
For $S_\calA$, let $S = \emptyset$, $T = \{x\}$, and $u$ is the additional seed.
It can be verified that only when $S_\calA = T \cup \{u\}$, $v$ becomes
	$\calA$-adopted, violating self-submodularity.


A concrete example of $\bQ$ for which submodularity does not hold is as follows: 
	$\qao = 0.078432$; $\qab = 0.24392$; $\qbo = 0.37556$; $\qba = 0.99545$.
Seed sets are the same as above.
We denote by $p_v(S_\calA)$ the probability that $v$ becomes $\calA$-adopted with A-seed set $S_\calA$.
It can be verified that:
$p_v(S) = 0$, $p_v(S \cup \{u\}) = 8.898 \cdot 10^{-5}$, $p_v(T) = 0.027254$, and $p_v(T \cup \{u\}) = 0.027383$.
Clearly, $p_v(T \cup \{u\}) - p_v(T) > p_v(S \cup \{u\}) - p_v(S)$.
Hence, replicating $v$ sufficiently many times will lead to
	$\sigma_\calA(T\cup\{u\}, S_\calB) - \sigma_\calA(T, S_\calB) \geq \sigma_\calA(S\cup\{u\} ,  S_\calB)- \sigma_\calA(S,  S_\calB)$, violating self-submodularity.
\qed
}
\end{example}


\begin{example}[Non-Cross-Submodularity]
\label{exp:complement2}
{\em
Consider the possible world in Figure~\ref{fig:counter-sub}.
The node thresholds are:
For $w$: $\qao < \alpha_\calA^w \leq \qab$, $\alpha_\calB^w \leq \qbo$;
for $z$: $\alpha_\calA^z \leq \qao$, $\alpha_\calB^z > \qba$;
for $v$: $\qao < \alpha_\calA^v \leq \qab$, $\alpha_\calB^v \leq \qbo$.
Fix $S_\calA = \{y\}$.
For $S_\calB$, let $S = \emptyset$, $T = \{x\}$, and $u$ is the additional seed.
It can be verified that only when $S_\calB = T \cup \{u\}$, $v$ becomes $\calA$-adopted,
	violating % both cross-monotonicity and 
	cross-submodularity. 
\qed
}
\end{example}

The above example applies even when \blue{$\qba = \qbo < 1$}.
The key is that $\qba < 1$ and $\alpha_\calB^z > \qba$, which prevents $\calB$ to
	pass through $z$, and thus another $\calB$-seed $u$ is needed to inform $v$ of $\calB$.



\section{Pseudo-code of {\large \timsimfast}}

Here we give the pseudo-code to \timsimfast that is omitted from \textsection\ref{sec:rrset}.
This is one of the RR-set generation
	procedure we proposed for \SIM in \textsection\ref{sec:rrset}.
\begin{algorithm}[h]
\DontPrintSemicolon
\caption{\timsimfast($G=(V,E)$, $v$, $S_\calB$)} \label{alg:rrset-sim-fast}
create an FIFO queue $Q$ and empty sets $R$, $T_1$\;
 $Q.\mathsf{enqueue}(v)$; \tcp{\rm\it first backward BFS}       \label{line:y1}
\While{\em $Q$ is not empty} { 
       $u \gets Q.\mathsf{dequeue}()$\;
	$T_1 \gets T_1 \cup \{u\}$\;
       \ForEach{\em unvisited $w \in N^-(u)$ such that $(w,u)$ is live } {
               $Q.\mathsf{enqueue}(w)$ and mark $w$ visited\;     \label{line:y2}
        }
}
\If {$T_1 \cap S_\calB \neq \emptyset$  } {  \label{line:y3}
	\tcp{auxiliary forward pass to determine $\calB$ adoption}
      clear $Q$, enqueue all nodes of $T_1\cap S_\calB$ into $Q$, and execute line \ref{line:x1} to line \ref{line:x2} in Algorithm~\ref{alg:rrset-sim}\;   \label{line:y4}
}
execute line \ref{line:x3} to line \ref{line:x4} in  Algorithm~\ref{alg:rrset-sim} 
\tcp{second backward BFS} 
 \label{line:y5}
\end{algorithm}





\section{Additional Experimental Results}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h!t!]
\scriptsize
\begin{minipage}[b]{0.48\hsize}\centering
	\begin{tabular}{rccc|ccc}
		\cline{2-7}
		\underline{\bf\SIM} & \multicolumn{3}{|c|}{\vanillaIC} & \multicolumn{3}{c|}{\copying} \\ \cline{2-7}
		$\qao$ & \multicolumn{1}{|c}{$0.1$} & $0.3$ & $0.5$ & $0.1$ & $0.3$ & \multicolumn{1}{c|}{$0.5$} \\ \cline{2-7}
		\dbBook & \multicolumn{1}{|c}{$2.16\%$} & $1.12\%$ & $0.71\%$ & $133\%$ & $419\%$ & \multicolumn{1}{c|}{$676\%$} \\
		\dbMovie & \multicolumn{1}{|c}{$4.38\%$} & $1.49\%$ & $0.87\%$ & $236\%$ & $737\%$ & \multicolumn{1}{c|}{$1283\%$} \\
		\flix & \multicolumn{1}{|c}{$10.6\%$} & $0\%$ & $0\%$ & $134\%$ & $352\%$ & \multicolumn{1}{c|}{$641\%$} \\
		\lastfm & \multicolumn{1}{|c}{$3.76\%$} & $2.65\%$ & $1.65\%$ & $398\%$ & $1355\%$ & \multicolumn{1}{c|}{$2525\%$} \\	
		\cline{2-7}
	\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[b]{0.48\hsize}\centering
   	\begin{tabular}{rccc|ccc}
		\cline{2-7}
		\underline{\bf\CIM}& \multicolumn{3}{|c|}{\vanillaIC} & \multicolumn{3}{c|}{\copying} \\ \cline{2-7}
		$\qbo$ & \multicolumn{1}{|c}{$0.1$} & $0.5$ & $0.8$ & $0.1$ & $0.5$ & \multicolumn{1}{c|}{$0.8$} \\ \cline{2-7}
		\dbBook & \multicolumn{1}{|c}{$548\%$} & $644\%$ & $717\%$ & $834\%$ & $238\%$ & \multicolumn{1}{c|}{$252\%$} \\
		\dbMovie & \multicolumn{1}{|c}{$1060\%$} & $994\%$ & $713\%$ & $637\%$ & $106\%$ & \multicolumn{1}{c|}{$89.2\%$} \\
		\flix & \multicolumn{1}{|c}{$956\%$} & $152\%$ & $102\%$ & $888\%$ & $119\%$ & \multicolumn{1}{c|}{$95\%$} \\
		\lastfm & \multicolumn{1}{|c}{$1361\%$} & $982\%$ & $710\%$ & $489\%$ & $65.3\%$ & \multicolumn{1}{c|}{$63.6\%$} \\
		\cline{2-7}
	\end{tabular}
\end{minipage}
%\vspace{-2mm}
\caption{Percentage improvement of \generalTIM over \vanillaIC \& \copying, where the other seed set is randomly chosen}
\label{tab:synGAP-random}
%\vspace{-3mm}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h!t!]
\scriptsize
\begin{minipage}[b]{0.48\hsize}\centering
	\begin{tabular}{rccc|ccc}
		\cline{2-7}
		\underline{\bf\SIM} & \multicolumn{3}{|c|}{\vanillaIC} & \multicolumn{3}{c|}{\copying} \\ \cline{2-7}
		$\qao$ & \multicolumn{1}{|c}{$0.1$} & $0.3$ & $0.5$ & $0.1$ & $0.3$ & \multicolumn{1}{c|}{$0.5$} \\ \cline{2-7}
		\dbBook & \multicolumn{1}{|c}{$0.34\%$} & $0.34\%$ & $0\%$ & $0.34\%$ & $0.34\%$ & \multicolumn{1}{c|}{$0\%$} \\
		\dbMovie & \multicolumn{1}{|c}{$0.64\%$} & $0.54\%$ & $0.36\%$ & $0.64\%$ & $0.54\%$ & \multicolumn{1}{c|}{$0.36\%$} \\
		\flix & \multicolumn{1}{|c}{$0\%$} & $0\%$ & $0\%$ & $0\%$ & $0\%$ & \multicolumn{1}{c|}{$0\%$} \\
		\lastfm & \multicolumn{1}{|c}{$1.73\%$} & $1.38\%$ & $0.80\%$ & $1.73\%$ & $1.38\%$ & \multicolumn{1}{c|}{$0.80\%$} \\	
		\cline{2-7}
	\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[b]{0.48\hsize}\centering
   	\begin{tabular}{rccc|ccc}
		\cline{2-7}
		\underline{\bf\CIM}& \multicolumn{3}{|c|}{\vanillaIC} & \multicolumn{3}{c|}{\copying} \\ \cline{2-7}
		$\qbo$ & \multicolumn{1}{|c}{$0.1$} & $0.5$ & $0.8$ & $0.1$ & $0.5$ & \multicolumn{1}{c|}{$0.8$} \\ \cline{2-7}
		\dbBook & \multicolumn{1}{|c}{$3.53\%$} & $1.19\%$ & $0.24\%$ & $1.03\%$ & $0.18\%$ & \multicolumn{1}{c|}{$0.05\%$} \\
		\dbMovie & \multicolumn{1}{|c}{$141\%$} & $22.2\%$ & $9.87\%$ & $138\%$ & $20.7\%$ & \multicolumn{1}{c|}{$8.67\%$} \\
		\flix & \multicolumn{1}{|c}{$3.93\%$} & $1.63\%$ & $-1.69\%$ & $3.93\%$ & $1.63\%$ & \multicolumn{1}{c|}{$-1.69\%$} \\
		\lastfm & \multicolumn{1}{|c}{$5.38\%$} & $2.19\%$ & $0.69\%$ & $2.72\%$ & $0.11\%$ & \multicolumn{1}{c|}{$-0.97\%$} \\
		\cline{2-7}
	\end{tabular}
\end{minipage}
%\vspace{-2mm}
\caption{Percentage improvement of \generalTIM over \vanillaIC \& \copying,
	where the other seed set is chosen to be the top-100 nodes by \vanillaIC}
\label{tab:synGAP-top100}
%\vspace{-3mm}
\end{table*}


\subsubsection*{\large \generalTIM vs.\ \vanillaIC and \copying}

\pink{
We now report additional results for the experiments done with 
	synthetic GAPs in \textsection\ref{sec:synGAPexp}.
}

\pink{
Table~\ref{tab:synGAP-random} shows the percentage improvement of
	\generalTIM over \vanillaIC and \copying baselines when the other
	seed set ($\calB$-seeds for \SIM and $\calA$-seeds for \CIM)
	consists of 100 {\em random nodes}.
As can be seen, \generalTIM is significantly better except when
	comparing to \vanillaIC in \SIM.
This is not surprising, as when $\calB$-seeds are chosen randomly, they
	are unlikely to be very influential and hence it is rather
	safe to ignore them when selecting $\calA$-seeds, which is
	essentially how \vanillaIC operates.
}

\pink{
Table~\ref{tab:synGAP-top100} shows the results when the other seed
	set is chosen to be the {\em top-100 nodes} from \vanillaIC.
These nodes represent the most influential ones under the IC model
	that can be found efficiently in polynomial time\footnote{Recall that influence maximization is NP-hard under the IC model, and thus the optimal top-100 most influential nodes are difficult to find. The seeds found by \vanillaIC can be regarded as a good proxy.}.
In this case, the advantage of \generalTIM over \vanillaIC and \copying
	is less significant.
On \flix dataset, the three algorithms achieve the same influence spread
	for \SIM, while for \CIM, when $\qbo = 0.8$, we even observe a slight
	disadvantage of \generalTIM in certain cases. 
The reason is that when $\qbo = 0.8$ (quite close to $1$), targeting
	the input $\calA$-seeds to be $\calB$-seeds is itself a good
	strategy (see Theorem~\ref{thm:cimOpt}).
For \SIM, we remark that \vanillaIC and \copying is equivalent.
%They are both very effective as the input $\calB$-seeds are already quite influential.
}

\pink{
Overall, considering Tables \ref{tab:synGAP}, \ref{tab:synGAP-random}, and \ref{tab:synGAP-top100}
	all together, we can see that in the vast majority of all test cases,
	\generalTIM outperforms these two baselines, often by a large margin.
This demonstrates that \generalTIM is robust w.r.t. different selection methods of the opposite seed set.
Furthermore, in real-world scenarios, the opposite seed sets may simply consist of ``organic'' early adopters, i.e., users who
	adopt the product spontaneously. %, instead of being targeted by the advertiser.
The robustness of \generalTIM is thus highly desirable as it is often
	difficult to foresee which users would actually become organic early adopters in real life.
}

\begin{table*}[t!]
	\centering
	\begin{tabular}{rrcccc}
		$\calA$ & $\calB$ & $\qao$ & $\qab$ & $\qbo$ & $\qba$ \\  \hline
		{\it Monster Inc.} & {\it Shrek} &  $.88 \pm .01$ & $.92 \pm .01$ & $.92 \pm .01$ & $.96 \pm .01$ \\ 
		{\it Gone in 60 Seconds} & {\it Armageddon} &  $.63 \pm .02$ & $.77 \pm .02$ & $.67 \pm .02$ & $.82 \pm .02$ \\ 
		{\it Harry Porter: Prisoner of Azkaban} & {\it What a Girl Wants} & $.85\pm .01$ & $.84\pm .02$ & $.66\pm .02$ & $.67 \pm .02$ \\ 
		{\it Shrek} & {\it The Fast and The Furious}  & $.92\pm .02$ & $.94\pm .01$ & $.80\pm .02$ & $.79\pm .02$ \\ \hline
	\end{tabular}
	\caption{Selected GAPs learned for movies from \flix}
	 \label{tab:Q-flix}
\end{table*}

\begin{table*}[t!]
	\centering
	\begin{tabular}{rrcccc}
		$\calA$ & $\calB$ & $\qao$ & $\qab$ & $\qbo$ & $\qba$ \\  \hline
		{\it The Unbearable Lightness of Being} & {\it Norwegian Wood (Japanese)} &  $.75 \pm .01$ & $.85\pm .02$ & $.92\pm .01$ & $.97\pm .01$ \\ 
		{\it Harry Potter and the Philosopher's Stone} & {\it Harry Potter and the Half-Blood Prince} &  $.99\pm 1$ & $1.0 \pm 0$ & $.97\pm .01$ & $.98\pm .01$ \\ 
		{\it Stories of Ming Dynasty III (Chinese)} & {\it Stories of Ming Dynasty VI (Chinese)} & $.94\pm .01$ & $1.0\pm 0$ & $.88\pm .03$ & $.98\pm .01$ \\ 
		{\it Fortress Besieged (Chinese)} & {\it Love Letter (Japanese)}  & $.89\pm .01$ & $.91\pm .03$ & $.82\pm .02$ & $.83 \pm .03$ \\ \hline
	\end{tabular}
	\caption{Selected GAPs learned for movies from \dbBook}
	 \label{tab:Q-dbBook}
\end{table*}
%
%
\begin{table*}[t!]
	\centering
	\begin{tabular}{cccccc}
		$\calA$ & $\calB$ & $\qao$ & $\qab$ & $\qbo$ & $\qba$ \\  \hline
		{\it Up } & {\it 3 Idiots} &  $.92\pm .01$ & $.94\pm .01$ & $.92 \pm .01$ & $.93 \pm .01$ \\ 
		{\it Pulp Fiction} & {\it Leon} &  $.81\pm .01$ & $.83\pm .01$ & $.95\pm .00$ & $.98\pm .01$ \\ 
		{\it The Silence of the Lambs} & {\it Inception} & $.90 \pm .01$ & $.86 \pm .01$ & $.92\pm .01$ & $.98\pm .01$ \\ 
		{\it Fight Club} & {\it Se7en}  & $.84\pm .01$ & $.89 \pm .01$ & $.89\pm .01$ & $.95\pm .01$ \\ \hline
	\end{tabular}
	\caption{Selected GAPs learned for movies from \dbMovie}
	 \label{tab:Q-dbMovie}
\end{table*}
%
%
\begin{figure*}
\centering
\begin{tabular}{cccc}
\hspace{-4mm}\includegraphics[width=.25\textwidth]{graphics/flixster_eps_spread_time_SIM}&
\hspace{0mm}\includegraphics[width=.25\textwidth]{graphics/flixster_eps_spread_time_CIM}&
\hspace{0mm}\includegraphics[width=.25\textwidth]{graphics/dbBook_eps_spread_time_SIM}&
\hspace{0mm}\includegraphics[width=.25\textwidth]{graphics/dbBook_eps_spread_time_CIM}\\
\hspace{-4mm} (a) \SIM, \flix  & \hspace{0mm} (b) \CIM, \flix   & \hspace{0mm} (c) \SIM, \dbBook & \hspace{0mm} (d) \CIM, \dbBook
\end{tabular}
\caption{Effects of $\epsilon$ on RR-set algorithms (\flix and \dbBook)}
\label{fig:epsilon}
\end{figure*}

\subsubsection*{GAPs learned from Real Social Networks}
Tables~\ref{tab:Q-flix} -- \ref{tab:Q-dbMovie} demonstrate selected 
	GAPs learned from \flix, \dbBook, and \dbMovie datasets, using methods in \textsection\ref{sec:exp}.
Here we not only show the estimated value of $\bQ$, but also give 95\% confidence intervals.
By the definition of GAPs (\textsection\ref{sec:model}), we can treat each GAP as the parameter of
	a Bernoulli distribution.
Consider any GAP, denoted $q$, and let $\bar{q}$ be its estimated value from action log data.
The 95\% confidence interval\footnote{See any standard textbooks on probability theory and statistics} of $\bar{q}$ is given by
\[
\left[ \bar{q} - 1.96\sqrt{\bar{q}(1-\bar{q})/n_q}, \; \bar{q} + 1.96\sqrt{\bar{q}(1-\bar{q})/n_q} \right],
\]
where $n_q$ is the number of samples used for estimating $q$.


\subsubsection*{Effect of {\large $\epsilon$} in {\large\generalTIM}}

%\noindent\textbf{Results \& Analysis: Effects of $\epsilon$.}
%We first evaluate the effects of $\epsilon$ on  \generalTIM.
As mentioned in \textsection\ref{sec:rrset}, $\epsilon$
	controls the trade-off between approximation ratio and efficiency.
Figure~\ref{fig:epsilon} plots influence spread and running time (log-scale)
	side-by-side, as a function of $\epsilon$, on \flix and \dbBook for
	both problems.
The results on other datasets are very similar and thus omitted.
We can see that as $\epsilon$ goes up from $0.1$ to $0.5$
	and $1$ (in fact, $\epsilon = 1 > (1-1/e)$ means theoretical approximation guarantees are lost),
	the running time of all versions of \generalTIM (\timsim, \timsimfast, \timcim)
	{\sl decreases dramatically}, by orders of magnitude.
	while, in practice, influence spread (\SIM) and boost (\CIM) are {\sl almost
	completely unaffected} (the largest difference among all test cases is only $0.45\%$).
%This allows us to set a reasonably large $\epsilon$: unless otherwise stated, we use 
%	$\epsilon=0.5$ for \timsim and \timsimfast, and $\epsilon = 1$ for \timcim.



\subsubsection*{Sandwich Approximation (SA)}
As discussed in \textsection\ref{sec:sandwich}, 
SA is likely to be effective for \SIM and \CIM when the adoption probabilities are
	close, which is indeed the case for the real world data we learn.
We now measure the effectiveness of SA by comparing the spread achieved
	by seed sets $S_\sigma, S_\nu, S_\mu$ obtained
	w.r.t.\ the original, upper bound, and lower bound functions respectively.
Such spread must be computed using the original function $\sigma$, and in our case,
	the unaltered GAPs.
More specifically, we calculate the relative error defined as follows (for \CIM, disregard $S_\mu$).
\[
\mathtt{SA\_error} ={\max\{|\sigma(S_\sigma) - \sigma(S_\mu)|, |\sigma(S_\sigma) - \sigma(S_\nu)|\}} \; / \; {\sigma(S_\sigma)}.
\]

In all four datasets, for both problems, the largest error is only $0.2\%$!
To see if this is due to that $\qbo$ and $\qba$ being close in the GAPs learned
	from action log data, we further ``stress test'' SA with a much more adversarial set-up.
For \SIM, vary $\qbo$ to be $\{.1, .5, .9\}$ and fix $\qba = .96$.
For \CIM, vary $\qba$ to be $\{.1, .5, .9\}$ and fix $\qbo = .1$ (to maintain complementarity).
No change is made to $\qao$ and $\qab$.

Figure~\ref{fig:sandwich} compares $\sigma(S_\sigma)$, $\sigma(S_\mu)$, and $\sigma(S_\nu)$
	on \flix.
As can be seen, even in this adversarial setting, SA is still highly effective for both \SIM and \CIM.
Amongst all test cases, the largest error is $0.4\%$.
The results on other datasets are very similar and hence omitted.
We further stress test more by separating $\qao$ and $\qab$ to a wider margin, and still achieve
	similar results (hence omitted).
This means the SA strategy is highly robust and useful for our problems. 

\begin{figure}[h!]
\centering
\includegraphics[width=0.375\textwidth]{graphics/sandwich}
\caption{Sandwich Approximation on \flix}
\label{fig:sandwich}
\end{figure}






\section{Proofs and Additional Theoretical Results}\label{sec:proof}

\subsection{Proofs for Results in Section~\ref{sec:problem}}

\smallskip\textsc{Theorem~\ref{thm:hard}} (re-stated).
{\em \theoremCIMHard}


\begin{proof}
%\CIM also subsumes influence maximization under classic IC: we set $\qao = 0$ (thus without $\calB$-seeds, any $\calA$-seed set would have an $\calA$-spread of $0$) and set $\qab = \qbo = \qba = 1$.
%We then create a special node $a$, which has a directed edge to all $v\in V$ with influence probability $1$.
%When $S_\calA = \{a\}$, finding a $\calB$-seed set to maximize the increase in $\calA$-spread is equivalent to maximizing $\calB$-spread.
%Hence, \CIM also subsumes influence maximization under the classic IC model.
%This completes the proof.

Let $\bf I$ be an instance of {\sc InfMax} with the IC model,
	defined by a directed graph $G=(V,E)$ and budget $b < |V|$.
We define an instance $\bf J$ of \CIM as follows.
For each $v\in V$, create a dummy copy $v'$ and a directed edge $(v',v)$ with influence probability $p_{v',v} = 1$.
Let $V'$ be the set of all dummy nodes.
Set $S_\calA = V'$, $\qao = 0$, $\qab = \qbo = \qba = 1$.
The budget $b$ of selecting $\calB$ seeds in instance 
	$\bf J$ is the same $b$ as in instance $\bf I$.
	
\begin{claim}\label{claim:cimhard1}
Consider the \CIM instance $\bf J$.
For all $\cal B$-seed sets $S_\calB$, there exists a set $T_\calB \subseteq V'$
	such that $\sigma_\calA(S_\calA, T_\calB) \geq \sigma_\calA(S_\calA, S_\calB)$.
\end{claim}

\begin{proof}[of Claim~\ref{claim:cimhard1}]
Let $v \in S_\calB \cap V$ be any regular node.
Assume for now that $v'\not\in S_\calB$. 
Let $S'_\calB$ denote the $\calB$-seed set obtained by replacing all such $v$ by
	its corresponding dummy copy $v'$.
Since $S_\calA=V'$, all dummy nodes are $\calA$-adopted and all regular nodes are
	$\calA$-informed. 
Choosing $v'$ to be a $\calB$-seed makes $v'$ and $v$ both $\calB$-adopted,
	so by reconsideration $v$ becomes $\calA$-adopted as well.
Clearly, the sets of regular nodes that are $\calB$-adopted 
	under the configurations $(S_\calA, S_\calB)$ and $(S_\calA, S'_\calB)$ are the same.
Thus,  sets of regular nodes that are $\calA$-adopted under these configurations
	are also the same, which verifies the claim. 

Now suppose $v, v'\in S_\calB$.
We claim that there exists a dummy node outside $S_\calB$, which follows from the fact that
	the budget $b < |V|=|V'|$.
Now, replace $v$ with any dummy node $u'$ not in $S_\calB$ and call the resulting $\calB$-seed set $S'_\calB$.
By an argument similar to the above case, we can see that every regular node that is $\calA$-adopted under 
	configuration $(S_\calA, S_\calB)$ is also $\calA$-adopted under configuration $(S_\calA, S'_\calB)$. 
There may be additional $\calA$-adopted regular nodes
	thanks to the seed $u'\in S'_\calB \setminus S_\calB$. 
Again, the claim follows.
Finally, if $S_\calB \cap V = \emptyset$ (no regular node in $S_\calB$),
	then the claim trivially holds as we can simply let $T_\calB = S_\calB$.
\end{proof}

Now consider any $T\subseteq V$ and let $\sigma_{IC}(T)$ denote the expected spread of
	$T$ under the IC model in $G$.
Let $T' = \{v'\in V' : v\in T\}$ be the set of corresponding dummy copies.
Since $S_\calA = V'$, all regular nodes (in $V$) would become $\cal A$-informed
	when $S_\calB = \emptyset$. %, and moreover, $\sigma_\calA(S_\calA, \emptyset) = |V'|$.
Now set $S_\calB = T'$, which would make all nodes in $T$ (regular) become $\calB$-adopted,
	%(recall that $\qbo =1$ and $p_{v',v} =1$ for all $v\in V$), 
	and then $\calA$-adopted (by reconsideration), and further propagate both $\calA$
	and $\calB$ over the network.
Hence,
\begin{align}\label{eqn:nphard}
\sigma_{IC}(T) = \sigma_\calA(S_\calA, T') - n,
\end{align}
where $n =_{\mathrm{def}} |V| = |V'|$.

%\weic{We cannot directly claim that $S^*_{\bf J}$ is a solution of $\bf I$,
%	because it may contain nodes in $V'$, which is not in the instance of
%	$\bf I$. I made some changes below.}

Next, to prove the theorem, it suffices to show:
\begin{claim}\label{claim:cimhard2}
The subset $T_*\subset V$ is an optimal solution to the {\sc InfMax} (with IC model)
	instance ${\bf I}$ if and only if $T_*' \subset V'$ is an optimal solution to
	the \CIM instance $\bf J$ under the \comic model, where $T_*' = \{v'\in V' : v\in T_*\}$.
\end{claim}

\begin{proof}[of Claim~\ref{claim:cimhard2}]
$(\Longrightarrow)$: Suppose for a contradiction that $T_*'$ is suboptimal to $\bf J$.
Let $X'$ be an optimal solution to $\bf J$ instead, which implies that
	$\sigma_\calA(S_\calA, X') > \sigma_\calA(S_\calA, T_*')$.

If $X'$ contains only dummy copies, let $X$ be the corresponding set of regular nodes.
Then, by Eq.~\eqref{eqn:nphard},
\[
\sigma_\calA(S_\calA, X') = \sigma_{IC}(X) + n > \sigma_\calA(S_\calA, T_*') = \sigma_{IC}(T_*) + n.
\]
Hence $\sigma_{IC}(X) > \sigma_{IC}(T_*)$, contradicting to the fact that $T_*$ is
	optimal to ${\bf I}$.

If $X'$ contains at least one regular node, then by repeated application of
	Claim~\ref{claim:cimhard1}, we can obtain a $\calB$-seed set with none regular nodes
	and furthermore dominates $X'$ w.r.t. $\calA$-spread.
Thus, w.l.o.g. we can ignore $\calB$-seed sets
	containing regular nodes. 
	
$(\Longleftarrow)$: Let $T_*'$ be an optimal solution to $\bf J$.
By the same domination argument, we can 
	assume w.l.o.g. that $T_*'$ consists of only dummy nodes.
Then, the optimality of $T_*$ for instance $\bf I$ can be argued
	using Eq.~\eqref{eqn:nphard} in an identical manner to the above. 
\end{proof}

This completes the proof that \CIM is NP-hard. $\square$


%In our experiments (\textsection\ref{sec:exp}) we empirically show that \CIM leads to a significant boost to the spread achieved by an $\calA$-seed set alone.
\eat{
Let $S^*_{\bf J}$ be the optimal solution to instance $\bf J$.
We construct $S^*_{\bf I}$ from $S^*_{\bf J}$ as follows:
	Let $S^*_{\bf I} = \{v\in V\mid v' \in S^*_{\bf J} \vee 
	v \in S^*_{\bf J} \}$.
And if $|S^*_{\bf I}| < b$ (because both $v$ and $v'$ are
	in $S^*_{\bf J}$ for some $v\in V$), add arbitrary nodes in
	$V$ to make it contain exactly $b$ nodes.

We claim that $S^*_{\bf I}$ is an optimal solution to $\bf I$.
If $S^*_{\bf J} \subset V'$, then the claim follows because of
	 Eq.~\eqref{eqn:nphard}.
Now suppose $S^*_{\bf J}$ contains some regular nodes from $V$:
	the boost to $\calA$-spread this set provides will not change
	if we replace all regular nodes in $S^*_{\bf J}$ with their
	corresponding dummy copies, due to that $p_{v',v} = 1$ for all $(v',v)$
	and that $\qbo = 1$.
This means that it is enough to consider only $S^*_{\bf J} \subset V'$.
Finally, if for some $v\in V$, $S^*_{\bf J}$ contains both $v$ and $v'$, 
	we can always remove one of them from the seed set $S^*_{\bf J}$ to
	achieve the same $\calB$-spread and $\calA$-spread while saving one
	seed budget.
In this case, if there is another node $u\in V$ that is not $\calB$-adopted
	with probability $1$ under the current seed set, we can always use the saved
	seed budget and set $u$ as a $\calB$ seed to achieve a higher $\calB$-spread
	and $\calA$-spread, contradicting to the assumption that $S^*_{\bf J}$
	is the optimal solution for instance $\bf J$.
Hence, in this case it must be that all nodes in $V$ are already $\calB$-adopted
	and $\calA$-adopted with probability $1$.
Therefore, we can add arbitrary nodes in $V$ into the constructed $S^*_{\bf I} $
	to make it of size $b$, and it is still the optimal solution for instance
	$\bf I$.
	
This proves the claim.
Now, suppose $S^*_{\bf J}$ can be computed in polynomial time, then
	Influence Maximization under the IC model can also be solved
	optimally in polynomial time, which is a contradiction unless P $=$ NP.
Hence, \CIM is NP-hard.
}
%I.e., we have $\sigma_{IC}(S) = \sigma_\calA(S_\calA, S') - |V'|$.
%Given that $p_{v',v} = 1$ for all $(v',v)$ and $\qbo = 1$, if \CIM can be solved optimally in polynomial time, so is Influence Maximization with IC model, which is impossible unless P $=$ NP.
%Clearly, by construction, a size-$k$ node-set $S$ is an optimal solution to $\cal I$ {\em iff} $S$ is an optimal solution to $\cal J$.
\end{proof}

\textsc{Theorem~\ref{thm:cimOpt}} (re-stated).
{\em \theoremCIMOpt}

\smallskip
The proof will rely on the possible world model as defined in \textsection\ref{sec:submod}.
Recall that each possible world consists of two real values $\alpha_\calA^v \in [0,1]$ and $\alpha_\calB^v \in [0,1]$
	for all $v\in V$.
This in theory suggests that the total number of possible worlds is infinite.
However, in terms of node-level decisions, we can create three equivalent classes of values
	for $\alpha_\calA^v$: $[0, \qao)$, $[\qao, \qab)$, $[\qab,1]$
	and $\alpha_\calB^v$: $[0, \qbo)$, $[\qbo, \qba)$, $[\qba,1]$.
By model definition, the node transition only depends on which equivalent classes $\alpha_\calA^v$ and $\alpha_\calB^v$ fall into.
There are totally nine possible combinations.
Thus, the number of ``effective'' possible worlds is still finite.

\note[Laks]{I find that the overview plot discussion above is not tightly connected with what is presented in the formal proof below. Specifically, the connection to the equivalence classes idea is not made in the proof. I'd prefer the proof to be presented top-down. If we do that, we can cut the plot discussion above. First start by restating the claim in the theorem in terms of the equivalence classes idea. Then reduce that to showing that the claim holds in individual worlds. Then give the ``for each world'' proof. } 

\begin{proof}
We first show the theorem holds in any possible world.
Consider an arbitrary PW $W$ where all edge status and $\alpha$-values of all nodes are
	determined.
Following Eq.~\eqref{eqn:labels}, when $S_\calA$ acts alone, we can classify all nodes into four
	types: $\calA$-adopted, $\calA$-rejected, $\calA$-suspended, and $\calA$-potential.
Clearly, only $\calA$-suspended and $\calA$-potential may later adopt $\calA$ with the help
	of $\calB$, and the other two types are not relevant to \CIM.
	
Now, let all nodes in $S_\calA$ be $\calB$-seeds, and thus they
	are $\calB$-adopted as well.
Since $\qbo = 1$, all nodes that can be reached by the seeds via live-edge paths will
	eventually become $\calB$-adopted, including all $\calA$-suspended and $\calA$-potential
	nodes.
For $\calA$-suspended nodes, after adopting $\calB$, they will adopt $\calA$ through
	re-consideration right away.
For $\calA$-potential nodes, the propagation of $\calA$ will reach them after $\calA$-suspended nodes
	upstream adopt $\calA$ (together with $\calB$), and after being reached, they adopt both items. 

Therefore, in this possible world, making $S_\calA$ to be $\calB$-seeds will ``convert''
	all nodes that can possibly become $\calA$-adopted, namely all $\calA$-suspended and
	$\calA$-potential nodes.
Hence, any additional $\calB$-seed will not further increase the spread of $\calA$
	as no other nodes can possibly be ``converted''.

Since the claim in this theorem holds true for any arbitrary possible world, and that
\[
\sigma_\calA(S_\calA, S_\calB) = \sum_{W\in {\cal W}} \Pr[W] \sigma_\calA^W(S_\calA, S_\calB)
\]
for all $S_\calA$ and $S_\calB$, where ${\cal W}$ denotes the set of all ``effective'' possible worlds, we have completed the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%



\subsection{Proofs for Results in Section~\ref{sec:submod}}

%%%%%%%%%%%%%%%%%%

\textsc{Lemma~\ref{lemma:pw}} (re-stated).
{\em \lemmaPW}

\begin{proof}
The proof is based on establishing equivalence on all edge-level and node-level behaviors in \model and the PW model.
By the principle of deferred decisions and the fact that each edge is only tested once in one diffusion, edge transition processes are equivalent.
To generate a possible world, the live/blocked status of an edge is pre-determined and revealed when needed, while in a Com-IC process, the status is determined on-the-fly.

Tie-breaking is also equivalent.
Note that each node $v$ only needs to apply the random permutation $\pi_v$ for breaking ties at most once.
For \comic, we need to apply $\pi_v$ only when $v$ is transitioning out of state ($\calA$-idle, $\calB$-idle) after being informed of both $\calA$ and $\calB$.
Clearly, this transition occurs at most once for each node.
The same logic applies to the PW model.
Thus, the equivalence is obvious due to the principle of deferred decisions.
%each in-neighbor of $v$ can open the information
%	channel to $v$ in at most one time step 
%	and thus it only needs to be checked in the random
%	permutation order once.

%\note[Wei Chen]{I changed the wording of the tie-breaking rule in both the rule-based
%	description and the possible world model.
%My change in the rule-based model is a convenient way to ensure that
%	event "$v$ is tested with in-neighbor $u$ and item $\calA$ or $\calB$" is always
%	well defined (alternative descriptions are possible).
%My change for the possible world model is to make it precise on the iterative 
%	descriptio step by step and on when tie-breaking is applied.
%The proof of the above paragraph reflect my changes in the model.}

The equivalence of decision-making for adoption is straightforward as $\alpha_\calA^v$ and $\alpha_\calB^v$ are chosen uniformly at random from $[0,1]$.
Hence, $\Pr[\alpha_\calA^v \leq q] = q$, where $q \in \{ \qao, \qab, \qbo, \qba \}$. 

As to reconsideration, w.l.o.g.\ we consider $\calA$.
In \model,  the probability of reconsideration is $\rho_\calA = \max\{ (\qab - \qao), 0 \} / (1 - \qao)$.
In PW, when $\qab \geq \qao$, this amounts to the probability that $\alpha_\calA^v \leq \qab$ given $\alpha_\calA^v > \qao$, which is $(\qab - \qao) / (1 - \qao)$.
On the other hand, when $\qab < \qao$, 
	$\alpha_\calA^v > \qao$ implies $\alpha_\calA^v > \qab$, which means reconsideration
	is meaningless, and this corresponds to 
	$\rho_\calA=0$ in \comic.
Thus, the equivalence is established.

Finally, the seeding protocol is trivially the same.
%The rest of the rules: initialization, seeding, and global iterations are trivially equivalent.
Combining the equivalence for all edge-level and node-level activities, we can see that the two models are equivalent and yield the same distribution of $\calA$- and $\calB$-adopted nodes, for any given $S_\calA$ and $S_\calB$.
\end{proof}


%%%%%%%%%%%%%%%%%%
\smallskip
\textsc{Theorem~\ref{thm:monotone}} (re-stated).
{\em \theoremMonotone}

\smallskip
For ease of exposition,  we also state a
	symmetric version of Theorem~\ref{thm:monotone}
	w.r.t.\ $\sigma_\calB$.
That is, {\em given any fixed $\calA$-seed set,
	$\sigma_\calB(S_\calA, S_\calB)$ is monotonically
	increasing in $S_\calB$ for any set of GAPs in
	$\bQ^+$ and $\bQ^-$.
Also, $\sigma_\calB(S_\calA, S_\calB)$ is monotonically
	increasing in $S_\calA$ for any GAPs in $\bQ^+$,
	and monotonically decreasing in $S_\calA$ for
	any $\bQ^-$.}
For technical reasons and notational convenience,
	in the proof of Theorem~\ref{thm:monotone}
	presented below, we ``concurrently'' prove both Theorem~\ref{thm:monotone}
	and this symmetric version, without loss of generality.


\begin{proof}[of Theorem~\ref{thm:monotone}]
We first fix a $\calB$-seed set $S_\calB$.
Since $S_\calB$ is always fixed, in the remaining proof we ignore $S_\calB$ from the notations whenever
	it is clear from context.
It suffices to show that monotonicity holds in an arbitrary, fixed possible world, which implies
	monotonicity holds for the diffusion model. 
Let $W$ be an arbitrary possible world generated according to \textsection\ref{sec:pw}.

Define $\Phi_\calA^W(S_\calA)$ (resp.\ $\Phi_\calB^W(S_\calA)$) to be the set of $\calA$-adopted (resp.\ $\calB$-adopted) nodes in possible world $W$ 
	with $S_\calA$ being the $\calA$-seed set (and $S_\calB$ being the fixed $\calB$-seed set).
Furthermore, for any time step $t \ge 0$, define $\Phi_\calA^W(S_\calA, t)$ (resp. $\Phi_\calB^W(S_\calA, t)$) to be the set of $\calA$-adopted (resp. $\calB$-adopted)  nodes in $W$ by the end of step $t$, given $\calA$-seed set $S_\calA$. % and (and $\calB$-seed set $S_\calB$).
Clearly, $\Phi_\calA^W(S_\calA) = \cup_{t\ge 0} \Phi_\calA^W(S_\calA, t)$ and $\Phi_\calB^W(S_\calA) = \cup_{t\ge 0} \Phi_\calB^W(S_\calA, t)$.
Let $S$ and $T$ be two sets, with $S\subseteq T\subseteq V$. 

\spara{Mutual Competition $\bQ^-$}
Our goal is to prove that for any $v \in V$, (a) if $v \in \Phi_\calA^W(S)$, then $v \in \Phi_\calA^W(T)$; 
	and (b) if $v \in \Phi_\calB^W(T)$, then $v \in \Phi_\calB^W(S)$.
Item (a) implies self-monotonic increasing property while item (b) implies cross-monotonic decreasing property.
We use an inductive proof to combine the proof of above two results together, as follows.
For every $t\ge 0$, we inductively show that $(i)$ if $v \in \Phi_\calA^W(S, t)$, then $v \in \Phi_\calA^W(T, t)$; 
	and $(ii)$ if $v \in \Phi_\calB^W(T, t)$, then $v \in \Phi_\calB^W(S, t)$.

Consider the base case of $t=0$.
If $v \in \Phi_\calA^W(S, 0)$, then it means $v \in S$, and thus $v\in T = \Phi_\calA^W(T, 0)$.
If $v \in \Phi_\calB^W(T, 0)$, it means $v \in S_\calB$, and thus $v \in \Phi_\calB^W(S, 0) = S_\calB$.

For the induction step, suppose that for all $t < t$, $(i)$ and $(ii)$ hold, and we show
	$(i)$ and $(ii)$ also hold for $t=t'$.
For $(i)$, we only need to consider $v \in \Phi_\calA^W(S, t') \setminus \Phi_\calA^W(S, t'-1)$,
	i.e. $v$ adopts $\calA$ at step $t'$ when $S$ is the $\calA$-seed set.
Since $v$ adopts $\calA$, we know that $\alpha_\calA^v \le \qao$.
Let $U$ be the set of in-neighbors of $v$ in the possible world $W$.
Let $U_\calA(S_\calA) = U \cap \Phi_\calA^W(S_\calA, t'-1)$ and
	$U_\calB(S_\calA) = U \cap \Phi_\calB^W(S_\calA, t'-1)$,
	i.e. $U_\calA(S_\calA)$ (resp. $U_\calB(S_\calA)$) is the set of in-neighbors of
	$v$ in $W$ that adopted $\calA$ (resp. $\calB$) by time $t'-1$, when $S_\calA$
	is the $\calA$-seed set.
Since $v \in \Phi_\calA^W(S, t')$, we know that $U_\calA(S) \ne \emptyset$.
By induction hypothesis, we have $U_\calA(S) \subseteq U_\calA(T)$ and $U_\calB(T) \subseteq U_\calB(S)$.

Thus, $U_\calA(T)\ne \emptyset$, which implies that by step $t'$, $v$ must have been informed of $\calA$ when $T$ is the $\calA$-seed set.
If $\alpha_\calA^v \le \qab$, then no matter if $v$ adopted $\calB$ or not, $v$ would adopt $\calA$ by step $t'$ according to the possible world model.
That is, $v \in \Phi_\calA^W(T, t')$.

Now suppose $\qab < \alpha_\calA^v \le \qao$.
For a contradiction suppose $v \not \in \Phi_\calA^W(T, t')$, i.e.,  $v$ does not adopt $\calA$ by step $t'$ when $T$ is the $\calA$-seed set.
Since $v$ has been informed of $\calA$ by $t'$, the only possibility that $v$ does not adopt $\calA$ is because $v$ adopted $\calB$ earlier than $\calA$,
	which means $v \in \Phi_\calB^W(T, t')$.
Two cases arise:

First, if $v \in \Phi_\calB^W(T, t'-1)$, then by the induction hypothesis $v \in \Phi_\calB^W(S, t'-1)$.
Since $v \in \Phi_\calA^W(S, t') \setminus \Phi_\calA^W(S, t'-1)$, it means that when $S$ is the $\calA$-seed set, $v$ adopts $\calB$ first before adopting $\calA$, but this contradicts to the condition that $\qab < \alpha_\calA^v$.
Therefore, $v \not \in \Phi_\calB^W(T, t'-1)$.

Second, $v \in \Phi_\calB^W(T, t') \setminus \Phi_\calB^W(T, t'-1)$.
Since $v \not \in \Phi_\calA^W(T, t')$, it means that $v$ is informed of $\calA$ at step $t'$ when $T$ is the $\calA$-seed set, and thus
	the tie-breaking rule must have been applied at this step and $\calB$ is ordered first before $\calA$.
However, looking at the in-neighbors of $v$ in $W$, by the induction hypothesis, 
	 $U_\calA(S) \subseteq U_\calA(T)$ and $U_\calB(T) \subseteq U_\calB(S)$.
This implies that when $S$ is the $\calA$-seed set, the same tie-breaking rule at $\calA$ would still order $\calB$ first before $\calA$, but
	this would result in $v$ not adopting $\calA$ at step $t'$, a contradiction.
Therefore, we know that $v \in \Phi_\calA^W(T, t')$.

%We now prove the induction step for $(ii)$.
The statement of $(ii)$ is symmetric to $(i)$: if we exchange $\calA$ and $\calB$ and exchange $S$ and $T$, $(ii)$ becomes $(i)$.
In fact, one can check that we can literally translate the induction step proof for $(i)$ into the proof for $(ii)$ by exchanging
	pair $\calA$ and $\calB$ and pair $S$ and $T$ (except that (a) we keep the definitions of $U_\calA(S_\calA)$ and $U_\calB(S_\calA)$, and 
	(b) whenever we say some set is the $\calA$-seed set, we keep this $\calA$).
This concludes the proof of the mutual competition case.

%We now consider the mutual complementarity case, i.e. $\qao \le \qab$ and $\qbo \le \qba$.
\spara{Mutual Complementarity $\bQ^+$}
The proof structure is very similar to that of the mutual competition case.
Our goal is to prove that for any $v \in V$, (a) if $v \in \Phi_\calA^W(S)$, then $v \in \Phi_\calA^W(T)$; 
	and (b) if $v \in \Phi_\calB^W(S)$, then $v \in \Phi_\calB^W(T)$.
To show this, we inductively prove the following: 
For every $t\ge 0$, $(i)$ if $v \in \Phi_\calA^W(S, t)$, then $v \in \Phi_\calA^W(T, t)$; 
	and $(ii)$ if $v \in \Phi_\calB^W(S, t)$, then $v \in \Phi_\calB^W(T, t)$.
The base case is trivially true.

For the induction step, suppose $(i)$ and $(ii)$ hold for all $ t < t'$, and we 
	show that $(i)$ and $(ii)$ also hold for $t=t'$.

For $(i)$, we only need to consider $v \in \Phi_\calA^W(S, t') \setminus \Phi_\calA^W(S, t'-1)$, i.e. $v$ adopts $\calA$ at step $t'$ when $S$ is the $\calA$-seed set.
Since $v$ adopts $\calA$, we know that $\alpha_\calA^v \le \qab$.
Since $v \in \Phi_\calA^W(S, t')$, we know that $U_\calA(S) \ne \emptyset$.
By induction hypothesis we have $U_\calA(S) \subseteq U_\calA(T)$.
Thus we know that $U_\calA(T)\ne \emptyset$, which implies that by step $t'$, $v$ must have been informed of $\calA$ when $T$ is the $\calA$-seed set.
if $\alpha_\calA^v \le \qao$, then no matter $v$ adopted $\calB$ or not, $v$ would adopt $\calA$ by step $t'$ according to the possible world model.
Thus, $v \in \Phi_\calA^W(T, t')$.

Now suppose $\qao < \alpha_\calA^v \le \qab$.
Since $v \in \Phi_\calA^W(S, t')$, the only possibility is that $v$ adopts $\calB$ first by time $t'$ so that after reconsideration, $v$ adopts $\calA$
	due to condition $\alpha_\calA^v \le \qab$.
Thus we have $v \in \Phi_\calB^W(S, t')$, and $\alpha_\calB^v \le \qbo$.

If $v \in \Phi_\calB^W(S, t'-1)$, by induction hypothesis $v \in \Phi_\calB^W(T, t'-1)$, which means that $v$ adopts $\calB$ by time $t'-1$ when
	$T$ is the $\calA$-seed set.
Since $v$ has been informed of $\calA$ by time $t'$ when $T$ is the $\calA$-seed set, condition $\alpha_\calA^v \le \qab$ implies that
	$v$ adopts $\calA$ by time $t'$ when $T$ is the $\calA$-seed set, i.e. $v \in \Phi_\calA^W(T, t')$.

Finally we consider the case of $v \in \Phi_\calB^W(S, t') \setminus \Phi_\calB^W(S, t'-1)$.
Looking at the in-neighbors of $v$ in $W$, $v \in \Phi_\calB^W(S, t')$, implies that $U_\calB(S) \ne \emptyset$.
By the induction hypothesis, we have $U_\calB(S) \subseteq U_\calB(T)$, and thus $U_\calB(T) \ne \emptyset$.
This implies that when $T$ is the $\calA$-seed set, node $v$ must have been informed of $\calB$ by time $t'$.
Since $\alpha_\calB^v \le \qbo$, we have that $v$ adopts $\calB$ by time $t'$ when $T$ is the $\calA$-seed set.
Then the condition $\alpha_\calA^v \le \qab$ implies that $v$ adopts $\calA$ by time $t'$ when $T$ is the $\calA$-seed set,
	i.e. $v \in \Phi_\calA^W(T, t')$.

This concludes the inductive step for item $(i)$ in the mutual complementarity case.
The induction step for item $(ii)$ is completely symmetric to the inductive step for item $(i)$. 
Therefore, we complete the proof for the mutual complementarity case.
As a result, the whole theorem holds.
\end{proof}


%%%%%%%%%%%%%%%%%%
\smallskip
\textsc{Lemma~\ref{lemma:tie}} (re-stated).
{\em \lemmaTie}

\begin{proof}
Without loss of generality, we only need to consider a node $v$ and two of its in-neighbours $u_\calA$ and $u_\calB$ which become $\calA$-adopted and $\calB$-adopted at $t-1$ respectively.
In a possible world, there are nine possible combinations of the values of $\alpha_\calA^v$ and $\alpha_\calB^v$.
We show that in all such combinations, the ordering $\pi_1  = \langle u_\calA, u_\calB \rangle$ and $\pi_2 = \langle u_\calB, u_\calA \rangle$ produce the same outcome for $v$.

{(1).\ $\alpha_\calA^v \leq \qao \wedge \alpha_\calB^v \leq \qbo$.}
Both $\pi_1$ and $\pi_2$ make $v$ $\calA$-adopted and $\calB$-adopted. 

{(2).\ $\alpha_\calA^v \leq \qao \wedge \qbo < \alpha_\calB^v \leq \qba$.}
Both $\pi_1$ and $\pi_2$ make $v$ $\calA$-adopted and $\calB$-adopted. 
With $\pi_2$, $v$ first becomes $\calB$-suspended, then $\calA$-adopted, and finally $\calB$-adopted due to re-consideration.

{(3).\ $\alpha_\calA^v \leq \qao \wedge \alpha_\calB^v > \qba$.}
Both $\pi_1$ and $\pi_2$ makes $v$ $\calA$-adopted only. 

{(4).\ $\qao < \alpha_\calA^v \leq \qab \wedge \alpha_\calB^v \leq \qbo$.}
%With both orderings, $v$ would adopt both $\calA$ and $\calB$, 
Symmetric to (2).
%In particular, if $U_\calA$ is ordered first, $v$ first becomes $\calA$-suspended and then adopts $\calA$ by reconsideration.

{(5).\ $\qao < \alpha_\calA^v \leq \qab \wedge \qbo < \alpha_\calB^v \leq \qba$.}
%It is easy to see that $v$ would adopt neither item.
In this case, $v$ does not adopt any item.

{(6).\ $\qao < \alpha_\calA^v \leq \qab \wedge \alpha_\calB^v > \qba$.}
In this case, $v$ does not adopt any item.

{(7).\ $\alpha_\calA^v > \qab \wedge \alpha_\calB^v \leq \qbo$.}
Symmetric to (3): $v$ is $\calB$-adopted only.
%$v$ only adopts $\calB$ and cannot adopt $\calA$ in either ordering.

{(8).\ $\alpha_\calA^v > \qab \wedge \qbo < \alpha_\calB^v \leq \qba$.}
Symmetric to (6).

{(9).\ $\alpha_\calA^v > \qab \wedge \alpha_\calB^v > \qba$.}
In this case, $v$ does not adopt any item.

Since the possible world model is equivalent to Com-IC (Theorem~\ref{lemma:pw}), the lemma holds as a result.
\end{proof}



%%%%%%%%%%%%%%%%%%

\smallskip
\textsc{Lemma~\ref{lemma:indiff}} (re-stated).
{\em \lemmaInDiff}

\begin{proof}
Consider an arbitrary possible world $W$.
Let $q := \qbo = \qba$.
A node $v$ becomes $\calB$-adopted in $W$ as long as $\alpha_\calB^v \leq q$ and there is a live-edge path $P_\calB$ from $S_\calB$ to $v$ such that for all nodes $w$ on $P_\calB$ (excluding seeds), $\alpha_\calB^w \leq q$.
Since $\qbo = \qba$, this condition under which $v$ becomes $\calB$-adopted in $W$ is completely independent of any node's state w.r.t.\ $\calA$.
Thus, the propagation of $\calB$-adoption is completely independent of the actual $\calA$-seed set (even empty).
Due to the equivalence of the possible world model and Com-IC, the lemma holds.
\end{proof}


%%%%%%%%%%%%%%%%%%

\smallskip
\textsc{Claim~\ref{clm:bjoina}} (re-stated).
{\em \lemmaClaimBA}

\begin{proof}[of Claim~\ref{clm:bjoina}]
Since $P_\calA$ is an $\calA$-path (where all nodes are $\calA$-adopted), every node $w$ on $P_\calA$ (except the starting node)
	has $\alpha^w_\calA \le \qab$.
For every such node $w$, if $\qao < \alpha^w_\calA \le \qab$, then $w$ adopting $\calA$ implies that
	$w$ must have adopted $\calB$ first and $\alpha^w_\calB \le \qbo$.
	
Now suppose a node $w$ on the path adopts $\calB$ (under some $\calB$-seed set), and all nodes before $w$
	on path $P_\calA$ are $\calA$-ready.
Then all nodes before $w$ on this path adopts $\calA$ regardless of $\calB$-seed set.
Thus $w$ is informed of $\calA$.
Since $\alpha^w_\calA \le \qab$, $w$ adopts $\calA$.

Then consider the node $w'$ after $w$ on the path $P_\calA$.
Node $w'$ must be informed by both $\calA$ and $\calB$ since $w$ adopts
	both $\calA$ and $\calB$ and the edge $(w,w')$ is live.
If $\alpha^{w'}_\calA \le \qao$, $w'$ will adopt $\calA$, and then since $\qba =1$,
	$w'$ will then adopt $\calB$ -- this is where we use the key assumption that $\qba = 1$.
If $\qao < \alpha^{w'}_\calA \le \qab$, then we have argued that in this case $\alpha^{w'}_\calB \le \qbo$,
	so $w'$ would adopt $\calB$, followed by adopting $\calA$.
We can then inductively use the above argument along the path to show that every node after
	$w$ will adopt both $\calA$ and $\calB$, which proves the claim.
\end{proof}


%%%%%%%%%%%%%%%%%%

\smallskip
\textsc{Claim~\ref{clm:bpathcrosssub}} (re-stated).
{\em \claimBPath}

\begin{proof}[of Claim~\ref{clm:bpathcrosssub}]
We construct such a path $P_\calB$ backwards from $w$ as follows.

Since $w$ adopts $\calB$, if $w \in T \cup\{u\}$, then we are done; otherwise, 
	there must be some $\calB$-path $P'_{\calB}$ from 
	$\calB$-seed set $T\cup \{u\}$ to $w$.
If $P'_{\calB}$ is a $\calB$-ready path, then we have found $P_\calB$ to be $P'_{\calB}$,
 	and its starting node is $x_0$. 
This is because even if $x_0$ is the only $\calB$-seed, $\calB$ can still pass through all nodes on $P_\calB$
	to reach $w$, without the need of any node on the path to adopt $\calA$, because by definition,
	all nodes $v$ on a $\calB$-ready path satisfies that $\alpha_\calB^v \leq \qbo$. 

Now suppose $P'_{\calB}$ is not $\calB$-ready.
	It is clear that every non-$\calB$-ready node on path
	$P'_{\calB}$ must be $\calA$-ready (otherwise, it would not be possible
	for such a node to adopt $\calB$).
If every such non-$\calB$-ready node has an $\calA$-ready path from $S_\calA$, then
	we still find $P_\calB = P'_{\calB}$ with its starting node is $x_0$.
This is because whenever $\calB$ reaches a non-$\calB$-ready node on the path, the node has an $\calA$-ready path
	from $S_\calA$ and thus the node always adopt $\calA$, which means it will also adopt $\calB$ (for $\qba = 1$).

Now consider the case where 
	there exists some non-$\calB$-ready node on path $P'_{\calB}$ that does not have 
	any $\calA$-ready path from $S_\calA$.
Let $x_1$ be the first such node (we count backwards from $w$).	
By the definition of $x_1$, we know that as long as $x_1$ adopts $\calB$
	(regardless what is the actual $\calB$-seed set), then $x_1$ would
	pass $\calB$ along path $P'_{\calB}$ to $w$.
Thus our backward construction has found the last piece of the path $P_\calB$ as the
	path segment of $P'_{\calB}$ from $x_1$ to $w$, now we move the construction
	backward starting from $x_1$.

At $x_1$, find a $\calA$-path $P'_{\calA}$ from $S_\calA$ to $x_1$.
By the definition of $x_1$\footnote{Recall that it is $\calA$-ready, on a $\calB$-path, and there is no $\calA$-ready path from $S_\calA$ to $x_1$}, we know that $P'_{\calA}$ is not $\calA$-ready.
Let $x_2$ be the first non-$\calA$-ready node on path $P'_{\calA}$ counting forward from the starting $\calA$-seed.
Then $x_2$ must have adopted $\calB$.
By Claim~\ref{clm:bjoina}, we know that as long as $x_2$ adopts $\calB$,
	all nodes after $x_2$ on path $P'_{\calA}$ would adopt both $\calA$ and $\calB$, regardless of the actual
	$\calB$-seed set.
Applying this to $x_1$, we know that $x_1$ is both $\calA$- and $\calB$-adopted.
Then our backward construction has found the next piece of $P_\calB$, which 
	is the path segment of $P'_{\calA}$ from $x_2$ to $x_1$, which guarantees that if $x_2$
	adopts $\calB$, then $w$ must eventually adopt $\calB$.
	
Now if $x_2$ is a $\calB$-seed, we are done.
If not, we will repeat the above ``zig-zag constructions'': there must be a
	$\calB$-path $P''_{\calB}$ from $\calB$-seed set $T\cup \{u\}$ to $x_2$.
The argument on path $P''_{\calB}$ is exactly the same as the argument on $P'_{\calB}$, 
	and if the construction still cannot stop, we will find path $P''_{\calA}$
	similar to $P'_{\calA}$, and so on.
	
The construction keeps going backwards, and since the construction actually follows the strict adoption
	time line and going backward in time, in the diffusion process when $T\cup \{u\}$ is the $\calB$-seed set,
	the construction must eventually reach a $\calB$-seed $x_0$ and stops.
Then we have found the desired path $P_\calB$ and the desired starting node $x_0$.
\end{proof}
	

%\subsection{Proof of Theorem~\ref{thm:cimOpt}}



\subsection{Proofs for Results in Section~\ref{sec:rrset}}

%%%%%%%%%%%%%%%%%%
\textsc{Lemma~\ref{lemma:generic-rr}} (re-stated).
{\em \lemmaGenericRR}

\begin{proof}
It is sufficient to prove that in every possible world $W \in \mathcal{W}$, $S$ activates $v$ if and only if $S$ intersects with $v$'s RR set in $W$, denoted by $R_W(v)$.

Suppose $R_W(v) \cap S \neq \emptyset$.
Without loss of generality, we assume a node $u$ is in the intersection.
By the definition of RR set, set $\{u\}$ can activate $v$ in $W$.
Per Property~{\it (P1)}, $S$ can also activate $v$ in $W$.

Now suppose $S$ activates $v$ in $W$.
Per Property~{\it (P2)}, there exists $u\in S$ such that $\{u\}$ can also activate $v$ in $W$.
Then by the RR-set definition, $u \in R_W(v)$.
Therefore, $S \cap R_W(v) \neq \emptyset$.
\end{proof}


%%%%%%%%%%%%%%%%%%
\smallskip
\textsc{Lemma~\ref{lemma:generic-rr-2}} (re-stated).
{\em \lemmaGenericRRSubmod}

\begin{proof}
First consider ``if''.
Suppose both properties hold in $W$.
Monotonicity directly follows from Property~{\it (P1)}.
For submodularity, suppose $v$ can be activated by set $T \cup \{x\}$ but not by $T$, where $x\not\in T$.
By Property~{\it (P2)}, there exists some $u \in T \cup \{x\}$ such that $\{u\}$ can activate $v$ in $W$.
If $u \in T$, then $T$ can also activate $v$ by Property~{\it (P1)}, a contradiction.
Hence we have $u = x$.
Then, consider any subset $S \subset T$.
Note that by Property~{\it (P1)}, $S$ cannot activate $v$ (otherwise so could $T$), while $S \cup \{x\}$ can.
Thus, $f_{v,W}(\cdot)$ is submodular.

Next we consider ``only if''.
Suppose $f_{v,W}(\cdot)$ is monotone and submodular for every $v\in V$.
Property~{\it (P1)} directly follows from monotonicity.
For Property~{\it (P2)}, suppose for a contradiction that there exists a seed set $S$ that can activate $v$ in $W$, but there is no $u\in S$ so that $\{u\}$ activates $v$ alone.
We repeatedly remove elements from $S$ until the remaining set is the minimal set that can still activate $v$.
Let the remaining set be $S'$.
Note that $S'$ contains at least two elements.
Let $u\in S'$, and then we have
	$f_{v,W}(\emptyset)=f_{v,W}(\{u\})=f_{v,W}(S'\setminus \{u\})=0$,
	but $f_{v,W}(S') = 1$, which violates submodularity, a contradiction.
This completes the proof.
\end{proof}


%%%%%%%%%%%%%%%%%%
\smallskip
\textsc{Theorem~\ref{thm:rrsim-correct}} (re-stated).
{\em \theoremRRSIMCorrect}

\begin{proof}
It suffices to show that, given a fixed possible world $W$, a fixed $\calB$-seed set $S_\calB$, and a certain node $u\in V$, for any node $v\not\in \Phi_\calA^W(\emptyset, S_\calB)$ with $\alpha_\calA^v \leq \qab$, we have: $v\in \Phi_\calA^W(\{u\}, S_\calB)$ if and only if there exists a live-edge path $P$ from $u$ to $v$ such that for all nodes $w\in P$, excluding $u$, $w$ satisfies $\alpha_\calA^w \leq \qab$, and in case $\alpha_\calA^w > \qao$,  then $w$ must be $\calB$-adopted.

The ``if'' direction is straightforward as $P$ will propagate the adoption information of $\calA$
	all the way to $v$.
If $\alpha_\calA^v \leq \qao$, it adopts $\calA$ without question.
If $\alpha_\calA^v \in (\qao, \qab]$, then $v$ must be $\calB$-adopted by the definition of $P$, which makes it $\calA$-adopted.

For the ``only if'' part,  suppose no such $P$ exists for $u$.
This leads to a direct contradiction since $u$ is the only $\calA$-seed, and $u$ lacks a live-edge path to $v$, it is impossible for $v$ to get informed of $\calA$, let alone adopting $\calA$.
Next, suppose there is a live-edge path $P$ from $u$ to $v$, but there is a certain node $w\in P$ which violates the conditions set out in the lemma.
First, $w$ could be have a ``bad'' threshold: $\alpha_\calA^w > \qab$.
In this case, $w$ will not adopt $\calA$ regardless of its status w.r.t.\ $\calB$, and hence the propagation of $\calA$ will not reach $v$.
Second, $w$ could have a threshold such that $\alpha_\calA^w \in (\qao, \qab]$ but it does not adopt $\calB$ under the influence of the  given $S_\calB$.
Similar to the previous case, $w$ will not adopt $\calA$ and the propagation of $\calA$ will not reach $v$.
This completes the ``only if'' part.

Then by Definition~\ref{def:generalRRset}, the theorem follows.
\end{proof}


%%%%%%%
\smallskip
\textsc{Lemma~\ref{lemma:rr-sim-time}}
{\em \lemmaRRSIMRuntime } (re-stated).

\begin{proof}
Given a fixed RR-set $R\subseteq V$, let $\omega(R)$ be the number
	of edges in $G$ that point to nodes in $R$.
Since in \timsim, it is possible that we do not examine incoming
	edges to a node added to the RR-set
	({\em cf}.\ Cases 1$(ii)$ and 2$(ii)$ in the backward BFS),
	we have:
\begin{align*}
\EPT_B \leq \mathbb{E}[\omega(R)],
\end{align*}
where the expectation is taken over the random choices of $R$.
By Lemma 4 in \cite{tang14} (note that this lemma only relies on 
	the activation equivalence property of RR-sets, which holds true
	in our current one-way complementarity setting), 
\begin{align*}
\frac{|V|}{|E|}\cdot \mathbb{E}[\omega(R)] \leq \OPT_k.
\end{align*}
This gives
\[
\frac{|V|}{|E|} \cdot \EPT_B \leq \OPT_k.
\]
Following the same analysis as in~\cite{tang14} one can check that the lower bound
	$LB$ of $\OPT_k$ obtained by the estimation method in
		\cite{tang14} guarantees that $LB \ge \EPT_B\cdot |V|/|E|$.
Since in our algorithm we set $\theta = \lambda / LB$, where (following Eq.\eqref{eqn:opt})
\[
\lambda = \epsilon^{-2} \left((8+2\epsilon)|V| \left(\ell \log|V| + \log\binom{|V|}{k} + \log 2\right) \right),
\]
then we have that the expected running time of generating all RR-sets is:

\begin{align*}
O(\theta \cdot \EPT)
&= O(\frac{\lambda}{LB} \cdot (\EPT_F + \EPT_B)) \\
&= O\left(\frac{\lambda|E|}{|V| \EPT_B} (\EPT_F + \EPT_B) \right) \\
&= O\left(\frac{\lambda|E|}{|V|} \left(1+ \frac{\EPT_F}{\EPT_B} \right) \right) \\
& = O\left((k+\ell)(|V|+|E|)\log |V|\left(1+ \frac{\EPT_F}{\EPT_B}\right) \right).
\end{align*}

The time complexity for estimating $LB$ and for calculating the final seed set 
	given RR-sets are the same as in~\cite{tang14}, and thus the final complexity
	is $O\left((k+\ell)(|V|+|E|)\log |V|\left(1+ \frac{\EPT_F}{\EPT_B}\right) \right)$.
\end{proof}



%%%%%%%%%%%%%%%%%%
\smallskip
\textsc{Theorem~\ref{thm:rrcim-correct}} (re-stated).
{\em \theoremRRCIMCorrect}

\begin{proof}
It suffices to show the following claim.

\begin{claim}\label{clm:rrcim-correct}
Consider any fixed possible world $W$, a fixed $\calA$-seed set $S_\calA$, and a certain node $u\in V$.
Then, for any node $v\not\in \Phi_\calA^W(S_\calA, \emptyset)$ with $\alpha_\calA^v \leq \qab$, we have: $v\in \Phi_\calA^W(S_\calA, \{u\})$ if and only if there exists a live-edge path $\mathcal{P}(u,v)$ from $u$ to $v$ such that one of the following holds :

$(i)$.\ $\mathcal{P}(u,v)$ consists entirely of $\calA$-adopted or diffusible $\calA$-suspended/potential nodes, and $u$ must be $\calA$-suspended, or

$(ii)$.\ There exists an $\calA$-suspended node $u' \neq u$ on $\mathcal{P}(u,v)$, such that all nodes on the sub-path of $\mathcal{P}(u,u')$ (excluding $u$) are $\calB$-diffusible and the remaining ones (excluding $u'$ and $v$) are either $\calA$-adopted or diffusible $\calA$-suspended/potential.
\end{claim}

\begin{proof}[of Claim~\ref{clm:rrcim-correct}]
$(\Longleftarrow).$
Suppose $(i)$ holds.
Clearly, $u$ will adopt $\calB$ first as a seed and then adopt $\calA$ by reconsideration.
Then all nodes on $\mathcal{P}(u,v)$ including $v$ will adopt both $\calA$ and $\calB$ since they are either $\calA$-adopted or diffusible $\calA$-suspended/potential.
Consider any node $w \neq v$ on  $\mathcal{P}(u,v)$: if $w$ is already $\calA$-adopted, it will adopt $\calB$ since $\qba = 1$; otherwise, $w$ adopts $\calB$ first since $\alpha_\calB^w \leq \qbo$ (diffusible) and then $\calA$.
Next, suppose $(ii)$ holds.
Since $S_\calB = \{u\}$, $u$ adopts $\calB$, so do all nodes on $\mathcal{P}(u,u')$.
Since $u'$ is $\calA$-suspended, it will then adopt $\calA$ by reconsideration.
The rest of the argument is exactly the same as the case above.

$(\Longrightarrow).$
Since $v$ is $\calA$-adopted, there must exist a live-edge path on $P_\calA$ from $S_\calA$ to $v$ such that all nodes on $P_\calA$ are $\calA$-adopted.
Suppose every node $w \in P_\calA$ have $\alpha_\calA^w \leq \qao$, then all nodes on $P_\calA$ would adopt $\calA$ when $S_\calB = \emptyset$, including $v$, which is a contradiction.
Thus, there exists at least one node $w\in P_\calA$ such that $\qao < \alpha_\calA^w \leq \qab$.
Let $w_1$ be the first of such nodes, counting from upstream.
In order for $v$ to adopt $\calA$, $w_1$ must adopt $\calA$, and in order for that to happen, $w_1$ must adopt $\calB$ first.

If the sub-path $\mathcal{P'}(w_1,v)$ does not have non-diffusible nodes, then it satisfies $(i)$ and $w_1 = u$ as in the theorem.
Now suppose there is one node $w_2 \in \mathcal{P'}(w_1,v)$ that is non-diffusible, i.e., $\alpha_\calB^{w_2} > \qbo$ and $\qao < \alpha_\calA^{w_2} \le \qab$.
This means in order for $w_2$ to adopt $\calA$ and $\calB$, it must be a seed for either or both items.
By construction, $w_2$ is not an $\calA$-seed, and thus it must be a $\calB$-seed.
Next, since $w_1$ adopts $\calB$ and $w_2$ is the only $\calB$-seed, there must be a live-edge path of $\calB$-diffusible nodes from $w_2$ to $w_1$.
In this way, $\mathcal{P'}(w_2,v)$ satisfies $(ii)$, with $w_2 = u$ and $w_1 = u'$ as in the theorem.
Also note that if there are more than one non-diffusible nodes on $\mathcal{P'}(w_1,v)$, all of them must be $\calB$-seeds in order to make $v$ adopt $\calA$.
Since the theorem only considers singleton $\calB$-seed sets, such paths will not lead $v$ to adopt $\calA$ with only one non-diffusible node as $\calB$-seed.
This completes the proof.
\end{proof}

By Definition~\ref{def:generalRRset}, the theorem thus holds true.
\qed
\end{proof}


%%%%%%%%%%
\smallskip
\textsc{Lemma~\ref{lemma:rrcim-time}} 
{\em \lemmaRRCIMTime} (re-stated).

\begin{proof}
The following inequality continues to hold for \timcim,
	by applying Lemma 4 in \cite{tang14}.
\[
 |V| \cdot \EPT_{BS} / |E| \leq \OPT_k,
\]
%\[
% |V| \cdot \mathbb{E}[\omega(R)] / |E| \leq \OPT_k,
%\]
%where $\omega(R)$ is the number of edges pointing
%	to a node in $R$, given a fixed $R$.
%To estimate a lower bound of $\OPT_k$, for \timcim,
%	we do not include the eligible non-diffusible
%	$\calA$-potential nodes that are also in $R$, but
%	only focus on edges pointing to $\calA$-suspended nodes.
%Clearly,
%\[
%|V| \cdot EPT_{BS} / |E| \leq  |V| \cdot \mathbb{E}[\omega(R)] / |E| \leq \OPT_k.
%\]

%With this, in the execution of \generalTIM \& \timcim, we can 
%	estimate $LB$ of $\OPT_k$ by the method in \cite{tang14}, but
%	only counting the edges pointing to $\calA$-suspended nodes.
%We use $\EPT_{BO}$ to denote the expected number of all other
%	edges examined in Phase~\rom{2}, including primary
%	and all secondary searches.
Since we employ lazy sampling (of possible worlds), we conclude
	that $\EPT_F + \EPT_{BS} + \EPT_{BO} \leq |E|$.
That is, in the process of generating a single RR-set, the worst case
	is to flip a coin for every edge, and every edge becomes live, and
	the search goes on.
The rest of the analysis is similar to Lemma~\ref{lemma:rr-sim-time}, and finally,
	the expected time complexity for \generalTIM + \timcim is
\[
O\left((k+\ell)(|V|+|E|)\log |V|\left(1+ \frac{\EPT_F+\EPT_{BO}}{\EPT_{BS}}\right) \right).
\]
\end{proof}


%%%%%%%%%%%%%%%%%%
%\smallskip
%\textsc{Lemma~\ref{lemma:rr-sim-plus}} (re-stated).
%{\em \lemmaRRSIMPlus}

\def\lemmaRRSIMPlus{
Consider any possible world $W$ under the \comic model.
Let $v$ be a root for generating an RR-set.
For any $u\in V$ that is backward reachable from $v$ via live-edges in $W$, $u$ is determined as $\calB$-adopted in \timsim if and only if $u$ is determined as $\calB$-adopted in \timsimfast.
}

\begin{lemma}\label{lemma:rr-sim-plus}
{\lemmaRRSIMPlus}
\end{lemma}


\begin{proof}
We first prove the ``if'' part.
Suppose $u$ is determined as $\calB$-adopted in \timsimfast.
This means that there exists a node $s \in T_1 \cap S_\calB$, such that there is a path from $s$ to $u$ consisting entirely of live-edges and $\calB$-adopted nodes (every node $w$ on this path satisfies that $\alpha_\calB^w \leq \qbo$).
Therefore, in \timsim, where $W$ is generated upfront, this live-edge path must still exist.
Thus, $u$ must be also $\calB$-adopted in \timsim as well.

Next we prove the ``only if'' part.
By definition, if $u$ is determined as $\calB$-adopted in possible world $W$, then there exists a path $P$ from some $s \in S_\calB$ to $u$ such that the path consists entirely of live edges and all nodes $w$ on the path satisfy that $\alpha_W^w \leq \qbo$.
It suffices to show that if $u$ is reachable by $v$ backwards in $W$, then $P$ will be explored entirely by \timsimfast.

Suppose otherwise.
That is, there exists a node $z \in P$, such that $z$ cannot be explored by the first round backward BFS from $v$.
We have established that in the complete possible world $W$, there is a live-edge path from $z$ to $u$ and from $u$ to $v$ respectively.
Thus, connecting the two paths at node $u$ gives a single live-edge path $P_z$ from $z$ to $v$.
Now recall that the continuation of the first backward BFS phase in \timsimfast relies solely on edge status (as long as an edge $(w,u)$ is determined live, $w$ will be visited by the BFS).
This means that $z$ must have been explored in the first backward BFS allow the backward
	path from $v$ to $u$ and then along the path $P$, which is a contradiction.
\end{proof}


%%%%%%%%%%%%%%%%%%
\smallskip
\textsc{Theorem~\ref{thm:sandwich}} (re-stated).
{\em 
Sandwich Approximation solution gives:
$$ %\begin{align} \label{eqn:sandapprox}
\sigma(S_{\mathit{sand}}) \ge \max \Big\{\frac{\sigma(S_\nu)}{\nu(S_\nu)}, \frac{\mu(S_\sigma^*)}{\sigma(S_\sigma^*)} \Big\}
  \cdot (1-1/e) \cdot  \sigma(S_\sigma^*),
$$ %\end{align}
where $S_\sigma^*$ is the optimal solution maximizing $\sigma$ (subject to  cardinality constraint $k$).
}


\begin{proof}
Let $S_\mu^*$ and $S_\nu^*$ be the optimal solution to maximizing $\mu$ and $\nu$ respectively.
We have
{\normalsize 
\begin{multline}\label{eqn:Snu}
 \sigma(S_\nu)  = \frac{ \sigma(S_\nu)}  {\nu(S_\nu)} \cdot \nu(S_\nu)  \geq \frac{\sigma(S_\nu)} {\nu(S_\nu)} \cdot (1-1/e) \cdot \nu(S_\nu^*) \\ 
 \geq \frac{\sigma(S_\nu)}{\nu(S_\nu)} \cdot (1-1/e) \cdot \nu(S_\sigma^*) \geq \frac{\sigma(S_\nu)}{\nu(S_\nu)} \cdot (1-1/e) \cdot \sigma(S_\sigma^*);
\end{multline}}
\vspace{-4mm}
{\normalsize
\begin{multline}\label{eqn:Smu}
\sigma(S_\mu) \geq \mu(S_\mu) \geq (1-1/e) \cdot \mu(S_\mu^*) \geq (1-1/e) \cdot \mu(S_\sigma^*) \\
 \geq \frac{\mu(S_\sigma^*)}{\sigma(S_\sigma^*)} \cdot (1-1/e) \cdot  \sigma(S_\sigma^*).
\end{multline}
}

The theorem follows by applying Eq. \eqref{eqn:sand}, the definition of $S_{\mathit{sand}}$.
\end{proof}

%%%%%%%%%%%%%%%%%%
\smallskip
\textsc{Theorem~\ref{thm:mono-q}} (re-stated).
{\em \theoremMonoQ}

\begin{proof}[(Sketch)]
The detailed proof would follow the similar induction proof structure for each possible world 
	as in the proof of Theorem~\ref{thm:monotone}.
Intuitively, 
%	for the mutual competition case, we would prove inductively that at every step increasing
%	$\qao$ or $\qab$ would increase $\calA$-adopted nodes and decrease $\calB$-adopted nodes;
%	for the mutual complementarity case, 
	we would prove inductively that at every step increasing
	$\qao$ or $\qab$  would increase both $\calA$-adopted and $\calB$-adopted nodes.
\end{proof}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Submodularity  Analysis for Competitive Cases of Com-IC}

%In competitive cases, there is no meaningful reasons
%	to study cross-submodularity as in the complementary settings.

First, we address cross-submodularity.
Note that by Theorem~\ref{thm:monotone}, $\sigma_\calA$ is monotonically decreasing w.r.t.\ $S_\calB$ (with any fixed $S_\calA$).
Intuitively, cross-submodularity for competitive products means adding an additional $\calB$-seed to a smaller $\calB$-seed set yields a larger decrease in the spread of $\calA$: for any $S\subseteq T\subseteq V$ and any $u\not\in T$, $\sigma_\calA(S_\calA, S) - \sigma_\calA(S_\calA, S\cup \{u\}) \geq \sigma_\calA(S_\calA, T) - \sigma_\calA(S_\calA, T\cup \{u\})$.
This notion is relevant and useful to the problem of influence blocking maximization, where one party wants to find the best seed set to block the spread of competitors~\cite{HeSCJ12,BudakAA11}.
Since influence blocking is not the focus of this work, from here on, we focus on self-submodularity and self-monotonicity only, and hereafter we
	drop ``self-'' in the terminologies.


When $q_{A|\emptyset} = q_{B|\emptyset} = 1$ and $q_{A|B} = q_{B|A} = 0$, the Com-IC model degenerates to 
	the homogeneous CIC model, for which submodularity and monotonicity both hold~\cite{infbook}.
In the general $\bQ^-$ setting, monotonicity holds (Theorem~\ref{thm:monotone}).
However, the following counter-example shows the opposite for submodularity.

\begin{example}%[Non-Self-Submodularity]
\label{exp:nonsub}
{\em
Consider the graph in Figure~\ref{fig:non-sub-compete}, where all edges have an influence probability of $1$.
Values of $\bQ$ are: $\qao = q \in (0,1)$, $\qab = \qba = 0$, $\qbo = 1$.
The $\calB$-seed set is $S_\calB = \{y\}$.
For $\calA$-seed set $S_\calA$, let $S = \{s_1\}$, $T = \{s_1, s_2\}$, and $u = s_3$.

We consider the probability $v$ becomes $\calA$-adopted with $S_\calA$, denoted by $ap_\calA(v, S_\calA)$ ($S_\calB$ is omitted since it is clear from context):
\begin{align*}
&ap_\calA(v, S) = 0, \\
&ap_\calA(v, S \cup \{u\}) = q^2, \\
&ap_\calA(v,T) = 0, \\
&ap_\calA(v,T \cup \{u\}) = q^2 + (1-q)\cdot q^6.
\end{align*}
%Thus, the marginal gain of $u$ w.r.t.\ $T$ is larger by $(1-q)\cdot q^6 > 0$, which is positive since $q\in (0,1)$.
Hence, we have
\begin{align*}
&\big(ap_\calA(v,T \cup \{u\}) - ap_\calA(v,T) \big) - \big(ap_\calA(v, S \cup \{u\}) - ap_\calA(v,S) \big)  \\
&= (1-q)\cdot q^6 > 0.
\end{align*}
Non-submodularity occurs for the entire graph if $v$ is replicated sufficiently many times.
\qed
}
\end{example}

The intuition of the above counter-example is that $\calA$-seeds $s_2$ and $s_3$
	together can block $\calB$ completely, and
	thus even if they cannot successfully activate $v$ to adopt $\calA$, $s_1$ could 
	later activate $v$ (with the additional probability $(1-q)\cdot q^6$), but
	when $s_2$ or $s_3$ acts alone, it cannot block $\calB$, so the influence of $\calA$
	from $s_1$ will not reach $v$.


\begin{figure}[t]
 \centering
   \includegraphics[width=0.5\textwidth]{graphics/counterExample3-competitive}
   \caption{Graph for Example~\ref{exp:nonsub}}
   \label{fig:non-sub-compete}
\end{figure}



Next, we show a positive result which says that submodularity is satisfied
	as long as $q_{A|\emptyset} = q_{B|\emptyset} = 1$.

\begin{theorem}
In the Com-IC model, when $q_{A|\emptyset} = q_{B|\emptyset} = 1$, the influence spread function $\sigma_\calA(S_\calA, S_\calB)$ is \emph{submodular} w.r.t.\ $S_\calA$, for any given $S_\calB$.
\end{theorem}

\begin{proof}
We fix a $\calB$-seed set $S_\calB$ and consider an arbitrary possible world $W$ to show
	that submodularity is satisfied in $W$.
%Hence, by Theorem~\ref{lemma:pw} and the linearity of submodularity, this submodularity of $\sigma^X(S_\calA, S_\calB)$ follows.

In the possible world $W$, for an $\calA$-adopted node $v$, there must exist a live-edge path from $\calA$-seed set $S_\calA$ to
	$v$ with all nodes on the path adopting $\calA$, and we call this path an $\calA$-path
	($\calB$-path is defined symmetrically).
With mutual competition, the length of the shortest $\calA$-path from $S_\calA$ to $v$ is the
	same as the time step at which $v$ adopts $\calA$.
This is because in competitions when a node is informed about an item, it only has one chance at the
	same time step to decide about the adoption (reconsideration in later steps is not possible).

\begin{claim}\label{clm:aorb}
If a node $v$ is reachable from $S_\calA$ or $S_\calB$ in the possible world $W$, then $v$ must adopt at least one of $\calA$ and $\calB$.
\end{claim}

\begin{proof}[of Claim~\ref{clm:aorb}]
This is due to the fact that $\qao = \qbo = 1$.
In this case, suppose a node $v$ is reachable from $S_\calA$, i.e. there is a path from $S_\calA$ to $v$ in the possible world $W$.
The claim can be proven by an induction on the path length.
Essentially, no matter which item an earlier node on the path adopts, it would inform the next node on the path, and since
	$\qao=\qbo=1$, the node would adopt the first item it get informed.
\end{proof}


Let $S\subseteq T \subseteq V$ be two sets of nodes, and $u\in V \setminus T$ be an additional $\calA$-seed.
For a fixed $\calB$-seed set $S_\calB$ (omitted from the following notations), let $\Phi_\calA^W(S_\calA)$ denote the set of $\calA$-adopted nodes in the possible world $W$ with $\calA$-seed set $S_\calA$ after the diffusion ends.
Consider a node $v \in \Phi_\calA^W(T \cup \{u\}) \setminus \Phi_\calA^W(T)$.
We need to show $v \in \Phi_\calA^W(S \cup \{u\}) \setminus \Phi_\calA^W(S)$.

We now construct a shortest $\calA$-path, denoted $P_\calA$, from some node 
	in $w_0 \in T \cup \{u\}$ to $v$ when $S_\calA = T \cup \{u\}$.
The path construction is done backwards.
Starting from $v$, if $v$ has only one in-neighbor $w$ attempting to inform $v$ through the 
	live edge (open information channel) from $w$ to $v$, 
	then in the previous time step, $w$ must have adopted $\calA$, and we select $w$ as the predecessor of $v$ on path $P_\calA$. 
If there are multiple in-neighbors that have live edges pointing to $v$, 
%let $w$ be the one ordered before all such in-neighbors which adopted $X$ or $XY$,
we examine the permutation $\pi_v$ and pick $w$ as $v$'s predecessor on this path, such that $w$ ranks first over all of $v$'s in-neighbors that adopted $\calA$ in the previous time step.
%and we select $w$ as the predecessor of $v$.
%Similarly, this node $w$ must have adopted $X$, or both with $X$ being adopted first.
We trace back and stop once we reach an $\calA$-seed in $T \cup \{u\}$.
It is clear that $P_\calA$ must be a shortest $\calA$-path from $T \cup \{u\}$ to $v$, since in every construction
	step we move back one time step.

\begin{claim}\label{clm:source}
Let $w_0 \in T \cup \{u\}$ be the starting point of $P_\calA$.
Then, even when $S_\calA = \{w_0\}$, all nodes on $P_\calA$ would still adopt $\calA$.
\end{claim}

\begin{proof}[of Claim~\ref{clm:source}]
Suppose, for a contradiction, that some node on $P_\calA$ \textsl{does not adopt $\calA$} when $S_\calA = \{w_0\}$.
Let $w$ be the first of such nodes on $P_\calA$ (counting from $w_0$)\footnote{$w \neq w_0$, since as a seed, $w_0$ adopts $\calA$ automatically.}.
By Claim~\ref{clm:aorb}, $w$ must adopt $\calB$ as it does not adopt $\calA$.
This means that there must exist a $\calB$-path from $S_\calB$ to $w$.
We construct a shortest $\calB$-path $P_\calB$  from $S_\calB$ to $w$ in the same way as we constructed $P_\calA$:
	start from $w'=w$ backwards and always select the in-neighbor of the current node $w'$ that adopts $\calB$ and is ordered first in $\pi_w$.
Moreover, since $w$ is informed of $\calA$ (by its predecessor on path $P_\calA$) but does not adopt $\calA$,
	it holds that $\qab < \alpha_\calA^w \leq \qao$ in $W$.

%\note[Wei]{Need to consider: what if $w_\calA = w_\calB$?}

We now compare the length of $P_\calB$, denoted by $\ell_\calB$, to the length
	of the segment of $P_\calA$ from $w_0$ to $w$, denoted by $\ell_\calA$.
Suppose $\ell_\calB > \ell_\calA$. Then $w$ would still adopt $\calA$ when $S_\calA = \{w_0\}$
	(regardless of whether it will adopt $\calB$ or not), a contradiction.
%If $\ell(P_\calB) < \ell(P_\calA[w_0, w])$, then $w$ would adopt $\calB$ first and reject $\calA$ even when $S_\calA = T \cup \{u\}$. % (as $P_\calB$ would still be effective with $T \cup \{u\}$, ).
Next consider $\ell_\calB < \ell_\calA$.
When $T \cup \{u\}$ is the $\calA$-seed set, from $\calB$-seed set $S_\calB$ and through the path $P_\calB$, every time step one more node
	on path $P_\calB$ has to adopt either $\calA$ or $\calB$ (by Claim~\ref{clm:aorb}).
Thus by time step $\ell_\calB$, $w$ adopts either $\calA$ or $\calB$.
But since $P_\calA$ is the shortest $\calA$-path from $T \cup \{u\}$ to $w$ and $\ell_\calA > \ell_\calB$, $w$ cannot adopt $\calA$
	at step $\ell_\calB$, so $w$ must adopt $\calB$ at step $\ell_\calB$.
Since $\alpha_\calA^w > \qab$, it means that $w$ would not adopt $\calA$ after adopting $\calB$, also a contradiction.

We are left with the case $\ell_\calB = \ell_\calA$.
Let $w_\calA$ and $w_\calB$ be the predecessor of $w$ on $P_\calA$ and $P_\calB$, respectively.
Assume $w_\calA \neq w_\calB$ (we deal with $w_\calA = w_\calB$ later).
If $w_\calA$ is ordered ahead of $w_\calB$ in $\pi_w$, then according to the tie-breaking rule, 
	$w$ would be informed of $\calA$ first and adopt $\calA$ (since $\alpha_\calA^w \le \qao$) when $w_0$ is the only $\calA$-seed,
	contradicting the definition of $w$.

If $w_\calB$ is ordered ahead of $w_\calA$ in $\pi_w$, then consider again the scenario when $S_\calA = T \cup \{u\}$.
By Claim~\ref{clm:aorb},  through the path $P_\calB$, $w_\calB$ adopts either $\calA$ or $\calB$ by step $\ell_\calB-1$.
If $w_\calB$ adopts $\calA$, it contradicts the construction of $P_\calA$ since we would have chosen $w_\calB$ instead of $w_\calA$ in the
	backward construction.
If $w_\calB$ adopts $\calB$, then $w$ would be informed of $\calB$ from $w_\calB$ first, and then due to
	$\alpha_\calA^w > \qab$, $w$ would not adopt $\calA$, again a contradiction.

Finally, we also need to consider the case of $w_\calA=w_\calB$.
Since $w$ does not adopt $\calA$ when $w_0$ is the only $\calA$-seed, according to our tie-breaking rule, node
	$w_\calA$ must adopt $\calB$ first and then adopt $\calA$ at the same step.
We then trace back the predecessor of $w_\calA$ on path $P_\calA$  and $P_\calB$ respectively.
If these two paths never branch backward, i.e. $P_\calA = P_\calB$, 
	then we know that $w_0$ is both $\calA$ and $\calB$-seed.
According to the possible world model we would use $\tau_{w_0}$ to decide whether $w_0$ adopts $\calA$ or $\calB$ first, and
	then all nodes on the path $P_\calA = P_\calB$ would follow the same order.
Since $w_\calA$ adopts $\calB$ first before $\calA$, we know that $\tau_{w_0}$ is such that $\calB$ is ranked ahead of $\calA$.

Now we consider the scenario when $S_\calA = T \cup \{u\}$.
By the construction of path $P_\calA$, the successor of $w_0$ on this path, $w_1$, orders $w_0$ first among all
	$\calA$-adopted in-neighbors, so $w_1$ would take $w_0$ to get informed of $\calA$, but since $w_0$ adopts $\calB$ first,
	this implies that $w_1$ also adopts $\calB$ first.
We can apply the same argument along the path $P_\calA$ to see that $w$ adopts $\calB$ first before $\calA$.
However, since $\alpha_\calA^w > \qab$, we know that $w$ would not adopt $\calA$, a contradiction.

If paths $P_\calA$ and $P_\calB$ branch at some node $x$ when we trace backward, then let $x_\calA$
	and $x_\calB$ are the two predecessors of $x$ on paths $P_\calA$  and $P_\calB$ respectively, and 
	$x_\calA \ne x_\calB$.
When $w_0$ is the only $\calA$-seed, we know from above that $w_\calA$ adopts $\calB$ first before adopting $\calA$.
By the construction of $P_\calB$, $w_\calA$ must be informed of $\calB$ from its predecessor on $P_\calB$, so if this
	predecessor has not branched yet, it must also adopts $\calB$ before $\calA$.
Using the same argument, we know that $x$ must adopt $\calB$ first before adopting $\calA$.
Then we know that $x_\calB$ must be ordered before $x_\calA$ in $\pi_x$.
Now consider the scenario when $S_\calA = T \cup \{u\}$.
The argument is exactly the same as the previous case of $w_\calB$ ordered before $w_\calA$, and we also reach a contradiction.

We have exhausted all cases and Claim~\ref{clm:source} is proven.
\end{proof}

Claim~\ref{clm:source} immediately implies that $w_0 = u$, since otherwise, we have $w_0 \in T$, and
	by the proof of monotonicity (Theorem~\ref{thm:monotone}) we know that $v \in \Phi_\calA^W(\{w_0\}) \subseteq \Phi_\calA^W(T)$.
This contradicts with the definition of $v \in \Phi_\calA^W(T \cup \{u\}) \setminus \Phi_\calA^W(T)$.

Again by monotonicity, we have $v \in \Phi_\calA^W(\{u\}) \subseteq \Phi_\calA^W(S \cup \{u\})$.
Since $S \subseteq T$ and $v \not\in \Phi_\calA^W(T)$, then $v \not\in \Phi_\calA^W(S)$.
This gives $v \in \Phi_\calA^W(S \cup \{u\}) \setminus \Phi_\calA^W(S)$, which was to be shown. \qed
\end{proof}




==> sec-staticRef.tex <==
\begin{thebibliography}{10}
%\smallskip
\small
\bibitem{nethept}
\newblock {\url{http://research.microsoft.com/en-us/people/weic/graphdata.zip}}.

\bibitem{twitter}
\newblock {\url{https://snap.stanford.edu/data/}}.


\bibitem{fullpaper}
P.~Banerjee, W.~Chen, L.~V.~S.~Lakshmanan, and W.~Lu.
\newblock Welfare maximization under economically postulated independent cascade model.
\newblock submitted to arxiv.org, June 2018.

\bibitem{BharathiKS07}
S.~Bharathi, D.~Kempe, M.~Salek.
\newblock Competitive influence maximization in social networks.
\newblock In {\em WINE}, pages 306--311, 2007.

\bibitem{borgs14}
C.~Borgs et al.
\newblock Maximizing social influence in nearly optimal time.
\newblock In {\em SODA}, pages 946--957, 2014.

\bibitem{cohen14} 
Edith Cohen, Daniel Delling, Thomas Pajor, Renato F. Werneck:
\newblock Sketch-based Influence Maximization and Computation: Scaling up with Guarantees. 
\newblock CIKM 2014, pages 629--638. 

\bibitem{foldes2000valuation}
L.~Foldes.
\newblock Valuation and martingale properties of shadow prices: An exposition.
\newblock In {\em Journal of Economic Dynamics and Control}, pages 1641--1701, 2000.

\bibitem{frittelli2000introduction}
M.~Frittelli.
\newblock Introduction to a theory of value coherent with the no-arbitrage principle.
\newblock In {\em Finance and stochastics}, pages 275--297, 2000.


\bibitem{easyim} 
S. Galhotra, A. Arora, and S. Roy. 
\newblock Holistic influence maximization: Combining scalability and efficiency with opinion-aware models. 
\newblock In SIGMOD, pages 743-758, 2016.

\bibitem{hodges1989optimal}
Stewart D.~Hodges.
\newblock Optimal replication of contingent claims under transaction costs.
\newblock In {\em Review of futures markets}, pages 223--238, 1989. 

\bibitem{hirshleifer1978}
J.~Hirshleifer. 
\newblock The private and social value of information and the reward to inventive activity.
\newblock In {\em Uncertainty in Economics}, pages 541--556, 1978.

\bibitem{Albertbidding07}
A.~Jiang and K. Leyton-Brown.  
\newblock Bidding agents for online auctions with hidden bids.
\newblock In {\em Machine Learning}, pages 117--143, 2007. 

\bibitem{kim2013}
J.~Kim et al.
\newblock Scalable and parallelizable processing of influence maximization for large-scale social networks.
\newblock In {\em ICDE}, pages 266--277, 2013.

\bibitem{jung2012}
J.~Kyomin et al.
\newblock Irie: Scalable and robust influence maximization in social networks.
\newblock In {\em ICDM}, pages 918--923, 2012. 

\bibitem{myerson1981optimal}
Roger B.~Myerson.
\newblock Optimal auction design.
\newblock In {\em Mathematics of operations research}, pages 58--73, 1981.

\bibitem{nisan2007}
N.~Nisan et al.  
\newblock Algorithmic game theory.
\newblock Cambridge university press, 2007. 

\bibitem{rasmusen1994}
E.~Rasmusen and B.~Blackwell.
\newblock Games and information.
\newblock In {\em MA 15}, 1994.


\bibitem{seeman2013}
L.~Seeman et al.
\newblock Adaptive seeding in social networks.
\newblock In {\em FOCS}, pages 459--468, 2013.



\bibitem{lu2015}
W.~Lu, W.~Chen, L.~V.~S. Lakshmanan.
\newblock From competition to complementarity: comparative influence diffusion and maximization.
\newblock In {\em VLDB}, pages 60--71, 2015.

\bibitem{lu2015arxiv}
W.~Lu, W.~Chen, L.~V.~S. Lakshmanan.
\newblock From competition to complementarity: comparative influence diffusion and maximization.
\newblock {\url {https://arxiv.org/pdf/1507.00317.pdf}}.

\bibitem{goyal11}
A.~Goyal et al.
\newblock A data-based approach to social influence maximization.
\newblock In {\em VLDB}, pages 73--84, 2011.

\bibitem{borodin10}
A.~Borodin et al.
\newblock Threshold models for competitive influence in social networks.
\newblock In {\em WINE}, pages 539--550, 2010.

\bibitem{buchbinder12}
N.~Buchbinder et al.
\newblock A tight linear time (1/2)-approximation for unconstrained submodular maximization.
\newblock In {\em SIAM Journal on Computing}, pages 1384--1402, 2015.

\bibitem{BudakAA11}
C.~Budak, D.~Agrawal, A.~El~Abbadi.
\newblock Limiting the spread of misinformation in social networks.
\newblock In {\em WWW}, pages 665--674, 2011.

\bibitem{CarnesNWZ07}
T.~Carnes et al.
\newblock Maximizing influence in a competitive social network: a follower's perspective.
\newblock In {\em ICEC}, pages 351--360, 2007.

\bibitem{ChenWW10}
W.~Chen, et al.
\newblock Scalable influence maximization for prevalent viral marketing in large-scale social networks.
\newblock In {\em KDD}, pages 1029--1038, 2010.

\bibitem{ChenWW10b}
W.~Chen, Y.~Yuan, and L.~Zhang.
\newblock Scalable influence maximization in social networks under the linear threshold model.
\newblock In {\em ICDM}, pages 88--97, 2010. 

\bibitem{ChenWW10c} 
Wei Chen, Yajun Wang, and Siyu Yang. Efficient Influence Maximization in Social Networks. Proceedings of the 15th ACM SIGKDD Conference on Knowledge Discovery and Data Mining (KDD'2009), Paris, France, June 2009.

\bibitem{ChenNegOpi11}
W.~Chen, et al.
\newblock Influence maximization in social networks when negative opinions may emerge and propagate.
\newblock In {\em SDM}, pages 379--390, 2011.

\bibitem{infbook}
W.~Chen, L.~V.~S. Lakshmanan, and C.~Castillo.
\newblock Information and Influence Propagation in Social Networks.
\newblock Synthesis Lectures on Data Management. Morgan {\&} Claypool
  Publishers, 2013.

\bibitem{dattaMS10}
S.~Datta, A.~Majumder, and N.~Shrivastava.
\newblock Viral marketing for multiple products.
\newblock In {\em ICDM 2010}, pages 118--127, 2010.

\bibitem{domingos01}
P.~Domingos and M.~Richardson.
\newblock Mining the network value of customers.
\newblock In {\em KDD}, pages 57--66, 2001.
  
\bibitem{Huang2017}  
K.~Huang et al. 
\newblock Revisiting the stop-and-stare algorithms for influence maximization.
\newblock In {\em VLDB}, pages 913--924, 2017.

\bibitem{Nguyen2016}
Hung T.~Nguyen et al. 
\newblock Stop-and-stare: Optimal sampling algorithms for viral marketing in billion-scale networks.
\newblock In {ICDM}, pages 695--710, 2016.


%
%\bibitem{goldenberg01}
%J.~Goldenberg, B.~Libai, and E.~Muller.
%\newblock Talk of the network: A complex systems look at the underlying process
%  of word-of-mouth.
%\newblock {\em Marketing Letters}, 12(3):211--223, 2001.

\bibitem{amit2010}
A.~Goyal, F.~Bonchi, and L.~V.~S. Lakshmanan.
\newblock Learning influence probabilities in social networks.
\newblock In {\em WSDM}, pages 241--250, 2010.
%
%\bibitem{granovetter78}
%M.~Granovetter.
%\newblock Threshold models for collective behavior.
%\newblock {\em The American Journal of Sociology}, 83(6):1420--1443, 1978.

\bibitem{HeSCJ12}
X.~He et al.
\newblock Influence blocking maximization in social networks under the competitive linear threshold model.
\newblock In {\em SDM}, pages 463--474, 2012.

\bibitem{kalish85}
S.~Kalish.
\newblock A new product adoption model with price, advertising, and uncertainty.
\newblock {\em Management Science}, 31(12):1569--1585, 1985.

\bibitem{kempe03}
D.~Kempe, J.~M. Kleinberg, and {\'E}.~Tardos.
\newblock Maximizing the spread of influence through a social network.
\newblock In {\em KDD}, pages 137--146, 2003.
%
%\bibitem{Kostka2008}
%J.~Kostka, Y.~A. Oswald, and R.~Wattenhofer.
%\newblock Word of mouth: Rumor dissemination in social networks.
%\newblock In {\em SIROCCO}, 2008.

\bibitem{lu2013}
W.~Lu, et al.
\newblock The bang for the buck: fair competitive viral marketing from the host perspective.
\newblock In {\em KDD}, pages 928--936, 2013.


\bibitem{mcauley15}
J.~J. McAuley, R.~Pandey, and J.~Leskovec.
\newblock Inferring networks of substitutable and complementary products.
\newblock In {\em KDD}, pages 785--794, 2015.

\bibitem{myers12}
S.~A. Myers and J.~Leskovec.
\newblock Clash of the contagions: Cooperation and competition in information diffusion.
\newblock In {\em ICDM}, pages 539--548, 2012.

\bibitem{narayanam2012viral}
R.~Narayanam and A.~A. Nanavati.
\newblock Viral marketing for product cross-sell through social networks.
\newblock In {\em PKDD}, pages 581--596, 2012.

\bibitem{submodular}
G.~L. Nemhauser, L.~A. Wolsey, and M.~L. Fisher.
\newblock An analysis of approximations for maximizing submodular set functions.
\newblock {\em Mathematical Programming}, 14(1):265--294, 1978.

\bibitem{cramton-etal-ca-book-2007} 
P.~Cramton et al. 
\newblock  Combinatorial Auctions. 
\newblock MIT Press, 2006. 

\bibitem{feige-vondrak-demand-2010}
U.~Feige and J.~Vondr\'ak. 
\newblock The Submodular Welfare Problem with Demand Queries.
\newblock In {\em Theory of Computing}, volume 6, number 11, pages 247--290, 2010.

\bibitem{simpath} 
A. Goyal et al. 
\newblock 
SIMPATH: An Efficient Algorithm for Influence Maximization under the Linear Threshold Model. 
\newblock ICDM 2011, pages 211--220. 


\bibitem{kapraov-etal-greedy-opt-soda-2013} 
M.~Kapralov et al. 
\newblock  Online Submodular Welfare Maximization: Greedy is Optimal. 
\newblock In {\em SODA}, pages 1216--1225, 2013.

\bibitem{korula-etal-online-swm-arxiv-2017} 
N.~Korula et al. 
\newblock  Online Submodular Welfare Maximization: Greedy Beats 1/2 in Random Order. 
\newblock  {CoRR}, {abs/1712.05450}, {2017}. 


\bibitem{pmc} 
N. Ohsaka, T. Akiba, Y. Yoshida, and K. Kawarabayashi. 
\newblock Fast and accurate influence maximization on large networks with pruned monte-carlo simulations. 
\newblock AAAI Conference, Quebec City, Canada., pages 138--144, 2014.

\bibitem{PathakBS10}
N.~Pathak, A.~Banerjee, and J.~Srivastava.
\newblock A generalized linear threshold model for multiple cascades.
\newblock In {\em ICDM}, pages 965--970, 2010.

%\bibitem{richardson02}
%M.~Richardson and P.~Domingos.
%\newblock Mining knowledge-sharing sites for viral marketing.
%\newblock In {\em KDD}, pages 61--70, 2002.

\bibitem{snyder08}
C.~Snyder and W.~Nicholson.
\newblock Microeconomic Theory, Basic Principles and Extensions (10th ed).
\newblock 2008.

\bibitem{tang15}
Y.~Tang, Y.~Shi, and X.~Xiao.
\newblock Influence maximization in near-linear time: a martingale approach.
\newblock In {\em SIGMOD}, pages 1539--1554, 2015.

\bibitem{tang14}
Y.~Tang, X.~Xiao, and Y.~Shi.
\newblock Influence maximization: near-optimal time complexity meets practical efficiency.
\newblock In {\em SIGMOD}, pages 75--86, 2014.

\bibitem{yuan2013we}
N.~Yuan et al.
\newblock We know how you live: exploring the spectrum of urban lifestyles.
\newblock In {\em COSN}, pages 3--14, 2013.



\end{thebibliography}


==> sec-sub_algo.tex <==
\subsubsection{Absence of the power of bundling}
  
First, we present the challenges that a submodular value function poses. In particular, the power of bundling is not present when the value is submodular. Hence it is difficult to come up with any simple greedy way of allocating the items. We present three different approaches that we can take and highlight the limitations of each of those approaches.

\spara{Pure greedy}

The first algorithm we present is called pure greedy, \pgrd \ for short. The pseudo code is shown in Algorithm \ref{alg:pgrd}. Given a graph and itemset, the algorithm greedily chooses a (node,item)-pair that maximizes the marginal gain in social welfare (line \ref{lin:pgreed}). The algorithm terminates once all budgets are exhausted or there is no further allocation that results is non-negative marginal gain in the welfare.

\begin{algorithm}[t!]
%\begin{small} 
\DontPrintSemicolon
\caption{  $\pgrd(I,\bvec, (\val,\price,\noise), G =(V,E))$} \label{alg:pgrd}
%Sort the items in non-increasing order of their budgets, i.e., $b_1 \geq ... \geq b_m$ \;
$\greedAlloc \leftarrow \emptyset$; \\ 

\While{$I$ is not empty}  {
	For $i \in I$ and $v \in V$, choose that $(v,i)$ pair that maximizes and has a non-negative $\rho((v,i)\mid \greedAlloc)$\; \label{lin:pgreed}
	$\greedAlloc \leftarrow \greedAlloc \cup (v,i)$\;
	$b_i$ $=$ $b_i -1$\;
	\If{$b_i = 0$} {
		Remove $i$ from $I$\;
	}
}	
%
\textbf{return} $\greedAlloc$ as the final allocation\;  

%\vspace{-8mm}
%\end{small}
\end{algorithm}


The problem with pure greedy is that it fails to detect that even an item which can have a high individual utility, may always reduces a bundle's utility when the item is bundled with other items. \pgrd allocates such an item to the best node, which can potentially cause a drop in the utility in the of the number of items. We formalize this problem of pure greedy next in the following lemma.


\begin{figure*}
	\centering
	\includegraphics{figs/greedy_counter2.PNG}
  \caption{Network for \pgrd } \label{fig:gc2}
\end{figure*}


\begin{lemma}\label{pgreedyq2}
Given an $\epsilon >0$, social welfare of pure greedy allocation can be $\frac{1+2 \epsilon}{m - 2}$ factor worse than the optimal welfare, when value is monotone and submodular, price is additive and there is no noise, and $m$ is the total number of items.
\end{lemma}

\begin{proof}

Consider an item set $\itemset = \{i_1, ..., i_m\}$, where $|\itemset| = m$. Let the budget be 1 for each item. The items propagate in a network that is shown in Figure \ref{fig:gc2}. All edge probabilities are 1. The value configuration is as follows. Every singleton item except item $i_1$ has value $2$, value of $i_1$ is $2 + 2 \epsilon$. We consider an explicit order among the items of the set $\itemset \setminus \{i_1 \cup i_2\}$. Let the order be based on the increasing index number, i.e. $i_3 > i_4> ... > i_m$. For an item subset involving $i_2$ and item in the specified order, value is set to be additive. Since each of those items has a value of 2, $\val(\{i_2 \cup i_3\}) = 4, \val(\{i_2 \cup i_3 \cup i_4\}) = 6, ... \val(\{i_2 \cup i_3 \cup ... \cup i_m\}) = 2m-2 $. For any other item (sub)set, its value is obtained by adding a marginal gain of $1 - \epsilon$ for every additional item added to the set. This value configuration conforms to submodularity.

Since item $i_1$ has the highest individual value in the itemset, \pgrd allocates $i_1$ to node $A$, the node having maximum expected reach. Once it allocates $i_1$ to $A$, since allocating any other item to $A$ reduces the welfare, \pgrd will allocate all other items to node $C$. Hence the overall allocation of \pgrd is $\greedAlloc = \{(A,i_1), (C,i_2), ..., (C,i_m)\}$. If the total number of nodes in the graph is $n$, then the allocation produces social welfare of $O((1 + 2 \epsilon) \times n)$. 

However, the optimal allocation should not allocate $i_1$ to $A$. In that case, it can allocate all the items that have additive values as a bundle to $A$. Hence the optimal allocation is $\optAlloc = \{(C,i_1), (A,i_2), ..., (A,i_m)\}$ and the corresponding optimal welfare is $O((m-2) \times n)$. This shows that the performance of greedy can be worse as the number of items increases.

\end{proof}

The problem with \pgrd stems from the fact that it ignores the effect of bundling altogether. Our next algorithm tries to mitigate this issue by considering all possible item bundles.

\spara{Subset greedy}

Instead of considering a singleton item, we consider all item subsets to choose the best allocation. The pseudo-code is presented in Algorithm \ref{alg:sgrd}. All item subsets that have a non-negative utility are selected in the $\mathbf{C}$ set, line \ref{lin:sgreed_1}. Next the (item subset, node)-pair is iteratively chosen that maximizes the marginal social welfare. The algorithm terminates once all budgets are exhausted or there is no further allocation that results is non-negative marginal gain in the welfare.

\begin{algorithm}[t!]
%\begin{small} 
\DontPrintSemicolon
\caption{  $\sgrd(I,\bvec, (\val,\price,\noise), G =(V,E))$} \label{alg:sgrd}
$\mathbf{I} \leftarrow 2^I, \mathbf{C} \leftarrow \emptyset$; \\

\For{$\mathcal{I} \in \mathbf{I}$}{
	\If{$\util(\mathcal{I}) \ge 0$} {
		$\mathbf{C} \leftarrow \mathbf{C} \cup \mathcal{I}$ \label{lin:sgreed_1}
	
	}
}
 
$\greedAlloc \leftarrow \emptyset$; \\ 

\While{$\mathbf{C}$ is not empty}  {
	For $\mathcal{C} \in \mathbf{C}$ and $v \in V$, choose that $(v,\mathcal{C})$ pair that maximizes and has a non-negative $\rho((v,\mathcal{C})\mid \greedAlloc)$\; \label{lin:sgreed_2}
	\For{$i \in \mathcal{C}$}{
		$\greedAlloc \leftarrow \greedAlloc \cup (v,i)$\;
		$b_i$ $=$ $b_i -1$\;
		\If{$b_i = 0$} {
			Remove $i$ from $I$\;
		}
	}
}	
%
\textbf{return} $\greedAlloc$ as the final allocation\;  

\end{algorithm}


By scanning over all possible item subsets, instead of singleton items while computing the marginal, \sgrd avoids the bottleneck of \pgrd. However it suffers from the problem of the other end. By choosing the highest utility item subset, it fails to choose a combination of two subsets that other subsets which when combined produce higher utility than the highest utility subset alone. It becomes more apparent when budget is more than 1. We will show that using an example next. 

\begin{figure*}
	\centering
	\includegraphics{figs/blockgreedy_counter.PNG}
  \caption{Network for \sgrd} \label{fig:bgc}
\end{figure*}

\begin{example}

Consider the network shown in Figure \ref{fig:bgc}. Let there be three items propagating in the network: $\{i_1,i_2,i_3\}$ and their values and prices be as follows.\\
$\val(\{i_1\}) = v_1+1, \price(\{i_1\}) = 1$,\\
$\val(\{i_2\}) = v_2+1, \price(\{i_2\}) = 1$,\\
$\val(\{i_3\}) = v_3+1, \price(\{i_3\}) = 1$,\\
$\val(\{i_1,i_2\}) = v_1 + v_2+2, \val(\{i_1,i_3\}) = v_1 + v_3+2$ \\
$\val(\{i_1,i_2,i_3\}) = \max\{v_1 + v_2, v_1+v_3\} +\epsilon +3$.\\

The item subsets with positive utilities are $\{i_1\}, \{i_2\}, \{i_3\}, \{i_1,i_2\}, \{i_1,i_3\}, \{i_2,i_3\}, \{i_1,i_2,i_3\}$.

Now consider the budget vector to be $\bvec = \{2,1,1\}$. Also assume $v_1>v_2>v_3$.\\
The subset greedy allocation will first select the pair $(A_1,\{i_1,i_2,i_3\})$ as this has the highest marginal gain in terms of the social welfare and then it will select $(B_1,i_1)$.
Thus the overall subset greedy allocation is $\{(A_1, i_1),(A_1, i_2),(A_1, i_3),(B_1, i_1)\}$. The welfare of this allocation is $(v_1+v_2+\epsilon)\times m+v_1 \times m$. \\
However the optimal allocation is $\{(A_1,i_1),(A_1,i_2),(B_1,i_1),(B_1,i_3)\}$ resulting in a welfare of $(v_1+v_2)\times m + (v_1+v_3) \times m$.\\
Hence the ratio is $\frac{2 v_1 + v_2 + \epsilon}{2 v_1 + v_2 + v_3}$. By setting $2 v_1 + v_2 = k $, we get a ratio of $\frac{k + \epsilon}{k + v_3}$.

\end{example}  

In this section we highlighted the difficulties of not having the power of bundling. We showed how two seemingly promising approaches fail to mitigate it. We are currently investigating other alternatives that can help us.


\subsubsection{Absence of the reachability property}

Unlike complementary items, competing items donot exhibit the reachability property. Instead, competing items can cause \textit{item blocking}, where propagation of a superior product can be blocked by an inferior product. Depending on the network structure, this can reduce the welfare of a greedy allocation that does not take into account the effect of item blocking. We next highlight a major consequence of the item blocking issue under the \pgrd allocation, which can be extended similarly for other greedy choices such as \sgrd.

For this discussion, assume that an inner world is fixed. I.e., all the edge probabilities and the noise terms are sampled. Let the sampled network be the one shown in Figure \ref{fig:bgc}.

==> sec-sub_prop.tex <==
Note that the noise and edge probabilities remain to be the same as under complementary items. Consequently, the possible world interpretation also remains to be the same as described in \textsection\ref{sec:prop_pw}. We donot repeat it for brevity.
We instead directly proceed to investigate the properties of the social welfare. For the rest of the discussion, we consider that value is monotone and submodular, price is additive and noise is global.

\subsubsection{Properties of social welfare} 

First we show that the monotonicity does not hold for social welfare under competitive items.

\begin{restatable}{theorem}{thmnotmonotone}
Expected social welfare is not monotone with respect to the sets of node-item allocation pairs.
\end{restatable}


\begin{proof} 

We give a counter example to monotonicity. Consider a network consisting of two nodes $v_1$ and $v_2$ with a single directed edge from $v_1$ to $v_2$, with probability 1. Let there be two items $i_1$ and $i_2$. Let $\val(i_1) > \price(i_1)$ and $\val(i_2) > \price(i_2)$. However $\val(\{i_1,  i_2\}) < \price(i_1) + \price(i_2)$. Assume that noise terms are bounded random variables, i.e., $|\noise(i_j)| \le |\val(i_2) - \price(i_2)|$, $j=1,2$. Lastly $\val(i_1) > 2 \val(i_2)$ and $\price(i_1)< 2 \times \price(i_2)$.
	Thus expected individual expected utilities of $i_1$ or $i_2$ are positive, but when they are offered together, the expected utility is negative. Further individual expected utility of $i_1$ is always higher than that of $i_2$.
	Now consider two seed allocations $\allalloc = \{(v_1,i_1)\}$ and $\allalloc' = \{(v_1, i_1),(v_2,i_2)\}$. Clearly $\allalloc \subset \allalloc'$. Under allocation $\allalloc$, both nodes $v_1$ and $v_2$ will adopt $i_1$ in every possible world. However under $\allalloc'$ $v_1$ adopts $i_1$ and $v_2$ adopts $i_2$ in every possible world. Thus we have,
	
	\begin{align*}
	\rho(\allalloc) &= 2 * \mathbb{E}[\util(i_1)]  \\
	& > \mathbb{E}[\util(i_1)] + \mathbb{E}[\util(i_2)] \\
	&= \rho(\allalloc')
	\end{align*}
	which breaks the monotonicity
	
\end{proof}

We next show two other counter examples for submodularity and supermodularity.

\begin{restatable}{theorem}{thmnotsubsuper2}
Expected social welfare is neither submodular nor supermodular, with respect to the sets of node-item allocation pairs.
\end{restatable}

\begin{proof}

We show two counter examples
	
	\noindent 
	\underline{Submodularity}: Consider the network with three nodes $v_1$, $v_2$ and $v_3$. There are two directed edges; one from node $v_1$ to $v_3$ and the other from $v_2$ to $v_3$. All edge probabilities are $1$. Let there be three items $\{\ia,\ib,\ic\}$ propagating in the network. Their values are prices be as follows:\\
$\val(\{\ia\}) = 2 + p, \price(\{\ia\}) = p$\\
$\val(\{\ib\}) = 1 + p$, $\price(\{\ib\}) = p$\\
$\val(\{\ic\}) = 1 + p, \price(\{\ic\}) = p$\\
$\val(\{\ia,\ib\}) = -1 + 2p$, $\val(\{\ia,\ic\})=-1 + 2p$\\
$\val(\{\ib,\ic\})=2 + 2p $\\
$\val(\{\ia,\ib,\ic\})= -5 + 3p$.

Let noise be a bounded random variable $|\noise(i_j)| \le p$, $j = 1,2,3$.

Now consider two allocations $\allalloc = \{(v_1,\ia)\}$ and $\allalloc' = \{(v_1,\ia),(v_3,\ib)\}$. Clearly $\allalloc \subset \allalloc'$. Further, let the additional allocation pair be $(v_2,\ic) \notin \allalloc'$. Hence we get,

	\begin{align*}
	\rho(\allalloc \cup \{(B,\ic)\}) - \rho(\allalloc) &= \mathbb{E}[\util(i_2)] \\
	&>2 \times \mathbb{E}[\util(i_2)] \\
	&= \rho(\allalloc' \cup \{(B,\ic)\}) - \sw(\allalloc')
	\end{align*}

which breaks the submodularity.
	
	\noindent
	\underline{Supermodularity}: For supermodularity, consider a network consisting of two nodes $v_1$ and $v_2$ with a single directed edge from $v_1$ to $v_2$, with probability 1. Let there be one item $i$ whose deterministic utility is positive, i.e., $\val(i) > \price(i)$. Again, assume that the noise term $\noise(i)$ is a bounded random variable, i.e., $|\noise(i)| \le |\val(i) - \price(i)|$. 
	Now consider two seed allocations $\allalloc = \emptyset$ and $\allalloc' = \{(v_1, i)\}$. Let the additional pair be $(v_2, i)$. Under allocation $\allalloc'$, both nodes $v_1$ and $v_2$ will adopt $i$ in every possible world. Hence adding the additional pair $(v_2, i)$ does not change item adoption in any world and consequently the expected social welfare is unchanged. Thus we have,
	
	\begin{align*}
	\rho(\allalloc \cup \{(v_2, i)\}) - \rho(\allalloc) &= \mathbb{E}[\util(i_1)] \\
	&>0  \\
	&= \rho(\allalloc' \cup \{(v_2, i)\}) - \rho(\allalloc')
	\end{align*} 
	which breaks supermodularity.  
	
	
\end{proof} 


Since welfare is neither monotone nor submodular or supermodular, designing an approximately optimal solution for the \emph{WelMax} (Problem \ref{prob:welmax}) is difficult. In the following section we investigate closely the challenges that the setting puts forward.
